Computational and Data Requirements for Learning Generic Properties of Simulation-Based Games

Empirical game-theoretic analysis (EGTA) is primarily focused on learning the equilibria of simulation-based games. Recent approaches have tackled this problem by learning a uniform approximation of the game's utilities, and then applying precision-recall theorems: i.e., all equilibria of the true game are approximate equilibria in the estimated game, and vice-versa. In this work, we generalize this approach to all game properties that are well behaved (i.e., Lipschitz continuous in utilities), including regret (which defines Nash and correlated equilibria), adversarial values, and power-mean and Gini social welfare. Further, we introduce a novel algorithm -- progressive sampling with pruning (PSP) -- for learning a uniform approximation and thus any well-behaved property of a game, which prunes strategy profiles once the corresponding players' utilities are well-estimated, and we analyze its data and query complexities in terms of the a priori unknown utility variances. We experiment with our algorithm extensively, showing that 1) the number of queries that PSP saves is highly sensitive to the utility variance distribution, and 2) PSP consistently outperforms theoretical upper bounds, achieving significantly lower query complexities than natural baselines. We conclude with experiments that uncover some of the remaining difficulties with learning properties of simulation-based games, in spite of recent advances in statistical EGTA methodology, including those developed herein.

==> algorithms/GS.tex <==
\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\Procedure{GS}{$\ConditionalGame{\ConditionSpace}, \ConditionDistribution, \UtilityIndices, \NumberOfSamples, \delta, \UtilityRange, \textsc{Bound}$} 
$\to \UtilityIntervals$
%$\to \UtilityIntervals_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$

% UNIFORM
%$\to (\tilde{\Utility}, \bm{\varepsilon})$

\State \Input Conditional game $\ConditionalGame{\ConditionSpace}$, black box 
%$\BlackBox$ 
from which we can sample distribution $\ConditionDistribution$,
index set $\UtilityIndices$, sample size $\NumberOfSamples$, failure probability $\delta$, utility range $\UtilityRange$, and bound type \textsc{Bound}.

% UNIFORM
%\State \Output Empirical utilities $\tilde{\Utility}, \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$, and additive error $\bm{\varepsilon}$. \amy{update}

\State \Output Empirical utility intervals $\UtilityIntervals$
%$\UtilityIntervals_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$.

\State $\Samples \sim \ConditionDistribution^\NumberOfSamples$ \Comment{Draw $\NumberOfSamples$ samples from distribution $\ConditionDistribution$}

%\State $\hat{\GameTuple} \gets \GameTuple_{\Samples}$ \Comment{Empirical estimate of $\expectedGame{\ConditionDistribution}$}

\State 
$\tilde{\Utility}_{\PlayerIndex} (\StratProfile) \gets
%\frac{1}{\NumberOfSamples}\sum_{\SampleIndex=1}^\NumberOfSamples \Utility_\PlayerIndex(\StratProfile; \Samples_\SampleIndex),
\hat{\Utility}_{\PlayerIndex}(\cdot; \Samples), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
\Comment{Compute empirical utilities}

%\State $\hat{\GameTuple}_{\Samples} \gets \langle \SetOfPlayers, \{\StrategySet\}_{i=1}^{\NumberOfPlayers}, \hat{\Utility} (\cdot) \rangle$ \Comment{Empirical game}

%\State $\hat{\GameTuple}_{\Samples} \gets \textsc{ConstructGame}(\GameTuple, \Samples)$ \Comment{Empirical estimate of $\InducedGame{\ConditionDistribution}$}

\If{\textsc{Bound} = \textsc{1-ERA}}

    \State $\vsigma \gets \Rademacher^{\NumberOfSamples}$
    
    \State $r \gets \DERC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\Samples}{\vsigma}$
    \Comment{1-ERA of $\InducedGame{\ConditionDistribution}$}
    
    \State $\bm{\varepsilon}_{\PlayerIndex} (\StratProfile) \gets 2r + 3 \UtilityRange \sqrt{\nicefrac{\ln(\slfrac{1}{\delta})}{2\NumberOfSamples}}, \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
    \Comment{1-ERA bound}
    
%\State $\epsilon_1 \gets 2r + 3 \UtilityRange \sqrt{\nicefrac{\lnp{\slfrac{1}{\delta}}}{2\NumberOfSamples}}$ \Comment{ERA tail bound term}

%\State $\epsilon_2 \gets \UtilityRange\sqrt{\nicefrac{\lnp{\abs{\Gamma}}}{2\NumberOfSamples}} + \UtilityRange\sqrt{\nicefrac{\lnp{\slfrac{1}{\delta}}}{2\NumberOfSamples}}$ \Comment{RA tail bound with Massart's lemma}

%\State $\epsilon \gets \min(\epsilon_1, \epsilon_2)$
    
\ElsIf{\textsc{Bound} = \textsc{Hoeffding}}

    \State $\bm{\varepsilon}_{\PlayerIndex} (\StratProfile) \gets \UtilityRange \sqrt{\nicefrac{\lnp{\slfrac{2\abs{\UtilityIndices}}{\delta}}}{2\NumberOfSamples}}, \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$ \Comment{Hoeffding bound}
    
%\ElsIf{\textsc{Bound} = \textsc{Subgaussian}}

    %\State $\epsilon \gets \UtilityRange \sqrt{\nicefrac{\lnp{\slfrac{2\SizeOfGame(\GameTuple)}{\delta}}}{2\NumberOfSamples}}$ \Comment{Subgaussian Chernoff Bound}
    
\ElsIf{\textsc{Bound} = \textsc{Uniform Bennett}} \Comment{Uniform Empirical Bennett}

    \State 
    $\displaystyle\EVarWimpy \gets \sup_{\raisebox{0.5mm}{\ensuremath{\mathsmaller{(\PlayerIndex, \StratProfile) \in \UtilityIndices}}}} \mathsmaller{\frac{1}{\NumberOfSamples - 1}} \mathsmaller{\sum_{j = 1}^{\NumberOfSamples}} 
\left( \Utility_{\PlayerIndex}(\StratProfile; \SamplePoint_j) - \tilde{\Utility}_{\PlayerIndex} (\StratProfile) \right)^2$

    \State 
    $\epsilon_{v} \gets \frac{\UtilityRange^{2}\ln(\frac{3}{\delta})}{\NumberOfSamples - 1} + \sqrt{\Bigl(\frac{\UtilityRange^{2}\ln(\frac{3}{\delta})}{\NumberOfSamples - 1}\Bigr)^{\smash{2}} \! + \frac{2\UtilityRange^{2}\EVarWimpy\ln(\frac{3}{\delta})}{\NumberOfSamples - 1}}$
    
    \State
    $\bm{\varepsilon}_{\PlayerIndex} (\StratProfile) \gets \min\! \left( \, c\sqrt{\frac{\ln({\frac{3\abs{\UtilityIndices}}{\delta}})}{2\NumberOfSamples}}, \ \frac{\UtilityRange\ln(\frac{3\abs{\UtilityIndices}}{\delta})}{3\NumberOfSamples} + \sqrt{\frac{2(\EVarWimpy + \epsilon_{v})\ln({\frac{3\abs{\UtilityIndices}}{\delta}})}{\NumberOfSamples}} \, \right), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
    
    \ElsIf{\textsc{Bound} = \textsc{Non-uniform Bennett}} \Comment{Non-uniform Empirical Bennett}
    
    \For{$(\PlayerIndex, \StratProfile) \in \UtilityIndices$}
    
    \State 
    $\displaystyle\EVarWimpy \gets \mathsmaller{\frac{1}{\NumberOfSamples - 1}} \mathsmaller{\sum_{j = 1}^{\NumberOfSamples}} 
\left( \Utility_{\PlayerIndex}(\StratProfile; \SamplePoint_j) - \tilde{\Utility}_{\PlayerIndex} (\StratProfile) \right)^2$

    \State 
    $\epsilon_{v} \gets \frac{\UtilityRange^{2}\ln(\frac{3\abs{\UtilityIndices}}{\delta})}{\NumberOfSamples - 1} + \sqrt{\Bigl(\frac{\UtilityRange^{2}\ln(\frac{3\abs{\UtilityIndices}}{\delta})}{\NumberOfSamples - 1}\Bigr)^{\smash{2}} \! + \frac{2\UtilityRange^{2}\EVarWimpy\ln(\frac{3\abs{\UtilityIndices}}{\delta})}{\NumberOfSamples - 1}}$
    
    \State
    $\bm{\varepsilon}_{\PlayerIndex} (\StratProfile) \gets \min\! \left( \, c\sqrt{\frac{\ln({\frac{3\abs{\UtilityIndices}}{\delta}})}{2\NumberOfSamples}}, \ \frac{\UtilityRange\ln(\frac{3\abs{\UtilityIndices}}{\delta})}{3\NumberOfSamples} + \sqrt{\frac{2(\EVarWimpy + \epsilon_{v})\ln({\frac{3\abs{\UtilityIndices}}{\delta}})}{\NumberOfSamples}} \, \right), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
    
    \EndFor
    
\EndIf

% UNIFORM
%\State $\Return~(\tilde{\Utility}, \bm{\varepsilon})$

%\State $\UtilityIntervals_{\PlayerIndex} (\StratProfile) \gets [ \tilde{\Utility}_{\PlayerIndex} (\StratProfile) ] \pm [0, \bm{\varepsilon}_{\PlayerIndex} (\StratProfile)] \cap [-\nicefrac{\UtilityRange}{2}, \nicefrac{\UtilityRange}{2}], \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$

\State $\UtilityIntervals_{\PlayerIndex} (\StratProfile) \gets [ \tilde{\Utility}_{\PlayerIndex} (\StratProfile) - \bm{\varepsilon}_{\PlayerIndex} (\StratProfile), \tilde{\Utility}_{\PlayerIndex} (\StratProfile) + \bm{\varepsilon}_{\PlayerIndex} (\StratProfile)] \cap [-\nicefrac{\UtilityRange}{2}, \nicefrac{\UtilityRange}{2}], \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$

\State $\Return~\UtilityIntervals$

%\State $\Return~\UtilityIntervals_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$

%\State $\Return \, [ \tilde{\Utility}_{\PlayerIndex} (\StratProfile) - \bm{\varepsilon}_{\PlayerIndex} (\StratProfile), \tilde{\Utility}_{\PlayerIndex} (\StratProfile) + \bm{\varepsilon}_{\PlayerIndex} (\StratProfile)] \cap [-\nicefrac{\UtilityRange}{2}, \nicefrac{\UtilityRange}{2}], \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$ \Comment{Non-uniform Case}

\EndProcedure
\end{algorithmic}
\caption{Global Sampling}
\label{alg:gs}
\end{algorithm}

%\cyrus{Need to specify that $\SizeOfGame(\GameTuple)$ is the number of parameters we're estimating.}

==> algorithms/PSP_gen.tex <==
\begin{algorithm}[htbp]
\algrenewcommand\algorithmicindent{1.0em}
\begin{algorithmic}[1]
\Procedure{PSP}{$\ConditionalGame{\ConditionSpace}, \ConditionDistribution, \SamplingSchedule, \bm{\delta}, \UtilityRange, \textsc{Bound}, \Property, \lambda, \epsilon$} $\to (\hat{\Property}, \hat{\epsilon})$

\State \Input 
Conditional game $\ConditionalGame{\ConditionSpace}$, black box 
%$\BlackBox$ 
from which we can sample distribution $\ConditionDistribution$, sampling schedule $\SamplingSchedule$, failure probability schedule $\bm{\delta}$, utility range $\UtilityRange$, bound type \textsc{Bound}, equilibrium type \textsc{Pure}, error threshold $\epsilon$.

\State \Output 
%Empirical utilities $\tilde{\Utility}$, $\forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace$, utility error $\tilde{\bm{\epsilon}}$,
Empirical equilibria $\hat{\Nash}$, 
equilibria error $\hat{\epsilon}$, 
failure probability $\hat{\delta}$.
%such that with probability at least $1 - \hat{\delta}$, $\Nash(\GameTuple) \subseteq \Nash_{2\hat{\epsilon}}(\hat{\GameTuple}) \subseteq \Nash_{4\hat{\epsilon}}(\GameTuple)$

\State $\UtilityIndices \gets \SetOfPlayers \times \StratProfileSpace$ \Comment{Initialize utility indices} \label{alg:psp:init-UtilityIndices}

\State $\UtilityIntervals^0_{\PlayerIndex} (\StratProfile) \gets [-\nicefrac{\UtilityRange}{2}, \nicefrac{\UtilityRange}{2}], \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
%\amy{it seems that this initialization to $\nicefrac{c}{2}$ is immediately overwritten. i am not sure if the value $\nicefrac{c}{2}$ is important here?}
%\amy{answer: it is; it is the base case of the induction.}
\Comment{Initialize utility estimates} \label{alg:psp:init-outputs}

\State \Comment{Bipartite graphs: (property vertices, utility vertices)}

\State $D \gets (\StratProfileSpace, \UtilityIndices, \{ E(s) - U(p, s) \mid \forall p,s, \ s' \text{ adj to } s \})$ \Comment{Pure Welfare}

\State $D \gets (\StrategySet_{p}, \UtilityIndices, \{ E(s) - U(p, s') \mid \forall s \in \StrategySet_{p}, \ s' \text{ s.t. } s'_{p} = s \})$ \Comment{Safety Value of Action for Player $\PlayerIndex$}

\State $D \gets (\StratProfileSpace, \UtilityIndices, \{ E(s) - U(p, s') \mid \forall s, \ s' \text{ adj to (inclusive) } s \})$ \Comment{Pure Regret / Minimax}

\State Construct complete bipartite graph with vertices $\PropertyIndices = \Property$ and $\UtilityIndices$

\For{$\TimeIndex \in 1, \dots, \abs{\SamplingSchedule}$} %\Comment{Progressive sampling iterations}

    \State $\UtilityIntervals \gets \mathrm{\GS}(\ConditionalGame{\ConditionSpace}, \ConditionDistribution, \UtilityIndices, \SamplingSchedule_\TimeIndex, \bm{\delta}_\TimeIndex, \UtilityRange, \textsc{Bound})$ \label{alg:psp:interval-gs} \Comment{Improve utility estimates}

    \State $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile) \gets \smash{\UtilityIntervals_{\PlayerIndex} (\StratProfile) \cap \UtilityIntervals^{t-1}_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices}$ \label{alg:psp:interval_unpruned-gs} 
    
    \State $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile) \gets \smash{\UtilityIntervals^{t-1}_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace \setminus \UtilityIndices}$ \label{alg:psp:interval_pruned-gs} 
    
\if 0    
    \For{$(\PlayerIndex, \StratProfile) \in \UtilityIndices$}
    \amy{this for loop is an opt'n}
    
    \State $\Regret^{t \uparrow}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \max \left\{ \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile') \, \middle| \, \StratProfile' \in \MixedAdjacent_{\PlayerIndex, \StratProfile} \setminus \{ \StratProfile \} \right\} - \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile)$ \Comment{Can be negative}
    \label{alg:psp:regret_ub} 

    \State $\Regret^{t \downarrow}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \max \left\{ \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile') \, \middle| \, \StratProfile' \in \MixedAdjacent_{\PlayerIndex, \StratProfile} \setminus \{ \StratProfile \} \right\} - \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile)$ \Comment{Can be negative}
    \label{alg:psp:regret_lb} 

    \State $\Regret^{t}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \left[ \Regret^{t \downarrow}_{\PlayerIndex} (\StratProfile), \Regret^{t \uparrow}_{\PlayerIndex} (\StratProfile) \right] \cap [0, \UtilityRange]$

    \EndFor
    
    \State $\Regret^t_{\PlayerIndex} (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \Regret^{t-1}_{\PlayerIndex} (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile), \forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace \setminus \UtilityIndices$
\fi
   
    \State $\PropertyIntervals_j \gets \Property_j (\UtilityIntervals^{t})$, for all property vertices $j \in \PropertyIndices$
    \Comment{Improve property estimates}
    
    %\State $u^* \gets \min_{i} \bm{J}_{i}^{\uparrow}$ \Comment{Find minimum upper bound $u^*$ across property interval estimates}
    
    \State $\mathcal{J} \gets \mathcal{J} \setminus \{ j \in \mathcal{J} \mid \bm{J}_{j}^{\downarrow} > \min_{k} \bm{J}_{k}^{\uparrow} \}$
    \label{alg:psp:pruning_non-equilibria}
    \Comment{Prune provably suboptimal property indices in $\PropertyIndices$: i.e., those whose lower bound is larger than the minimum upper bound across all property interval estimates} \amy{pruning vertices automatically prunes incident edges}

    \State $\UtilityIndices \gets \UtilityIndices \setminus \smash{\{ (\PlayerIndex, \StratProfile) \in \UtilityIndices \mid \text{length of interval } \UtilityIntervals^t_{\PlayerIndex} (\StratProfile) \leq \nicefrac{\epsilon}{\lambda} \}}$
    \label{alg:psp:pruning_well-estimated}
    \Comment{Prune well-estimated utility indices}
    
    \State %\cyrus{Edge pruning:} 
    %Prune $E(j, i)$ from property index $j$ to utility index $i$ if: $\forall \bm{u} \in U (\UtilityIntervals^{\TimeIndex})$, choose $\bm{u}' \in U (\UtilityIntervals^{\TimeIndex})$ that agrees with $\bm{u}$ except at index $i$ (i.e., $\Utility_{p} (\StratProfile) = \Utility'_{p} (\StratProfile)$ except at $(p, \StratProfile) = i$), we have $\abs{ \Property(j, \bm{u}) - \Property(j, \bm{u}')} = 0$
    $\displaystyle \mathcal{E} \gets \mathcal{E} \setminus \{ (j, i) \in \mathcal{E} : \sup_{\Utility, \Utility' \in \UtilitySet(\UtilityIntervals^{\TimeIndex}) \text{ s.t. }  \forall (\PlayerIndex, \StratProfile) \neq i: \Utility_{\PlayerIndex}(\StratProfile) = \Utility'_{\PlayerIndex}(\StratProfile)} \abs{ \Property_{j} (\Utility) - \Property_{j} (\Utility')} = 0 \}$
    \Comment{Prune an edge $(j,i)$ whenever utility index $i$ has no impact on property $\Property_{j}$}
    \amy{notion of game adjacency; games differ only at index $i = (\PlayerIndex, \StratProfile)$}

    \State Prune all vertices with degree 0
    \Comment{Garbage collection}
    
    \If{$\UtilityIndices = \emptyset$
    %$\hat{\epsilon} \leq \epsilon$
    or $\TimeIndex = \abs{\SamplingSchedule}$}
    \label{alg:psp:termination}
    \Comment{Termination condition}
    
    \if 0
        \For{$(\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace$}
    
        \If{$\Regret^{t \downarrow}_\PlayerIndex (\UtilityIntervals^t_{\PlayerIndex}, \StratProfile) \le 0$}
            \State $\tilde{\Utility}_{\PlayerIndex} (\StratProfile) \gets \nicefrac{1}{2} \left( \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile) + \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile) \right)$
        \Else
            \State $\tilde{\Utility}_{\PlayerIndex} (\StratProfile) \gets -\infty$
        \EndIf
        
        \EndFor
    \fi
        
        \State $\hat{\epsilon}$ is the maximum length of any property interval estimate $\PropertyIntervals_j$ among $j \in \PropertyIndices$
        
        \amy{meaning of being in $\PropertyIndices$: might minimize the property: e.g., have the smallest regret}
        
        \amy{$\hat{\epsilon} \gets$ maximum uncertainty among minimal (i.e., good/still alive) property estimates}
          
    \if 0
    %e.g., welfare
        \State optimal welfare can be as low as the lowest lower bound, and as high as the highest upper bound
    \fi
        
    \if 0
    % REGRET, specifically
        \State $\hat{\epsilon} \gets \smash{\max \left\{ \Regret^{\uparrow} (\UtilityIntervals, \StratProfile) \bigm| \StratProfile \in \StratProfileSpace \textrm{ s.t.}\, \Regret^{\downarrow} (\UtilityIntervals, \StratProfile) = 0 \right\}}$
        \label{alg:psp:epsilon-hat}
    \fi

    \if 0
        \If{$\UtilityIndices = \emptyset$} \label{alg:psp:eps-hat}
            \State$\hat{\epsilon} \gets \epsilon$
        \Else
            \State $\hat{\epsilon} \gets \sup_{(\PlayerIndex, \StratProfile) \in \UtilityIndices}$ length of interval $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile)$
            %equivalently, $\Regret^{t \uparrow}_\PlayerIndex (\UtilityIntervals^t_{\PlayerIndex}, \StratProfile)$
        \EndIf
    \fi

        %\State $\hat{\Nash} \gets \Nash (\UtilityIntervals)$
        %\Comment{Compute equilibria}

        %\State $\hat{\Nash} \gets \left\{ \begin{array}{rcl} \textsc{Pure} & : & \Nash_{\hat{\epsilon}}(\tilde{\Utility}) \\ \neg\textsc{Pure} & : & \Nash^{\diamond}_{\hat{\epsilon}}(\tilde{\Utility}) \\ \end{array} \right.$
        %\Comment{Compute equilibria}

        %TODO could take grand averages
    	\State $\Return~\smash{\left( \hat{\Nash} := \Nash (\UtilityIntervals), \hat{\epsilon} \right)}$
    	\label{alg:psp:return}
    	
    	\State return 
    	%$\PropertyIntervals$ (the property estimates) and
    	$\PropertyIndices$ \amy{and $\UtilityIntervals^{\TimeIndex}$}
    \EndIf

\EndFor

%\State \Error ``\textsc{Insufficient samples to produce $\epsilon$-$\delta$ guarantee}''

\label{alg:psp}
\EndProcedure
\end{algorithmic}

%\cyrus{Do we want to take an initial index set $\UtilityIndices_0$?  How does this effect the guarantees we can get?}

%\amy{NOT TODAY!!! but we can discuss further next week. i agree it's a little weird/asymmetric at present, as \GS{} takes UtilityIndices and \PSP{} does not, but initializes them immediately.}

\caption{Generic Progressive Sampling with Pruning}
\label{alg:psp_eqa}
\end{algorithm}

==> algorithms/PSP_generic.tex <==
\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\Procedure{PSP}{$\GameTuple, \ConditionDistribution, \bm{M}, \epsilon, \bm{\delta}, A, B, \UtilityRange$, \textsc{Bound}} $\to (\hat{Y}, \hat{\epsilon}, \hat{\delta})$
 
\State \Input Conditional game $\GameTuple$, distribution $\ConditionDistribution$, sampling schedule $\bm{M}$, error tolerance $\epsilon$, failure probability schedule $\bm{\delta}$, pruning function $A$, estimation function $B$, range $\UtilityRange$, bound type \textsc{Bound}.

\State \Output Empirical estimate $\hat{Y}$, additive error $\hat{\epsilon}$, and failure probability $\hat{\delta}$. 
%such that with probability at least $1 - \tilde{\delta}$, $\Nash(\GameTuple) \subseteq \Nash_{2\epsilon}(\tilde{\GameTuple}) \subseteq \Nash_{4\epsilon}(\GameTuple)$

\State $\UtilityIndices_0 \gets \SetOfPlayers \times \StratProfileSpace$ \Comment{Initial index set} 
%(the unrestricted game)

%\State $\hat{\GameTuple}_0 \gets \GameTuple$ \Comment{Begin with the unrestricted game.}

%\State $\tilde{\StratProfileSpace}_0 \gets \strategies(\GameTuple)$ 
%\Comment{Initialize game with all strategies in $\GameTuple$}

%\State $S_{\TimeIndex=0:n} \gets \min((2^{\TimeIndex} - 1)s_1, \NumberOfSamples)$
%\Comment{Sampling schedule}

%\State $m_{\TimeIndex=1:n} \gets S_\TimeIndex - S_{\TimeIndex - 1}$
%\Comment{Size of each sample}

\For{$\TimeIndex \in 1, \dots, \abs{\bm{M}}$} \Comment{Progressive sampling iterations}
    \State $(\hat{\Utility}_{\TimeIndex}, \epsilon_\TimeIndex)
    			\gets \textsc{GS}(\GameTuple,  \ConditionDistribution, 
    			\UtilityIndices_{\TimeIndex - 1},
    			\bm{M}_\TimeIndex, 
    			\bm{\delta}_\TimeIndex,
    			\UtilityRange,
    			\textsc{Bound})$ \Comment{Unpruned empirical utilities} \label{alg:psp:gs}
    			
    \State $\hat{\Utility}_{\TimeIndex, \PlayerIndex} (\StratProfile) \gets \hat{\Utility}_{\TimeIndex - 1, \PlayerIndex} (\StratProfile), \ \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices_0 \setminus \UtilityIndices_{\TimeIndex - 1}$ \Comment{Propagate pruned utilities}
    
    \State \amy{Cyrus, i'm not seeing where $\tilde{\GameTuple}_\TimeIndex$ gets updated} \cyrus{This is a mistake.  $\tilde{\GameTuple}_\TimeIndex$ should use $\tilde{\Utility}_\TimeIndex$, but I think it's more stylistically consistent to modify $A$ and $B$ to take a utility function instead of a game.} \amy{well, i wouldn't call it a mistake, but yes, we have a notation problem.}
    
    \State $\UtilityIndices_{\TimeIndex} \gets A(\tilde{\GameTuple}_\TimeIndex, \epsilon_\TimeIndex)$ \Comment{Prune irrelevant parameters} \label{alg:psp:pruning}
    
    \State $(\hat{Y}_\TimeIndex, \epsilon'_\TimeIndex) \gets B(\tilde{\GameTuple}_\TimeIndex, \epsilon_\TimeIndex)$ \Comment{Run estimation procedure} \label{alg:psp:estimation}
    
    \If{$\epsilon'_\TimeIndex \leq \epsilon$ or $t = \abs{\bm{M}}$}
        \State $\Return (\hat{Y}_\TimeIndex, \epsilon'_\TimeIndex, \sum_{i=1}^\TimeIndex \bm{\delta}_i)$
    \EndIf
\EndFor

%\State \Error ``\textsc{Insufficient samples to produce $\epsilon$-$\delta$ guarantee}''

\EndProcedure
\end{algorithmic}
\if 0 %Before parameterizing the goal:
\begin{algorithmic}[1]
\Procedure{PSP}{$\GameTuple, \ConditionDistribution, \bm{M}, \epsilon, \bm{\delta}, A, B, \UtilityRange$, \textsc{Bound}} $\to (\tilde{\GameTuple}, \epsilon, \tilde{\delta})$
 
\State \Input Conditional game $\GameTuple$, distribution $\ConditionDistribution$, sampling schedule $\bm{M}$, error tolerance $\epsilon$, failure probability schedule $\bm{\delta}$, range of values $\UtilityRange$, bound type \textsc{Bound}.

\State \Output Empirical game $\tilde{\GameTuple}$, error $\epsilon$, failure probability $\tilde{\delta}$. 
%such that with probability at least $1 - \tilde{\delta}$, $\Nash(\GameTuple) \subseteq \Nash_{2\epsilon}(\tilde{\GameTuple}) \subseteq \Nash_{4\epsilon}(\GameTuple)$

\State $\tilde{\GameTuple}_0 \gets \GameTuple$

\State $\tilde{\StratProfileSpace}_0 \gets \strategies(\GameTuple)$ 
%\Comment{Initialize game with all strategies in $\GameTuple$}

%\State $S_{\TimeIndex=0:n} \gets \min((2^{\TimeIndex} - 1)s_1, \NumberOfSamples)$
%\Comment{Sampling schedule}

%\State $m_{\TimeIndex=1:n} \gets S_\TimeIndex - S_{\TimeIndex - 1}$
%\Comment{Size of each sample}

\For{$\TimeIndex \in 1, \dots, \abs{\bm{M}}$} \Comment{Progressive sampling iterations}
   
    \State $(\tilde{\GameTuple}_\TimeIndex, \epsilon_\TimeIndex)
    			\gets \textsc{GS}(\restrict(\tilde{\GameTuple}_{\TimeIndex-1}, \tilde{\StratProfileSpace}_{\TimeIndex-1}), \ConditionDistribution, \bm{M}_\TimeIndex, \bm{\delta}_\TimeIndex,
    			\UtilityRange,
    			\textsc{Bound})$
    			
    \If{$\epsilon_\TimeIndex \le \epsilon$ or $\TimeIndex = \abs{\bm{M}}$}
    	\State $\Return~(\tilde{\GameTuple}_\TimeIndex, \epsilon_\TimeIndex, \sum_{i=1}^\TimeIndex \bm{\delta}_i)$
    \EndIf

    \State $\tilde{\StratProfileSpace}_{\TimeIndex} \gets \CKR_{2\epsilon_\TimeIndex}(\tilde{\GameTuple}_\TimeIndex)$ 
    \label{step:rat}
    \Comment{Prune dominated strategies}
\EndFor

%\State \Error ``\textsc{Insufficient samples to produce $\epsilon$-$\delta$ guarantee}''

\EndProcedure
\end{algorithmic}
\fi
\caption{Progressive Sampling with Pruning}
\label{alg:psp_gen}
\end{algorithm}

==> algorithms/PSP_soft.tex <==
\begin{algorithm}[htbp]
\algrenewcommand\algorithmicindent{1.0em}
\begin{algorithmic}[1]
\Procedure{PSP}{$\ConditionalGame{\ConditionSpace}, \ConditionDistribution, \SamplingSchedule, \bm{\delta}, \UtilityRange, \textsc{Bound}, \Property, \lambda, \epsilon$} $\to (\hat{\Property}, \hat{\epsilon})$

\State \Input 
Conditional game $\ConditionalGame{\ConditionSpace}$, black box 
%$\BlackBox$ 
from which we can sample distribution $\ConditionDistribution$, sampling schedule $\SamplingSchedule$, failure probability schedule $\bm{\delta}$, utility range $\UtilityRange$, bound type \textsc{Bound}, equilibrium type \textsc{Pure}, error threshold $\epsilon$.

\State \Output 
%Empirical utilities $\tilde{\Utility}$, $\forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace$, utility error $\tilde{\bm{\epsilon}}$,
Empirical equilibria $\hat{\Nash}$, 
equilibria error $\hat{\epsilon}$, 
failure probability $\hat{\delta}$.
%such that with probability at least $1 - \hat{\delta}$, $\Nash(\GameTuple) \subseteq \Nash_{2\hat{\epsilon}}(\hat{\GameTuple}) \subseteq \Nash_{4\hat{\epsilon}}(\GameTuple)$

\State $\UtilityIndices \gets \SetOfPlayers \times \StratProfileSpace$ \Comment{Initialize utility indices} \label{alg:psp:init-UtilityIndices}

\State $\UtilityIntervals^0_{\PlayerIndex} (\StratProfile) \gets [-\nicefrac{\UtilityRange}{2}, \nicefrac{\UtilityRange}{2}], \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices$
%\amy{it seems that this initialization to $\nicefrac{c}{2}$ is immediately overwritten. i am not sure if the value $\nicefrac{c}{2}$ is important here?}
%\amy{answer: it is; it is the base case of the induction.}
\Comment{Initialize utility estimates} \label{alg:psp:init-outputs}

\State \Comment{Bipartite graphs: (property vertices, utility vertices)}

\State $\PropertyIndices \gets \{ 1, \ldots, \abs{\Property} \}$

\State $\UtilityIndices \gets \SetOfPlayers \times \StratProfileSpace$

\State $E \gets \{ (j, i, \lambda_j (\Property_j, i, \UtilityIntervals^0)) \mid j \in \PropertyIndices, i \in \UtilityIndices \}$

\amy{complete graph!!! with edge weights as local Lipschitz constants: for each property $M_j$ wrt $(p,\bm{s})$ in the subdomain $\UtilitySet (\UtilityIntervals)$: i.e., how much changing $(p,\bm{s})$ can affect $M_j$}

\[
\lambda_j (\Property_j, (\PlayerIndex, \StratProfile), \UtilityIntervals) \gets \sup_{\Utility \in \UtilitySet (\UtilityIntervals)} \abs{\frac{\partial \Property_j (\Utility)}{\partial \Utility_{\PlayerIndex} (\StratProfile)}}
\]

\amy{is this specific to the infinity norm?}
\cyrus{Maybe actually 1 norm}

\State $\lambda (\PropertyIndices, (\PlayerIndex, \StratProfile), \UtilityIntervals) \gets \max_{j \in \PropertyIndices} \lambda_j (\Property_j, (\PlayerIndex, \StratProfile), \UtilityIntervals))$

\For{$\TimeIndex \in 1, \dots, \abs{\SamplingSchedule}$} %\Comment{Progressive sampling iterations}

    \State $\UtilityIntervals \gets \mathrm{\GS}(\ConditionalGame{\ConditionSpace}, \ConditionDistribution, \UtilityIndices, \SamplingSchedule_\TimeIndex, \bm{\delta}_\TimeIndex, \UtilityRange, \textsc{Bound})$ \label{alg:psp:interval-gs} \Comment{Improve utility estimates}

    \State $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile) \gets \smash{\UtilityIntervals_{\PlayerIndex} (\StratProfile) \cap \UtilityIntervals^{t-1}_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \UtilityIndices}$ \label{alg:psp:interval_unpruned-gs} 
    
    \State $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile) \gets \smash{\UtilityIntervals^{t-1}_{\PlayerIndex} (\StratProfile), \forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace \setminus \UtilityIndices}$ \label{alg:psp:interval_pruned-gs} 
    
\if 0    
    \For{$(\PlayerIndex, \StratProfile) \in \UtilityIndices$}
    \amy{this for loop is an opt'n}
    
    \State $\Regret^{t \uparrow}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \max \left\{ \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile') \, \middle| \, \StratProfile' \in \MixedAdjacent_{\PlayerIndex, \StratProfile} \setminus \{ \StratProfile \} \right\} - \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile)$ \Comment{Can be negative}
    \label{alg:psp:regret_ub} 

    \State $\Regret^{t \downarrow}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \max \left\{ \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile') \, \middle| \, \StratProfile' \in \MixedAdjacent_{\PlayerIndex, \StratProfile} \setminus \{ \StratProfile \} \right\} - \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile)$ \Comment{Can be negative}
    \label{alg:psp:regret_lb} 

    \State $\Regret^{t}_\PlayerIndex (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \left[ \Regret^{t \downarrow}_{\PlayerIndex} (\StratProfile), \Regret^{t \uparrow}_{\PlayerIndex} (\StratProfile) \right] \cap [0, \UtilityRange]$

    \EndFor
    
    \State $\Regret^t_{\PlayerIndex} (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile) \gets \Regret^{t-1}_{\PlayerIndex} (\UtilityIntervals^{t}_{\PlayerIndex}, \StratProfile), \forall (\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace \setminus \UtilityIndices$
\fi
   
    \State $\PropertyIntervals_j \gets \Property_j (\UtilityIntervals^{t})$, for all property vertices $j \in \PropertyIndices$
    \Comment{Improve property estimates}
    
    %\State $u^* \gets \min_{i} \bm{J}_{i}^{\uparrow}$ \Comment{Find minimum upper bound $u^*$ across property interval estimates}
    
    \State $\mathcal{J} \gets \mathcal{J} \setminus \{ j \in \mathcal{J} \mid \bm{J}_{j}^{\downarrow} > \min_{k} \bm{J}_{k}^{\uparrow} \}$
    \label{alg:psp:pruning_non-equilibria}
    \Comment{Prune provably suboptimal property indices in $\PropertyIndices$: i.e., those whose lower bound is larger than the minimum upper bound across all property interval estimates}

    \State $\UtilityIndices \gets \UtilityIndices \setminus \smash{\{ (\PlayerIndex, \StratProfile) \in \UtilityIndices \mid \text{length of interval } \UtilityIntervals^{t}_{\PlayerIndex} (\StratProfile) \cdot \lambda (\PropertyIndices, (\PlayerIndex, \StratProfile), \UtilityIntervals^{t}) \leq \epsilon \}}$
    \label{alg:psp:pruning_well-estimated}
    \Comment{Prune well-estimated utility indices}

    %\State $\UtilityIndices \gets \{ (\PlayerIndex, \StratProfile) \in \UtilityIndices \mid \Regret^{t \uparrow}_\PlayerIndex (\UtilityIntervals^t_{\PlayerIndex}, \StratProfile) \ge \epsilon \}$ 
    %\label{alg:psp:pruning_well-estimated}
    %\Comment{Prune well-estimated}

    \If{$\UtilityIndices = \emptyset$
    %$\hat{\epsilon} \leq \epsilon$
    or $\TimeIndex = \abs{\SamplingSchedule}$}
    \label{alg:psp:termination}
    \Comment{Termination condition}
    
    \if 0
        \For{$(\PlayerIndex, \StratProfile) \in \SetOfPlayers \times \StratProfileSpace$}
    
        \If{$\Regret^{t \downarrow}_\PlayerIndex (\UtilityIntervals^t_{\PlayerIndex}, \StratProfile) \le 0$}
            \State $\tilde{\Utility}_{\PlayerIndex} (\StratProfile) \gets \nicefrac{1}{2} \left( \UtilityIntervals^{t \uparrow}_{\PlayerIndex} (\StratProfile) + \UtilityIntervals^{t \downarrow}_{\PlayerIndex} (\StratProfile) \right)$
        \Else
            \State $\tilde{\Utility}_{\PlayerIndex} (\StratProfile) \gets -\infty$
        \EndIf
        
        \EndFor
    \fi
        
        \State $\hat{\epsilon}$ is the maximum length of any property interval estimate $\PropertyIntervals_j$ among $j \in \PropertyIndices$
        
        \amy{meaning of being in $\PropertyIndices$: might minimize the property: e.g., have the smallest regret}
        
        \amy{$\hat{\epsilon} \gets$ maximum uncertainty among minimal (i.e., good/still alive) property estimates}
        
    \if 0
    %e.g., welfare
        \State optimal welfare can be as low as the lowest lower bound, and as high as the highest upper bound
    \fi
        
    \if 0
    % REGRET, specifically
        \State $\hat{\epsilon} \gets \smash{\max \left\{ \Regret^{\uparrow} (\UtilityIntervals, \StratProfile) \bigm| \StratProfile \in \StratProfileSpace \textrm{ s.t.}\, \Regret^{\downarrow} (\UtilityIntervals, \StratProfile) = 0 \right\}}$
        \label{alg:psp:epsilon-hat}
    \fi
        
    \if 0
        \If{$\UtilityIndices = \emptyset$} \label{alg:psp:eps-hat}
            \State$\hat{\epsilon} \gets \epsilon$
        \Else
            \State $\hat{\epsilon} \gets \sup_{(\PlayerIndex, \StratProfile) \in \UtilityIndices}$ length of interval $\UtilityIntervals^t_{\PlayerIndex} (\StratProfile)$
            %equivalently, $\Regret^{t \uparrow}_\PlayerIndex (\UtilityIntervals^t_{\PlayerIndex}, \StratProfile)$
        \EndIf
    \fi

        %\State $\hat{\Nash} \gets \Nash (\UtilityIntervals)$
        %\Comment{Compute equilibria}

        %\State $\hat{\Nash} \gets \left\{ \begin{array}{rcl} \textsc{Pure} & : & \Nash_{\hat{\epsilon}}(\tilde{\Utility}) \\ \neg\textsc{Pure} & : & \Nash^{\diamond}_{\hat{\epsilon}}(\tilde{\Utility}) \\ \end{array} \right.$
        %\Comment{Compute equilibria}

        %TODO could take grand averages
    	\State $\Return~\smash{\left( \hat{\Nash} := \Nash (\UtilityIntervals), \hat{\epsilon} \right)}$
    	\label{alg:psp:return}
    	
    	\State return 
    	%$\PropertyIntervals$ (the property estimates) and
    	$\PropertyIndices$ \amy{and $\UtilityIntervals^{\TimeIndex}$}
    \EndIf

\EndFor

%\State \Error ``\textsc{Insufficient samples to produce $\epsilon$-$\delta$ guarantee}''

\label{alg:psp}
\EndProcedure
\end{algorithmic}

%\cyrus{Do we want to take an initial index set $\UtilityIndices_0$?  How does this effect the guarantees we can get?}

%\amy{NOT TODAY!!! but we can discuss further next week. i agree it's a little weird/asymmetric at present, as \GS{} takes UtilityIndices and \PSP{} does not, but initializes them immediately.}

\caption{SOFT Progressive Sampling with Pruning}
\label{alg:psp_eqa}
\end{algorithm}

==> algorithms/alg_psp_generic.tex <==
\subsection{Progressive Sampling with Pruning}
\label{subsec:PSP}

Next, we present \PSP{} (\Cref{alg:psp_gen}),
which draws progressively larger samples, refining the empirical game at each iteration, and stopping when it can approximate the property of interest to the desired accuracy, or when its sampling budget is exhausted.
Although not guaranteed, PSP can potentially learn using vastly fewer resources than global sampling.

%\PSP{} operates over multiple iterations.
%In each, it draws a progressively larger sample, with which it improves its utility estimates, with which it then refines its property estimate $\hat{Y}$, repeating this process until the accuracy guarantee is achieved, or the sampling budget is exhausted.

\amy{where does this sentence go!!??}
Failure probabilities are combined via a union bound, so the failure probability of the result is the sum of the failure probabilities at each iteration.

Like \GS, \PSP{} takes in a conditional game $\GameTuple$, a distribution $\ConditionDistribution$, a utility magnitude $\UtilityRange$, and a bound type {\sc Bound}.  
Instead of a single sample size, however, it takes in a \emph{sampling schedule} $\bm{M}$, which is a non-decreasing sequence of integers; and instead of a single failure probability, it takes in a \emph{failure probability schedule} $\bm{\delta}$, with each $\bm{\delta}_i$ in this sequence, and its sum $\in (0, 1)$.
These two schedules dictate the number of samples to draw and the failure probability to use at each iteration.
Finally, \PSP{} also takes in pruning and estimation functions $A$ and $B$ (discussed below), as well as an \emph{approximation threshold} $\epsilon$, which determines the termination condition.

%In its most basic form, the goal is, for some (fixed) $\epsilon$ and $\delta$, to simulate $\InducedGame{\ConditionDistribution}$ only as many times as necessary to guarantee that with probability at least $1 - \delta$, the estimated game $\hat{\GameTuple}$ satisfies $\norm{\InducedGame{\ConditionDistribution} - \hat{\GameTuple}}_\infty \leq \epsilon$.  Often we are only interested in learning a game to estimate some property of the game (such as its equilibria, or minimax-optimal strategies), and in these cases, \PSP{} takes additional hyperparameters which allow it to avoid estimating parameters of $\hat{\Utility}$ more accurately than required for the task at hand, saving computational and statistical resources.  \PSP{} terminates, providing a $\hat{\epsilon}$-$\hat{\delta}$ estimate of the desired quantity, which when appropriately parameterized, are always superior to the requested $\epsilon$-$\delta$ guarantee.  %A run of \PSP{} either terminates in failure, or by providing an $\epsilon$-$\delta$ estimate of the quantity of interest that is at least as required by $\epsilon$ and $\delta$.

%Algorithm~\ref{alg:psp} iteratively calls Algorithm~\ref{alg:globalSample} with sample sizes according to $P$, and after each iteration, it removes strategies that it can guarantee with probability at least $1 - \delta$ (jointly) are dominated in $\InducedGame{\ConditionDistribution}$.  Algorithm~\ref{alg:psp} continues this process until the sampling schedule is exhausted, at which point it returns an $\epsilon$-$\delta$ guarantee with $\epsilon$ greater than requested, or a sufficiently good approximation of $\InducedGame{\ConditionDistribution}$ has been learned, in which case both $\epsilon$ and $\delta$ may be smaller than requested.  We now formalize the guarantees of this algorithm.

\cyrus{The idea is that, e.g., we know playing this action in this SP is definitely worse than all the other actions, so it's never part of an equilibrium, so there's no point in improving our estimate, because it still won't be an equilibrium}

\PSP{} depends on the property of interest $Y$ through a \emph{pruning function} $A(\hat{\GameTuple}, \hat{\epsilon})$ and an \emph{estimation function} $B(\hat{\GameTuple}, \hat{\epsilon})$, each of which depend on an estimate $\hat{\GameTuple}$ with a corresponding quality guarantee $\hat{\epsilon}$.  
Informally, $A$ produces an index set $\UtilityUtilityIndices \subseteq \SetOfPlayers \times \StratProfileSpace$, such that $\hat{\GameTuple}$ already estimates all UtilityUtilityIndices 
%in $\SetOfPlayers \times \StratProfileSpace \setminus \UtilityUtilityIndices$
\emph{not\/} in $\UtilityUtilityIndices$ sufficiently well so as to provably not impact the estimation of $\hat{Y}$.
Informally, $B$ produces an estimate $\hat{Y}$ of $Y$ and approximation threshold $\hat{\epsilon}$, such that 
%for some $\norm{\cdot}_{\mathcal{Y}}$,
$\norm{Y - \hat{Y}}_{\mathcal{Y}} \leq \hat{\epsilon}$.
%
$B$ is necessary to provide approximation guarantees for arbitrary properties of games.
$A$ is not necessary, but allows the \PSP{} algorithm to prune the search space, conserving computational and statistical resources.  

For example, if the task is to estimate the optimal utilitarian welfare, then we may take $B(\hat{\GameTuple}, \epsilon) = \left( \sup_{\StratProfile \in \StratProfileSpace} \Welfare (\hat{\Utility}, \StratProfile), \NumberOfPlayers \epsilon \right)$, and the pruning criterion $A$ can prune all strategy profiles that are $2\NumberOfPlayers\epsilon$-suboptimal in $\hat{\GameTuple}$, as by Theorem~\ref{thm:lipschitz-properties}(\ref{thm:lipschitz-properties:welfare}), any strategy profile outside this set can not possibly maximize welfare, and hence cannot impact the optimal utilitarian welfare. 
%
Similarly, to estimate a maximin-optimal strategy, $B$ can produce the maximin-optimal strategy over $\hat{\GameTuple}$ and an error guarantee, and $A$ can prune strategies that are provably maximin-suboptimal.
%
With this intuition and these examples in mind, we now rigorously define these concepts.

\begin{definition}[Pruning and Estimation Functions]
\label{def:pruning-estimation}
Suppose games $\GameTuple$ and $\hat{\GameTuple}$, and $\hat{\epsilon} \geq 0$.  Suppose also \mydef{pruning function} $A$ and \mydef{estimation function} $B$ taking $\hat{\GameTuple}$ and $\hat{\epsilon}$, with $A$ producing some $\UtilityUtilityIndices \subseteq \SetOfPlayers \times \StratProfileSpace$ and $B$ producing some $(\hat{Y},\hat{\epsilon}) \in \mathcal{Y} \times \R$ pair, letting $B_1$ and $B_2$ be selection operators that return the first and second outputs of $B$, respectively.  
%Take $B_1$ to be the %$A$ and $B$ are said to be a \mydef{pruning function} and an \mydef{estimation function} for some parameter $Y \in \mathcal{Y}$ where $Y \doteq B_1(\GameTuple, 0)$ if they satisfy 
We require that $A$ and $B$ obey the following properties for all $\hat{\GameTuple}_1$, $\hat{\GameTuple}_2$, $\hat{\epsilon}_1 \leq \hat{\epsilon}_2$, such that $\norm{\GameTuple - \hat{\GameTuple}_1}_\infty \leq \hat{\epsilon}_1$ and $\norm{\GameTuple - \hat{\GameTuple}_2}_\infty \leq \hat{\epsilon}_2$, and for all $\hat{\GameTuple}_3$ with utilities equal to those of $\hat{\GameTuple}_1$ at all UtilityUtilityIndices in $A(\hat{\GameTuple}_1, \hat{\epsilon}_1)$ and to those of $\hat{\GameTuple}_2$ at the remaining UtilityUtilityIndices:
%
\begin{enumerate}

\item \mydef{Pruning Monotonicity}: $A(\hat{\GameTuple}_1, \hat{\epsilon}_1) \subseteq A(\hat{\GameTuple}_2, \hat{\epsilon}_2)$

\item \mydef{Pruning Equivalence} $B(\hat{\GameTuple}_1, \hat{\epsilon}_1) = B(\hat{\GameTuple}_3, \hat{\epsilon}_1)$

\item \mydef{Estimation Approximation} $\smash{\norm{Y - B_1(\hat{\GameTuple}_1, \hat{\epsilon}_1)}_{\mathcal{Y}} \leq B_2(\hat{\GameTuple}_1, \hat{\epsilon}_1)}$ and $B_2(\GameTuple, 0) = 0$

\item \mydef{Estimation Monotonicity} If $\mathcal{B}_\infty(\hat{\GameTuple}_1, \hat{\epsilon}_1) \subseteq \mathcal{B}_\infty(\hat{\GameTuple}_2, \hat{\epsilon}_2)$, then $B_2(\hat{\GameTuple}_1, \hat{\epsilon}_1) \leq B_2(\hat{\GameTuple}_2, \hat{\epsilon}_2)$, where $\mathcal{B}_\infty(x, y)$ is the radius $y$ $\ell_\infty$ ball about $x$
%\item \mydef{Estimation Convergence} $B_2(\GameTuple, 0) = 0$
%\item \mydef{Pruning Independence}: If $\norm{\GameTuple - \hat{\GameTuple}'_1}_\infty \leq \hat{\epsilon}_1$, and $\forall (\PlayerIndex, \StratProfile) \in A(\hat{\GameTuple}')$, then $B(\hat{\GameTuple}_1, \hat{\epsilon}_1) = B(\hat{\GameTuple}'_1, \hat{\epsilon}_1)$
%\item \mydef{Estimation Monotonicity}: If $\norm{\GameTuple - \hat{\GameTuple}_1}_\infty \leq \hat{\epsilon}_1  \hat{\GameTuple_1} $%B(\hat{\GameTuple}_1, \hat{\epsilon}_1) \subseteq B(\hat{\GameTuple}_2, \hat{\epsilon}_2)$
%\item \mydef{Pruning Independence}: 

\end{enumerate}
\end{definition}

%Old informal definition:
%of \emph{UtilityUtilityIndices}, which are (player index, strategy profile) pairs $\UtilityUtilityIndices \subseteq \SetOfPlayers \times \StratProfileSpace$ such that for any $\hat{\GameTuple}'$ such that $\norm{\hat{\GameTuple} - \hat{\GameTuple}'}_\infty \leq \hat{\epsilon}$ with utility function identical for each (player index, strategy profile) combination in $\UtilityUtilityIndices$, it holds that $B_1(\hat{\GameTuple}, \cdot) = B_1(\hat{\GameTuple}', \cdot)$.  The estimation procedure $B(\cdot, \cdot)$ then takes the approximate game, and from it estimates some property of the game, returning this estimate $\hat{Y}$ and an approximation quality bound $\hat{\epsilon}'$ such that for some norm $\norm{\cdot}_B$, $\norm{\hat{Y} - B_1(\GameTuple_{\ConditionDistribution}, 0)}_B \leq \hat{\epsilon}'$.  We require also that $A(\cdot, \cdot)$ decreases monotonically in its second argument, $B_1(\GameTuple, \cdot)$ is either independent (for numeric quantities) of its second argument, or obeys $B_1(\GameTuple, \epsilon_1) \subseteq B_1(\GameTuple, \epsilon_2)$ for $\epsilon_1 \leq \epsilon_2$ (for set estimates), and $B_2(\cdot, 0) = 0$.  Intuitively, we require these properties, as through $A$ we can determine which values of the utility function have already been estimated sufficiently so as to have provably no impact on the estimation of the desideratum.

%the degenerate pruning function $A(\hat{\GameTuple}, \epsilon) = \SetOfPlayers \times \StratProfileSpace$ always exhibits pruning monotonicity

While perhaps somewhat opaque, these properties are not difficult to show for many pruning and estimation functions for many quantities of interest.  Note that for any quantity we wish to estimate, given an estimator for that quantity, we can construct an estimation function (though this requires some analysis in obtaining the estimation quality guarantee), and with the estimation function, we can construct a pruning function that satisfies the required properties.  \cyrus{Intuitive explanation of properties here:} Briefly put, \emph{pruning monotonicity} ensures that as the estimate of the game improves, the set of UtilityUtilityIndices the pruning function indicates must be explored decreases monotonically, \emph{pruning equivalence} ensures that each index that improving the estimates at any index that is pruned has no effect on the estimate, \emph{estimation approximation} ensures that the approximation quality guarantee given by $B$ holds, and that the property is estimated with perfect accuracy when the game is known with perfect accuracy, and finally \emph{estimation monotonicity} ensures that the estimation quality guarantee improves monotonically as the utility estimates improve.  The whole framework is rather mechanical, but we nonetheless discuss each of the Lipschitz properties of Theorem~\ref{thm:lipschitz-properties} to illustrate the point.  

To estimate a perfect-recall approximate-precision set of utilitarian-welfare-maximal strategy profiles, we take $\mathcal{Y}$ to be the space of strategy profile sets with $Y$ the set of welfare-maximizing profiles in $\InducedGame{\ConditionDistribution}$, and $\norm{Y - \hat{Y}}_{\mathcal{Y}}$ is then $\infty$ if $Y \not \subseteq \hat{Y}$, and otherwise it is $\sup_{\StratProfile \in Y} \Welfare(\Utility_\ConditionDistribution, \StratProfile) - \inf_{\StratProfile \in \hat{Y}} \Welfare(\Utility_\ConditionDistribution, \StratProfile)$.  We now take $B(\hat{\GameTuple}, \epsilon) \doteq \{\StratProfile \in \StratProfileSpace \ | \ \Welfare(\hat{\Utility}, \StratProfile) + \NumberOfPlayers\epsilon \geq \sup_{\StratProfile \in \StratProfileSpace}\Welfare(\hat{\Utility}, \StratProfile)\}$, and may take $A(\hat{\GameTuple}, \epsilon) \doteq \SetOfPlayers \times B_1(\hat{\GameTuple}, \epsilon)$, as in this case, the set of possibly optimal strategy profiles is the quantity we wish to estimate, and the remaining profiles may be pruned as they can't possibly optimize utilitarian welfare.  

To estimate the set of maximin-optimal strategies for player $\PlayerIndex$, we now take $\mathcal{Y}$ to be the space of strategies sets for $\PlayerIndex$, and now take $\norm{Y - \hat{Y}}_{\mathcal{Y}}$ to measure the suboptimality of the estimated strategy set, or $\infty$ if $Y \not \subseteq \hat{Y}$, and take $B(\hat{\GameTuple}, \epsilon) \doteq (\{ \StratProfile \ | \ \PessimalValue(\hat{\Utility}, \PlayerIndex, \Strategy) + \epsilon \geq \MinimaxValue(\hat{\Utility}, \PlayerIndex) \}, \epsilon)$, and now take $A \doteq \{\PlayerIndex\} \times B_1(\hat{\GameTuple}, \epsilon)$.  

The case of pure Nash equilibria is similar; we take $\mathcal{Y}$ to be the space of strategy profile sets, and again take $\norm{\cdot}_\mathcal{Y}$ to measure error with respect to perfect recall and approximate precision, and obtain $B(\hat{\GameTuple}, \epsilon) \doteq (\Nash_{2\epsilon}(\hat{\GameTuple}), 2\epsilon)$ and $A \doteq \SetOfPlayers \times \Nash_{2\epsilon}(\hat{\GameTuple})$.  Finally, the case of mixed Nash equilibra exhibits greater subtlety, as even if a strategy profile has high regret, it may occur with nonzero probability in a Nash equilibrium for some \emph{mixed strategy profile}.  In this case, we take $B(\hat{\GameTuple}, \epsilon) \doteq (\Nash^{\diamond}_{2\epsilon}(\hat{\GameTuple}), 2\epsilon) $ and $A$ to yield the set of all UtilityUtilityIndices that do not contain a $2\epsilon$-iteratively dominated strategy (as computed via iterated elimination of $2\epsilon$-dominated strategies).

\cyrus{Need to discuss how the pruning function (and thus the quantity we want to estimate) impacts sample complexity.  Ex. pure Nash pruning criterion dominates mixed, so always require less for pure.}

\cyrus{We could say something about estimating multiple quantities simultaneously, pruning functions, estimating the utility function (absolute and relative guarantees).  We should also contrast between estimating real parameters (optimal value) and sets (set of approximately-optimal), and the dichotomy between the optimization problem and the dual-containment set stuff.  We should also discuss the perfect-recall approximate-precision guarantee and alternatives.}

%TODO: Should talk about sets versus real numbers.
%To estimate the set of $\epsilon$-utilitarian-welfare optimal profiles, we take $\norm{Y - \hat{Y}}_{\mathcal{Y}} = ?$

%Utilitarian welfare maximization is discussed above, minimax-optimal values and actions 



%TODO: Older informal version, anything good we can mine out of this?
\if 0
The simplest instantiation of \PSP{} is to estimate an $\epsilon$-uniform approximation of $\GameTuple_{\ConditionDistribution}$.  In this case, $\norm{\cdot}_B = \norm{\cdot}_\infty$, and we may take $B(\GameTuple, \epsilon) = (\GameTuple, \epsilon)$.  Once utilities are estimated well enough to prune, the game has been learned, so in this case, we gain no benefit from pruning, and may thus take $A(\GameTuple, \epsilon) = \SetOfPlayers \times \StratProfileSpace$.  As a second example, if we want to uniformly estimate the \emph{maximum utilitarian welfare} of a game, we may take $\norm{\cdot}_B = \abs{\cdot}$, $B(\hat{\GameTuple}, \hat{\epsilon}) = (\sup_{\StratProfile \in \StratProfileSpace}\Welfare(\hat{\Utility}, \epsilon), \NumberOfPlayers\epsilon)$, and $A(\hat{\GameTuple}, \hat{\epsilon})$ can be used to prune any strategy profile with $2\NumberOfPlayers\hat{\epsilon}$-suboptimal empirical utilitarian welfare.  We can similarly estimate mixed Nash equilibria, by taking $B(\hat{\GameTuple}, \hat{\epsilon}) = (\Nash^{\diamond}_{2\hat{\epsilon}}(\hat{\GameTuple}), 2\epsilon)$, and taking $A$ to prune strategies that are $2\epsilon$-dominated (see \citep{gibbons1992game} for details as to why this is valid) \cyrus{need to work out details of exactly what pruning function does there.}  We can similarly handle the case of pure Nash equilibria, but in this case we may employ a stronger pruning criterion that simply prunes any strategy profile $\StratProfile$ that has regret $> 2\epsilon$ for some player (as $\Regret(\hat{\GameTuple}, \StratProfile) > 2\hat{\epsilon} \implies \Regret(\GameTuple_{\ConditionDistribution}, \StratProfile) > 0$.  \cyrus{Probably want all these $\hat{\epsilon}$s to be $\epsilon$.}

\cyrus{Above introduces PSP, explains the meta-algorithm, and how pruners and estimators work.  The algorithm pseudocode uses them as well.  I now need to prove the properties.}

%Next, we present \PSP, which prunes strategies, and thereby has the potential to expedite learning, and obtain tighter bounds than \GS, given the same number of samples and computation time.  During each iteration, \PSP{} removes strategies which are provably irrelevant to the property of interest, freeing up computational and statistical power for the remaining strategies.  Moreover, \PSP{} terminates once the desired approximation accuracy is reached.

\cyrus{Let's try to combine the detailed content below with the extremely terse content in the above paragraph.  There's a middle ground where we can explain these pruning criteria clearly and concisely, and briefly express why the pruning doesn't effect the solutions..}

When the property of interest is Nash equilibrium, \PSP{} includes as a subroutine the iterative removal of dominated strategies.  When it is utilitarian welfare, \PSP{} removes welfare-dominated strategies.  These concepts are defined presently.

\begin{definition}[$\epsilon$-Utilitarian Welfare Dominated Strategy]
Given a game $\GameTuple$,
a strategy profile $\StratProfile \in \StratProfileSpace$ is said to $\epsilon$-\mydef{utilitarian welfare dominate} another strategy profile $\StratProfile' \in \StratProfileSpace$ if 
$\Welfare (\GameTuple, \StratProfile) \geq \Welfare (\GameTuple, \StratProfile') + \epsilon$.
\end{definition}

\begin{definition}[$\epsilon$-Utilitarian Welfare Dominated Set]
The set $\WelUndom_{\epsilon} (\GameTuple)$ is the set of strategy profiles that remain after removing all $\epsilon$-utilitarian welfare dominated strategy profiles.
\end{definition}

\begin{definition}[$\epsilon$-Dominated Strategy]
Given a game $\GameTuple$,
a strategy $\Strategy \in \StrategySet_\PlayerIndex$ for agent $\PlayerIndex$ is said to $\epsilon$-\mydef{dominate} another strategy $\Strategy' \in \StrategySet_\PlayerIndex$ if, for all pure strategy profiles $\StratProfile$, it holds that $\Utility_\PlayerIndex(\StratProfile) \geq \Utility_\PlayerIndex(\StratProfile') + \epsilon$, where $\StratProfile' = (\Strategy_1, \dots, \Strategy_{\PlayerIndex-1}, \Strategy, \Strategy_{\PlayerIndex+1}, \dots, \Strategy_{\NumberOfPlayers})$.
\end{definition}

\begin{definition}[Iterative Elimination of $\epsilon$-Dominated Strategies]
The \emph{$\epsilon$-rationalizable} strategies $\CKR_{\epsilon}(\GameTuple)$ of game $\GameTuple$ are those that remain after iteratively removing all $\epsilon$-dominated strategies.
\end{definition}

Only strategies in $\WelUndom_{0}(\GameTuple)$ can maximize welfare, and only strategies in $\CKR_{0}(\GameTuple)$ can have positive weight in a mixed $\epsilon$-Nash equilibria~\cite{gibbons1992game}. Eliminating $\epsilon$-dominated strategies 
%and $\epsilon$-welfare dominated strategies are
is thus a natural pruning criterion. The next definition is convenient when referring to games with pruned strategies.

\begin{definition}[Restricted Game]
Given game $\GameTuple$ and $\StratProfileSpace' \subseteq \StratProfileSpace(\GameTuple)$, define $\restrict(\GameTuple, \StratProfileSpace')$ as the game $\GameTuple$ that ignores  strategies $\StratProfileSpace \setminus \StratProfileSpace'$. \cyrus{Not sure if ``ignores'' is a clear definition, and I think we need to be able to ``ignore'' (strategy profile, player) pairs.}
\end{definition}

\fi

\input{algorithms/PSP_generic}

%\todo{Next version of this algorithm needs to work on confidence intervals, which changes how the pruning function and estimation function work.  The function can then return the grand average, rather than the final average, as the estimate of $\Utility$, which is slightly biased (fully controlled for by the CI), but more accurate.}

\begin{theorem}[Approximation Guarantees of Progressive Sampling with Pruning]
\label{thm:psp-guarantee}
Suppose conditional game $\GameTuple$ and distribution $\ConditionDistribution$, 
%such that all utility values are restricted to an interval of length $\UtilityRange$.
such that for all $\StratProfile \in \StratProfileSpace$, $\PlayerIndex \in \NumberOfPlayers$, it holds that $\Utility_{\PlayerIndex}(\SamplePoint, \StratProfile) \in [a, b]$, and take $\UtilityRange \doteq b - a$.  Suppose also $\bm{M}, \epsilon, \bm{\delta}, A, B$, and $\textsc{Bound}$ as required by \PSP{}. 
%, such that for some $\norm{\cdot}_\mathcal{Y}$, $\forall \hat{\epsilon}, \hat{\GameTuple} \text{s.t.} \norm{\GameTuple_{\ConditionDistribution} - \hat{\GameTuple}}_\infty \leq \hat{\epsilon}$, it holds that $\norm{B_1(\hat{\GameTuple}, \hat{\epsilon}) - B_1(\hat{\GameTuple}_\ConditionDistribution,0)}_\mathcal{Y} \leq B_2(\hat{\GameTuple}, \epsilon)$.  
Now take $(\hat{Y}, \hat{\epsilon}, \hat{\delta}) \gets \PSP(\GameTuple, \ConditionDistribution, \bm{M}, \epsilon, \bm{\delta}, A, B, \UtilityRange, \textsc{Bound})$.  The following then hold:
%
\begin{enumerate}

\item \label{thm:psp-guarantee:delta} $\hat{\delta} \leq \sum_{\delta_i \in \bm{\delta}} \delta_i$ %, \hat{\delta} \in (0, 1)$.

\item \label{thm:psp-guarantee:epsilon} If $\displaystyle \lim_{i \to \infty} \nicefrac{\ln(\bm{\delta}_{i})}{\bm{M}_i} = 0$ and $\displaystyle \lim_{\epsilon \to 0^+} \smallsup{\hat{\GameTuple} \ | \ \norm{\GameTuple_{\ConditionDistribution} - \hat{\GameTuple}} \leq \epsilon} B_2(\hat{\GameTuple},\epsilon) = 0$, then $\hat{\epsilon} < \epsilon$% and $\hat{\delta} \leq \sum_{\delta_i \in \bm{\delta}} \delta_i$.

\vspace{-0.05cm}
\item \label{thm:psp-guarantee:error} %$\Probp{\norm{\hat{Y} - B_1(\InducedGame{\ConditionDistribution}, 0)} > \hat{\epsilon}} \leq \hat{\delta}$.
With probability at least $1 - \hat{\delta}$, $\lVert{B_1(\InducedGame{\ConditionDistribution}, 0) - \hat{Y}\rVert}_\mathcal{Y} \leq \hat{\epsilon}$
\end{enumerate}

\cyrus{I'd like to show that if $B_2(\cdot, \epsilon) \leq Q(\epsilon)$ for some $Q$, then we can obtain high-probability guarantees about the number of samples consumed by PSP that are competitive with Hoeffding-GS where an oracle tells you how many samples to use, even if no pruning ever actually occurs (proving pruning will occur is very complicated, and depends on the data distribution and the pruning criterion).}
\end{theorem}

\if 0

Furthermore, with probability at least $1 - \hat{\delta}$, the following hold (simultaneously):

\begin{enumerate}
\setcounter{enumi}{2}
\item \label{thm:psp-guarantee:dominated} $(\strategies(\InducedGame{\ConditionDistribution}) \setminus \strategies(\hat{\GameTuple})) \intersect \CKR_0(\InducedGame{\ConditionDistribution}) = \emptyset$ 
%$\forall s$ such that $s \in \strategies(\Gamma) \setminus \strategies(\hat{\GameTuple})$, $\exists s' \neq s \in \strategies(\Gamma)$ such that $s'$ dominates $s$. \cyrus{Is there a more concise term for a dominated strategy?}
\item \label{thm:psp-guarantee:norm} $\norm{\restrict(\InducedGame{\ConditionDistribution}, \strategies(\hat{\GameTuple})) - \hat{\GameTuple}}_\infty \leq \hat{\epsilon}$.
\item \label{thm:psp-guarantee:nash} $\Nash(\InducedGame{\ConditionDistribution}) \subseteq \Nash_{2\hat{\epsilon}}(\hat{\GameTuple}) \subseteq \Nash_{4\hat{\epsilon}}(\InducedGame{\ConditionDistribution})$.
\end{enumerate}

\fi

\amy{also, i didn't read the proof yet.}

\begin{proof}
First note that (\ref{thm:psp-guarantee:delta}) follows, as $\hat{\delta}$ is computed via union bound as a partial sum of $\bm{\delta}$.  To see (\ref{thm:psp-guarantee:epsilon}), first note that the limit condition on $\lim_{\epsilon \to 0^+} \sup_{\hat{\GameTuple} \ | \ \lVert{\GameTuple_{\ConditionDistribution} - \hat{\GameTuple}}\rVert \leq \epsilon} B_2(\hat{\GameTuple},\epsilon)$ implies that there exists an $\epsilon' > 0$ such that an $\epsilon'$-approximation of the unpruned UtilityUtilityIndices of $\GameTuple_{\ConditionDistribution}$ is sufficient to obtain an $\epsilon$-approximation $\hat{Y}$ of $Y$ (this follows via the properties described in \cref{def:pruning-estimation}).  Furthermore, under the limit condition on $\nicefrac{\ln(\bm{\delta}_i)}{\bm{M}_i}$, both the Hoeffding + union and Rademacher bounds used in \GS{} tend to 0 (as both decay as $\mathcal{O} \sqrt{\nicefrac{\ln(\bm{\delta}_i^{-1})}{\bm{M}_i}}$), thus eventually \PSP{} reaches a sufficient sample size to produce this $\epsilon'$, after which $B$ produces a $\hat{Y}$ that satisfies the desideratum.  Finally, (\ref{thm:psp-guarantee:error}) holds, as if \PSP{} terminates at time $t$, union bound over \GS{} in rounds $1, \dots, t$ guarantees that with probability at least $1 - \sum_{i=1}^t \bm{\delta}_t = 1 - \hat{\delta}$, each round of \GS{} produces an estimate of the unpruned utilities of $\GameTuple_{\ConditionDistribution}$ with some $\hat{\epsilon}_t$ guarantee (line~\ref{alg:psp:gs}), and the estimate $\hat{Y}$ produced by $B$ is then a $\hat{\epsilon}_t'$ guarantee (line~\ref{alg:psp:estimation}, as required by \cref{def:pruning-estimation}), which in the final iteration of \PSP{} is returned as $\hat{\epsilon}$, thus we may conclude the result.
\end{proof}

\if 0

\ref{thm:psp-guarantee:delta} and \ref{thm:psp-guarantee:epsilon} follow rather straightforwardly from examination of \PSP.  \ref{thm:psp-guarantee:delta} follows, as $\hat{\delta}$ is a sum over some subsequence of $\bm{\delta}$, each term of which and the sum of which are in the range $(0, 1)$.  \ref{thm:psp-guarantee:epsilon} is more subtle, but note that under these conditions, the Hoeffding + union and Rademacher bounds used in \GS{} tend to 0 asymptotically, thus eventually \PSP{} reaches a sufficient sample size, and terminates with the desired approximation.
\amy{i'm confused; i thought it could fail.}

For each of \ref{thm:psp-guarantee:dominated}, \ref{thm:psp-guarantee:norm}, \ref{thm:psp-guarantee:nash}, we first assume the conclusions of Theorem~\ref{thm:global-guarantee} hold with probability at least $1 - \hat{\delta}$.  The remainder of the proof is conditional on this property.

We now show \ref{thm:psp-guarantee:dominated}.  
%We seek to show that any pure strategy in $\GameTuple$ not dominated by another strategy appears in $\hat{\GameTuple}$. 
At each iteration, it holds that $\norm{\restrict(\Gamma_\ConditionDistribution, \hat{S}_t) - \hat{\Gamma}_t}_\infty \leq \epsilon_t$.  So no pure strategy that is rational in $\Gamma_\ConditionDistribution$ could be $2\epsilon$-irrational in $\hat{\Gamma}_t$.  We thus conclude that pruning removes only strategies that are irrational in $\Gamma_\ConditionDistribution$, and the claim holds.

\ref{thm:psp-guarantee:norm} is a direct consequence of the most terminal\amy{???} application of \GS.  \ref{thm:psp-guarantee:nash} follows similarly, noting that no Nash equilibrium of $\Gamma_\ConditionDistribution$ ever involves any dominated strategies.

\fi

Finally, we propose two possible sampling and failure probability schedules for \PSP, $\bm{M}$ and $\bm{\delta}$, depending on whether the sampling budget is finite or infinite.  Given a finite sampling budget $m < \infty$, a neutral choice is to take $\bm{M}$ to be a doubling sequence such that $\sum_{p \in \bm{M}} p \leq m$, with $\bm{M}$ sufficiently large so as to possibly permit pruning after the first iteration (iterations that neither prune nor achieve $\epsilon$-accuracy are effectively wasted), and to take $\bm{\delta}_i = \nicefrac{\delta}{\abs{\bm{M}}}$, where $\delta$ is some maximum tolerable failure probability.  This strategy %always respects the sampling budget, but
may fail to produce the desired $\epsilon$-approximation, as it may exhaust the sampling budget first.  
%, but may terminate with an $\hat{\epsilon}$ greater than the requested approximation threshold $\epsilon$ if the sampling schedule is exhausted
%If we want the tightest bound possible, without regard to computational or sample computation, we may take $\epsilon=0$, ensuring PSP runs to completion.  %Good content, had to get cut for a page limit.
If we want to guarantee a particular $\epsilon,\delta$-approximation, then we can take $\bm{M}$ to be an infinite doubling sequence, and $\bm{\delta}$ to be a geometrically decreasing sequence such that $\sum_{i=1}^\infty \bm{\delta}_i = \delta$, for which the conditions of Theorem~\ref{thm:psp-guarantee}(\ref{thm:psp-guarantee:epsilon}) hold. 
%though it may take an arbitrarily large number of samples to do so.

==> conclusion.tex <==
\section{Summary and Future Directions}

Estimating \emph{all\/} the utilities in an empirical game is non-trivial, in part because of the \mydef{multiple comparisons problem} (MCP), which arises when estimating many parameters simultaneously, since accurate inferences for each individual parameter do not necessarily imply a similar degree of accuracy for the parameters in aggregate.  Controlling the \mydef{family-wise error rate} (FWER)---the probability that one or more of the approximation guarantees is violated---is one way to control for multiple comparisons.
%
In this work, we consider two approaches to FWER control in empirical games.
The first builds on classical methods, using concentration inequalities to first establish confidence intervals about each parameter \emph{individually}, and then applying a statistical correction (e.g., Bonferroni or \v{S}id\'{a}k) to bound the probability that all 
%confidence intervals 
approximation guarantees hold \emph{simultaneously}, often incurring
%inducing \amy{introducing? (i know inducing is what you meant -- i.e., that it isn't a typo -- but i like introducing better if it is okay with you)}
looseness in one or both steps.
The second is based on Rademacher averages, which directly bound the error of all parameters simultaneously, by replacing the per-parameter concentration inequalities with a single concentration inequality, and an additional data-dependent term, thereby circumventing the looseness inherent in classical methods.
%, at the cost of introducing a data dependency.



This work is a contribution to the 
%incipient
theoretical literature on empirical game-theoretic analysis, a methodology for the analysis of multi-agent systems.
%
One important future-work application for our techniques is equilibria estimation in meta-games.
%~\citep{tavares2016rock,wellman2006methods}, 
Meta-games are simplified versions of intractably large games, where, instead of modeling every possible strategy an agent might implement, one analyzes a game with a substantially reduced set of strategies, each of which is usually given by a complicated algorithmic procedure (i.e., a heuristic). For example, 
%instead of analyzing a game in terms of its low-level game-theoretic strategies---a computationally intractable task in a game such as Go---
one might analyze a reduced version of the game of Starcraft~\citep{tuyls2018generalised} where agents play according to higher-level strategies given by reinforcement learning algorithms: e.g., variants of AlphaGo~\citep{silver2016mastering}.
Simulation is in order; and since each run of the game can result in either agent winning (depending on various stochastic elements, including possibly the agents' strategies), one can only obtain noisy utilities. Our techniques are directly applicable to the construction of empirical meta-games, and provide guarantees on the quality of the properties of the corresponding simulation-based meta-games.

Our methodology is also applicable in the area of \mydef{empirical mechanism design}~\citep{vorobeychik2006empirical}, where the mechanism (game) designer wishes to optimize the rules of a game so that the ensuing equilibria achieve certain goals. For example, a network designer might want to minimize \emph{congestion} assuming selfish agents~\citep{roughgarden2002bad}.
In related work, we extend our methodology so that we can learn empirically optimal mechanisms, under appropriate assumptions~\citep{areyan2019pmduu}.


While uniform $\epsilon$-approximations allow us to estimate equilibria, not all properties of games can be estimated using approximations.
For example, while a uniform $\epsilon$-approximation allows us to estimate welfare to within $\NumberOfPlayers\epsilon$ additive error, they are not sufficient to estimate the welfare of the \emph{worst\/} (pure or mixed) Nash equilibrium, because the worst Nash equilibrium in $\GameTuple'$ could be arbitrarily better or worse than the worst equilibrium in $\GameTuple$, and even the worst $2\epsilon$-Nash equilibrium in $\GameTuple'$ could be arbitrarily worse than the worst Nash equilibrium in $\GameTuple$.  Thus quantities like the \mydef{price of anarchy} are also difficult to estimate, even given a uniform $\epsilon$-approximation.


\if 0

We subsequently showed that other properties that exhibit various notions of instability cannot easily be approximated, in the sense that, without additional assumptions, no value of $\epsilon$ is sufficient to yield an approximation bound.

\fi


Traditional approaches to empirical game-theoretic analysis, including past theory that employed statistical analysis, applied solely to finite games.
%, meaning finitely many agents and finite pure strategy spaces.
Likewise, our learning algorithms depend on an enumeration of all agents' utilities at all pure strategy profiles.
Our Rademacher bounds, however, do not require the finite assumption; they apply even to 
%infinite 
games with an infinite number of utilities, including countably infinite (or uncountably infinite, subject to standard measurability concerns) agents and/or pure strategies.
In future work, we will extend our methods to use function approximators in infinite games, and establish uniform convergence from only a finite sample, under alternative assumptions: e.g., Lipschitz utilities in games with finitely many agents and bounded, continuous pure strategy spaces.
%%%From convo w/ Cyrus:
%With parametric models, we can perhaps show that these models nearly uniformly approximate the simulation-based game using only a finite sample; with non-parametric models, we will have to do some work to show that the Rademacher averages converge. 
Finally, we also hope to replace the generic McDiarmid concentration inequalities used to show the Rademacher bounds with tighter concentration inequalities, after making additional assumptions, such as uniformly bounded variance.

%The bound is actually proved by combining 4 different concentration inequalities with tail bounds (the idea is quite simple, but the details are very messy).  One of them uses the empirical variance (specifically the largest empirical variance of any function in the family), because if that is small, it means the 1-draw estimation of the Rademacher average (with a few extra details) also has low variance.  Then, at the end, it uses the distribution-variance (largest distribution variance of any function in the family), to prove that every function in the family has a sample average that approximates the distribution average.  While we could assume we know the distribution variance a priori, that's less useful in practice, so I structured the bound to compute the sample variance, and bound the distribution variance in terms of the sample variance, so the assumption is not required (i.e., the bound is data-dependent, both in terms of empirical variance and empirical Rademacher averages).

%%%% I (Enrique) have commented out this to produce the ArXiv pdf! But, we should get back to this at some point.

\begin{comment}
\cyrus{We should compare what we're doing to bandit strategies and multiplicative weights update.}
\amy{Cyrus, can you please be more specific about what you mean here? thanks.}

\amy{should we uncomment out the Chernoff bound stuff? that is, why not include those results as well in this version of unlimited length, esp.\ if they compare favorably / relate well to the literature.}
\cyrus{Yes, we can use the subgaussian bound stuff; it allows us to handle games with unbounded noise, so long as the noise is ``subgaussian,'' which intuitively means that the likelihood of drawing a point that is $x$ away from the mean decays at least at a $e^{-x^2}$ rate (which is the Gaussian decay rate).  The main problem is in the presentation: now we need to explain that $c$ is the bounded difference for McDiarmid's inequality, and Rademacher bounds, but is the subgaussian constant (which acts like the standard deviation of a Gaussian).  The other issue is that we weaken the case for the Rademacher bounds, as these can only handle the bounded-noise case.}
\amy{future work}
\end{comment}

==> derived-games.tex <==
We can apply \Cref{cor:lipschitz-properties} and \Cref{cor:dual_containment} not only to estimate properties of NFGs, but further to estimate properties of games derived from NFGs, such as those that arise when computing correlated equilibria, and team games, defined herein.
\samy{}{(See Appendix~\ref{sec:derived}.)}

%\input{correlated}
%\input{team_games}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

%%% MIXED NASH EXP'TS
%\amy{Enrique, why no exp'ts with mixed NE? b/c of PPAD-completeness, for example?}
%\enrique{Here is something we can write to justify no mixed Nash experiments. But, the truth is, it never even occurred to me to compute mixed Nash as I don't even know how to do it and is probably very cumbersome to do! I would prefer to ignore the next bit in the final version but is there in case we decide to include it.}

%\enrique{In this paper, we wanted to test the performance of our algorithms under a variety of different games. Since computing mixed Nash-equilibria is computationally  intractable~\citep{daskalakis2009complexity} even for games with only 2 players, we opted to compute only pure Nash equilibria. Future experimental work includes testing the robustness of our algorithms assuming mixed Nash equilibria.}

\begin{remark}[Estimation Complexity]
While estimating an arbitrary game requires estimating $\NumberOfPlayers\prod_{i=1}^{\NumberOfPlayers}|\StrategySet_\PlayerIndex|$ parameters, many games of practical importance require far fewer parameters. For example, in symmetric games, where all players have the same strategy set $\StrategySet$, there are only ${\NumberOfPlayers + |\StrategySet| - 1 \choose \NumberOfPlayers}$ many pure strategy profiles \enrique{(e.g., $O(\NumberOfPlayers)$ in case $|\StrategySet| = 2$ and $O(\NumberOfPlayers^2)$ in case $|\StrategySet| = 3$)}.\amy{Enrique, vs.\ what? there should be a comparison with the non-symmetric case.}\amy{how many is this compared to the whole game in big-$O$ notation?} \enrique{This is tricky, depends on $|\StrategySet|$. I think worst-case, in O notation this is some factorial of $|\StrategySet|$ and $\NumberOfPlayers$, but I am not sure, will have to work it out later.} 

%A natural situation is one where $\StrategySet$ is small, e.g., in a meta-game, where one explores the dynamics of a limited number of complex heuristics. In this case, one would need to learn substantially fewer parameters. 
\end{remark}


%\paragraph{Uniform Approximations are not a Panacea}
\begin{remark}[Limitations of Uniform Approximations]
Some properties of games are unstable under $\epsilon$-perturbations (e.g., even $\epsilon$-uniform approximations).
For example, whether a strategy is $\gamma$-rationalizable may depend on whether another strategy is $\epsilon$-rationalizable (due to IEDS), and the gap between $\gamma$ and $\epsilon$ may be arbitrarily wide.\amy{example needed.}
\textbf{For instance, whether a strategy is rationalizable depends on which other strategies are rationalizable; thus, if it is ambiguous whether strategy $\Strategy_1$ of agent 1 is dominated by strategy $\Strategy_2$, it can be ambiguous whether strategy $\Strategy_3$ of agent 2 is rationalizable, as it could be dominated (by an arbitrarily large margin) by strategy $\Strategy_4$ of agent 2, \emph{unless\/} agent 1 plays $\Strategy_1$.}
Consequently, while estimating $\epsilon$-minimax strategies is possible, estimating $\epsilon$-minimax strategies under the common knowledge of rationality assumption (i.e., no dominated strategies) is not.\amy{example would help.}
%strategies under common knowledge of rationality are unstable in the sense that their utility values can occupy an arbitrarily large range, even when a game is uniformly $\epsilon$-approximated.
\end{remark}

==> equilibria.tex <==
\begin{theorem}[Approximability of Equilibria]
\label{thm:equilibria-approximation-bounds}
If two normal-form games, $\GameTuple$ and $\GameTuple'$, are uniform approximations of one another,
%(i.e., if $\norm{\GameTuple - \GameTuple'}_{\!\infty} \leq \epsilon$), 
then:

\begin{enumerate}
\item $\Nash(\GameTuple) \subseteq \Nash_{2\epsilon} (\GameTuple') \subseteq \Nash_{4\epsilon}(\GameTuple)$

\item $\Nash^\diamond (\GameTuple) \subseteq \Nash^{\diamond}_{2\epsilon} (\GameTuple') \subseteq \Nash^{\diamond}_{4\epsilon} (\GameTuple)$
\end{enumerate}
\end{theorem}

\begin{proof}
First note the following: if $\smash{A \subseteq B}$, then $\smash{C \cap A \subseteq C \cap B}$.
Hence, since any pure Nash equilibrium is also a mixed Nash equilibrium, taking $C$ to be the set of all pure strategy profiles, we need only show 2.
We do so by showing $\smash{\Nash^\diamond_\gamma (\GameTuple) \subseteq \Nash^\diamond_{2\epsilon + \gamma} (\GameTuple')}$, for $\gamma \ge 0$, which implies both containments, taking $\gamma = 0$ for the lesser, and $\gamma = 2\epsilon$ for the greater.

Suppose $\StratProfile \in \Nash^\diamond_\gamma (\GameTuple)$, for all $\PlayerIndex \in \SetOfPlayers$.
We will show that $\StratProfile$ is ($2\epsilon + \gamma$)-optimal in $\GameTuple'$, for all $\PlayerIndex \in \SetOfPlayers$.
%
Fix an agent $\PlayerIndex$, and
define $\MixedStratProfileSpaceAlt_{\PlayerIndex, \StratProfile} \doteq \{ \MixedStratProfileAlt \in \MixedStratProfileSpace \mid \MixedStratProfileAlt_q = \StratProfile_q, \forall q \neq \PlayerIndex \}$.
In words, $\MixedStratProfileSpaceAlt_{\PlayerIndex, \StratProfile}$ is the set of all mixed strategy profiles in which the strategies of all agents $q \ne \PlayerIndex$ are fixed at $\StratProfile_q$.
Now take
$\StratProfile^* \in \argmax_{\MixedStratProfileAlt \in \MixedStratProfileSpaceAlt_{\PlayerIndex, \StratProfile}} \Utility_\PlayerIndex (\MixedStratProfileAlt)$ and
$\StratProfile'^* \in \argmax_{\MixedStratProfileAlt \in \MixedStratProfileSpaceAlt_{\PlayerIndex, \StratProfile}} \Utility'_\PlayerIndex (\MixedStratProfileAlt)$.
%$\displaystyle\StratProfile^* \doteq  \!\!\!\!\! \argmax_{\tilde{\StratProfile} \in \MixedStratProfileSpace: \tilde{\StratProfile}_j = \StratProfile_j, \forall j \neq \PlayerIndex} \!\!\!\! \Utility_\PlayerIndex (\tilde{\StratProfile})$ and $\displaystyle{\StratProfile'}^* \doteq \!\!\!\!\! \argmax_{\tilde{\StratProfile} \in \MixedStratProfileSpace: \tilde{\StratProfile}_j = \StratProfile_j, \forall j \neq \PlayerIndex} \!\!\!\! \Utility'_\PlayerIndex (\tilde{\StratProfile})$.
%\amy{why $\doteq$ here? shouldn't it be $\in$?}
Then:
%
\begin{align*}
%\sup_{\PlayerIndex \in \SetOfPlayers}\sup_{...} 
\Regret_\PlayerIndex (\GameTuple', \StratProfile)
&= \Utility'_\PlayerIndex({\StratProfile'}^*) - \Utility'_\PlayerIndex(\StratProfile) \\
&\leq (\Utility_\PlayerIndex({\StratProfile'}^*) + \epsilon) - (\Utility_\PlayerIndex(\StratProfile) - \epsilon) \\
&\leq (\Utility_\PlayerIndex(\StratProfile^*) + \epsilon) - (\Utility_\PlayerIndex(\StratProfile) - \epsilon) \\
 &\leq (\Utility_\PlayerIndex(\StratProfile^*) + \epsilon) - (\Utility_\PlayerIndex(\StratProfile^*) - \epsilon - \gamma) = 2\epsilon + \gamma
\end{align*}

%\cyrus{Better notation for $s'^*$; primes and stars don't mix well.} \amy{i like the primes and stars. stars mean optimal. primes mean the approximate game. i think it works. but note that i got rid of the tildes.} \cyrus{I agree with that, I just don't like having both a prime and a star on the same variable.} \amy{and I agree with that! but don't have a better alternative at the moment.}

\noindent
The first line follows by definition.
The second holds by Lemma~\ref{lemma:mixed-approximation} and the fact that $\Gamma'$ is a uniform $\epsilon$-approximation of $\Gamma$, the third as $\StratProfile^*$ is optimal for $\PlayerIndex$ in $\GameTuple$, and the fourth as $\StratProfile$ is a $\gamma$-Nash in $\GameTuple$.
\end{proof}

%Proof with BRGs:
\begin{comment}
First note that 1 and 2 follow from 3 and 4, by \cref{lemma:mixed-properties}, noting that each pure %BRG edge or
equilibrium is also an %edge or 
equilibrium in the stochastic game.

\enrique{Need to update this proof to remove mentions of BRGs}
We now show 3, noting that the general form $\BRG_{\gamma}(\diamond(\GameTuple)) \subseteq \BRG_{\gamma + 2\epsilon}(\diamond(\GameTuple'))$ is sufficient to show containment in both directions (taking $\gamma = 0$ for the lesser and $\gamma = 2\epsilon$ for the greater).  For any agent $\PlayerIndex$ and edge from $\StratProfile$ to $\StratProfile'$ in $\BRG_{\gamma}(\diamond(\GameTuple))$, take $\StratProfile^*$ to be $\argmax_{\StratProfile^* \in \Neighborhood(\StratProfile)}\Utility_\PlayerIndex(\StratProfile^*)$ and ${\StratProfile'}^*$ to be $\argmax_{{\StratProfile'}^* \in \Neighborhood(\StratProfile)} \Utility'_\PlayerIndex({\StratProfile'}^*)$.  We seek to show that $\StratProfile' \in \BRG_{\gamma + 2\epsilon}(\GameTuple')$, which is equivalent to showing that $\Utility'_\PlayerIndex({\StratProfile'}^*) - \Utility'_\PlayerIndex(\StratProfile') \leq \gamma + 2\epsilon$.

\begin{align*}
\Utility'_\PlayerIndex({\StratProfile'}^*) - \Utility'_\PlayerIndex(\StratProfile') & \leq (\epsilon + \Utility_\PlayerIndex({\StratProfile'}^*)) - (\Utility_\PlayerIndex(\StratProfile') - \epsilon) & \textsc{\cref{lemma:mixed-approximation}} \\
 &\leq (\epsilon + \Utility_\PlayerIndex(\StratProfile^*)) - (\Utility_\PlayerIndex(\StratProfile') - \epsilon) & \Utility_\PlayerIndex({\StratProfile'}^*) \leq \Utility_\PlayerIndex(\StratProfile^*) \\
 &\leq (\epsilon + \Utility_\PlayerIndex(\StratProfile^*)) - (\Utility_\PlayerIndex(\StratProfile^*) - \gamma - \epsilon) & \Utility_\PlayerIndex(\StratProfile') \geq \Utility_\PlayerIndex(\StratProfile^*) - \gamma \\
 &= \gamma + 2\epsilon
\end{align*}

As this argument applies to all edges in the BRG, it is sufficient to show that $\BRG_\gamma(\diamond(\Gamma)) \subseteq \BRG_{\gamma + 2\epsilon}(\diamond(\Gamma))$, which implies 3.  4 now follows from 3, by the definitions of approximate Nash equilibria.
\end{comment}

==> experiments.tex <==
\section{Experiments}
\label{sec:expts}

In this section, we describe the performance of our learning algorithms, experimentally.
We demonstrate that they consistently outperform their theoretical guarantees, in multiple experiments with random games, under various noise conditions.
Moreover, we show that in cases of interest, \PSP{} consistently requires fewer data than \GS.
%, thus empirically outperforming the state-of-the-art.

We start by describing the games we designed for these experiments; we then present our findings. We use the notation $U[a, b]$, where $a < b$, to denote the uniform distribution, both in the discrete case ($a, b \in \N$)
%\amy{$\in \Z$?} 
%\enrique{I just checked and I think $\in \N$ is fine}
and in the continuous case ($a, b \in \R$). Unless otherwise noted (i.e., in the empirical success rate experiments), $\delta$ is fixed at $0.1$ throughout. %\amy{Enrique, is it ever otherwise? if so, please point me to where. thx.}
%\enrique{the point of the average failure rate experiment is precisely to vary $\delta$}

%with $x, y \in \R$ and $x \le y$ to denote the continuous uniform distribution over reals in the interval $(x, y)$\amy{just checking you don't mean $[x,y]$}.\enrique{no, I really mean $(x,y)$}

\subsection{Experimental Setup}
\label{subsec:experimentalSetup}

\paragraph{Uniform Random Games.} 
For $k \in \mathbb{Z}_+, u_0 \in \mathbb{R}$, a game $\GameTuple$ drawn from a uniform random game distribution $\RandomGame(\NumberOfPlayers, k, u_0)$ has $\NumberOfPlayers$ agents where each agent $\PlayerIndex$ has $k$ pure strategies. The utilities for each agent $\PlayerIndex$ in each profile $\StratProfile$ are drawn i.i.d.\ as $\smash{\Utility_\PlayerIndex (\StratProfile) \sim U(\nicefrac{-u_0}{2}, \nicefrac{u_0}{2})}$, where $u_0 > 0$ is a parameter controlling the magnitude of the utilities. We set $u_0 = 10$.

\paragraph{Finite Congestion Games.} 
Congestion games are a class of games known to exhibit pure strategy Nash equilibria~\citep{rosenthal1973class}. We use this class of games in our experiments for precisely this reason, so that we can more easily identify equilibria.

A tuple $\smash{\CongestionGame = (\SetOfPlayers, \SetOfFacilities, \{ \CongestionSetOfStrategies_\PlayerIndex \mid \PlayerIndex \in \SetOfPlayers \}, \{ \FacilityCostFunction_\FacilityIndex \mid \FacilityIndex \in \SetOfFacilities \})}$ is a \mydef{congestion game}~\citep{christodoulou2005price}, where $\smash{\SetOfPlayers = \{1, \ldots, \NumberOfPlayers\}}$ is a set of agents and $\smash{\SetOfFacilities = \{1, \ldots, \NumberOfFacilities\}}$ is a set of facilities. %$\smash{\CongestionSetOfStrategies_\PlayerIndex \subseteq 2^\SetOfFacilities}$ is the pure strategy set for agent $\PlayerIndex$. 
A strategy $\smash{\Strategy_\PlayerIndex \in \CongestionSetOfStrategies_\PlayerIndex} \subseteq 2^\SetOfFacilities$ is a set of facilities, and $\smash{\FacilityCostFunction_\FacilityIndex}$ is a (universal: i.e., non-agent specific) cost function associated with facility $\FacilityIndex$. 
%A pure strategy profile $\Strategy = (\Strategy_1, \ldots, \Strategy_{\NumberOfPlayers})$ is a vector of strategies, one for each agent.

In a finite congestion game, each agent prefers to select, among all their available strategies, one that minimizes their cost. Given a profile of strategies $\StratProfile$, agent $\PlayerIndex$'s cost is defined as $\smash{\PlayerCost_\PlayerIndex(\StratProfile) = \sum_{\FacilityIndex\in\Strategy_\PlayerIndex} \FacilityCostFunction_\FacilityIndex(n_\FacilityIndex(\StratProfile))}$, where $n_\FacilityIndex(\StratProfile)$ is the number of agents who select facility $\FacilityIndex$ in $\StratProfile$. We experiment with simple cost functions of the form $\FacilityCostFunction_\FacilityIndex(n) = n$.

For $\NumberOfPlayers \in \mathbb{Z}_+, \NumberOfFacilities \in \mathbb{Z}_+, k \in \mathbb{Z}_+$ such that $k \le 2^{\NumberOfFacilities} -1$,%
\footnote{We constrain $k \le 2^{\NumberOfFacilities} -1$, not $k \le 2^{\NumberOfFacilities}$, so that no agent's strategy set is empty.} 
%\amy{why the $-1$?}\enrique{we don't want players picking an empty strategy space}\amy{this is totally unclear without explanation, so add a footnote or maybe just delete the -1} 
a finite congestion game $\CongestionGame$ drawn from a random congestion distribution $\smash{\RandomCongestionGame(\NumberOfPlayers, \NumberOfFacilities, k)}$ is played by $\NumberOfPlayers$ agents on $\NumberOfFacilities$ facilities.
Each agent $\PlayerIndex$ is assigned a random number $\smash{\abs{\StrategySet_\PlayerIndex} \sim U[1, k]}$ of pure strategies. Each pure strategy $\Strategy_{\PlayerIndex, j} \in \StrategySet_\PlayerIndex$ is constructed as follows. The probability that facility $\FacilityIndex \in \{1, \ldots, \NumberOfFacilities\}$ is included in $\Strategy_{\PlayerIndex, j}$ is given by the power law $\smash{\mathbb{P} [\FacilityIndex \in \Strategy_{\PlayerIndex, j}] = \alpha^{-\FacilityIndex}}$, where $\alpha \in [0,1]$. We report results for $\alpha = 0.1$. This distribution is a simple but useful model of situations where agents' preferences are clustered around a few preferred facilities. Power law models abound in the literature; they are used to model distributions of population in cities, of incomes, and of species among genera, among many other applications~\citep{simon1955class, mitzenmacher2004brief}.

%\cyrus{Letters in math mode (as in the $\RandomCongestionGame$ macro) run together and just look like a bunch of variables.  Can we redefine with some other script (using for instance \\DeclareMathOperator or \\mathrm?)}
%\enrique{done}

\paragraph{Noise simulation.} To test our algorithms, we query a black-box simulator to obtain noisy samples of the agents' utilities. Given a game $\GameTuple$, a sample of
agent $\PlayerIndex$'s utility at strategy profile $\StratProfile$ is given by $\smash{\Utility_\PlayerIndex(\StratProfile, \ConditionValue) = \Utility_\PlayerIndex(\StratProfile) + \ConditionValue}$, where $\smash{\ConditionValue \sim U(\nicefrac{-\NoiseCondition}{2}, \nicefrac{\NoiseCondition}{2})}$ and i.i.d..
%those two periods are deliberate. :)
The parameter $\NoiseCondition$ controls the magnitude of the noise. 
This simple model is meant to capture situations 
%often found in practice, 
where it is hard or even impossible to make accurate distributional assumptions about noise.

==> experiments/anarchy_gap_experiments.tex <==
\paragraph{Anarchy Gap Experiments}

%\subsection{Experimental setup}

For these experiments, we draw congestion games at random using GAMUT~\cite{nudelman2004run}, a state-of-the-art suite of game generators.%\footnote{Note that we normalize all payoffs to be in range $[1, 10]$.}
Let $\GameTuple(n, k)$ be a congestion game drawn from GAMUT with $n$ players and $k$ facilities, and $\Utility_{n, k}$ its utility function. For these experiments, $\GameTuple(n, k)$ is our ground-truth game. Our goal is to observe the empirical performance of the bound given in \Cref{thm:anarchy-gap}, namely, $\abs{ \AnarchyGap_{\Lambda} (\Utility) - \AnarchyGap_{\Lambda} (\Utility') } \leq 2 (\lambda_{\Welfare} + \Lambda) \epsilon$. 

%\begin{figure}[h!]
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.35cm}
\hspace{-0.25cm}\includegraphics[width=0.48\textwidth]{experiments/graphs/cg-3-3.png}
\vspace{-0.5cm}
\caption{Anarchy gap results}
\vspace{-0.25cm}
\label{fig:anarchygapresults}
\end{wrapfigure}
%\end{figure}

For this purpose, we draw $\epsilon$-uniform approximations of $\GameTuple(n, k)$ by adding random noise to $\Utility_{n, k}$. Specifically, given $\Utility_{n, k}$, we construct $\GameTuple'(n, k)$, an $\epsilon$-uniform approximation of $\GameTuple(n, k)$, by setting $\Utility'_{n, k} = \Utility_{n, k} + \bm{\epsilon}$. Here, $\bm{\epsilon}$ is a vector of randomly drawn components where each component, $\epsilon_{\PlayerIndex, \StratProfile}$, corresponds to a pair (player, strategy profile) of $\GameTuple(n, k)$. 

We experimented with two noise models: a mean-concentrated model and a biased model. 
%
In the mean-concentrated model, for each $(\PlayerIndex, \StratProfile)$, we draw $\epsilon_{\PlayerIndex, \StratProfile}$ from a Wigner-semicircular distribution on range $[-\epsilon, \epsilon]$. The goal of this model is to have the utilities of the estimated game closer to the utilities of the ground-truth game (as one would expect via, for example, the central limit theorem) than tail bounds would mandate.
%
In the biased model, for each $(\PlayerIndex, \StratProfile)$, we draw $\epsilon_{\PlayerIndex, \StratProfile}$ from an arcsine distribution on range $[-\epsilon, \epsilon]$. The goal of this model is to have the utilities of the estimated game farther away from the utilities of the ground-truth game, as more-extreme games are more likely to exhibit large changes in $\AnarchyGap_{\Lambda}(\cdot)$.

\Cref{fig:anarchygapresults} shows a representative result for $\AnarchyGap_{\Lambda}(\Utility_{3, 3})$. The figure shows several violin plots, one plot for each value of $\Lambda \in \{0, 0.25, 0.5, \ldots, 2.0\}$. Each half of a violin plots the distribution of $\AnarchyGap_{\Lambda}(\Utility'_{3, 3})$ for each of reduced bias and biased noise models. The plot also shows the upper and lower bound of \Cref{thm:anarchy-gap}, as dashed lines. Finally, the plot shows a dashed line representing an improved upper-bound on $\AnarchyGap_{\Lambda}$  by noting 
this quantity decreases monotonically in $\Lambda$. 

%\cyrus{future work: prove / reference monotonicity}\enrique{fill here: montonicity of upper bound}. \enrique{stuff missing: what welfare functions was used for experiments? answer, the utilitarian welfare! as defined in this paper, i.e., the average of all utilities.}

%\enrique{Add analysis of results}\cyrus{in future work}


==> experiments/nashHistogram.tex <==
\paragraph{$2\epsilon$-Nash learning as a function of the number of samples.}
In these experiments, we ran the GS algorithm using 1-ERA bounds on one game with 32 strategy profiles drawn from distribution $\RandomCongestionGame(5,5,2)$ with noise parameter $\NoiseCondition = 2$. This game has a unique pure Nash equilibrium.
%, which we found via exhaustive search.

\Cref{fig:1ERA-GS-Performance} (b) depicts four histograms, corresponding to four different sample sizes, each one plotting the frequencies of strategy profiles deemed pure $2\epsilon$-Nash equilibria, using exhaustive search and applying Theorem~\ref{thm:gs-guarantee} to the error returned by \GS. The profiles not shown had zero frequency. The unique pure Nash equilibrium is correctly identified in all cases. Moreover, as the number of samples increases, the frequency of false positives (i.e., profiles that are not Nash but are deemed so by \GS) decreases.
%confirming in practice our methodology. 

%depicts the ability of \GS{} to correctly identify $2\epsilon$-Nash equilibria while at the same time reducing the number of false positive, i.e., profiles that are not pure Nash but are deemed so by \GS. 

%\cyrus{Can we also plot the frequency with which any SPs that are not $4\epsilon$-Nash are claimed to be $2\epsilon$-Nash?  We want to show that this is happens < $\delta$ proportion of the time.}
%\enrique{This is a great idea, I will see if I have time to finish this today. We do have the failure probability experiments which test both containments.}
%\amy{there seem to be a few questions to ask here: 
%\begin{itemize}
%\item the one Enrique answers: confirmation that the set of 2eps-eqa GS finds contains the true eqm? 
%\item the one Cyrus asks: are any of the 2eps-eqa GS finds not even true 4eps eqa? this should not happen more than $\delta$ percent of the time.
%\end{itemize}}

\begin{comment}
\enrique{move this somewhere else!}
Moreover, we have observed through multiple draws from $\RandomGame$ and $\RandomCongestionGame$ distributions, as well as multiple runs of \GS, that the true Nash equilibria are consistently identified almost always, despite the fact that our guarantees are only for $1 - \delta = 0.9$ fraction of time.
\end{comment}

\begin{comment}
Figure~\ref{fig:nashHistogramRandomGame} is a similar collection of histogram as shown in Figure~\ref{fig:nashHistogramCongestionGame}, but for a bigger game drawn from distribution $\RandomGame(4, 2, 10)$ with a total of 16 strategy profiles. Note that for a small number of samples (50), the algorithm considers every strategy profile as an $\epsilon$-Nash equilibrium at least once. As the number of samples increases, fewer strategies are considered equilibria (strategies not shown in the histogram had zero frequency). For a relatively large number of samples (500) the algorithm has narrow down all the possible Nash equilibria to only 4 strategy profiles. Note that the game contains two pure strategy profiles: (0,0,0,1) and (1,1,0,0).
\end{comment}

==> experiments/old_probFailure.tex <==
\begin{comment}
\begin{figure}
    \centering
    %\includegraphics[width=0.40\textwidth]{experiment_results/graphs/73DI3L_failure_plot.png}
    \includegraphics[width=0.40\textwidth]{experiment_results/graphs/failure_prob.png}
    \captionsetup{justification=centering}
    \caption{Average failure rate vs.\ theoretical bounds, for \GS{}.}
    \label{fig:probFail}
\end{figure}
\end{comment}

\begin{comment}
\paragraph{Empirical probability failure.}
In these experiments, we test the probabilistic guarantees of \GS. As stated in \cref{thm:global-guarantee}, \GS{} returns with probability at least $1 - \delta$ a set of estimated $2\epsilon$-Nash equilibria which contains all the Nash equilibria of the induced game and is contained in the set of $4\epsilon$-Nash equilibria of the induced game. For simplicity, in these experiments we test these containments only for pure $\epsilon$-Nash equilibria. In \cref{fig:probFail}, we report 95\% confidence intervals around the empirical probability of failure of \GS{} for 200 games drawn from $\RandomGame(3,3)$ and 200 games drawn from $\RandomCongestionGame(3,3,2)$. The empirical probability of failure is simply the ratio of the count of times the algorithm succeed to meet the conditions of \cref{thm:global-guarantee} to the total number of times the algorithm was executed, which in this case is 200 times for each value of $\delta$ and each game. As per our guarantees, the failure probability should be above line $1 -\delta$, shown in \cref{fig:probFail} in black. In the figure we plot the empirical probability estimate for multiple values of noise $c \in \{5,10,50,100\}$. We note that the algorithm consistently meets its $1-\delta$ guarantee and for our experiments it is very often the case that guarantees of \cref{thm:global-guarantee} are meet with empirical probability close to 1. 
\end{comment}

==> experiments/probFailure.tex <==
\paragraph{Empirical success rate.}
In these experiments, we ran the \GS{} algorithm using 1-ERA bounds and Hoeffding's bound with a Bonferroni correction on 200 games drawn at random from $\RandomCongestionGame(3, 3, 2)$ and another 200 games drawn at random from $\RandomGame(3,3)$, both with $\NoiseCondition = 5$. 

In~\Cref{fig:GSvsPSP} (a), we report 95\% confidence intervals around the empirical success rate, meaning the ratio of the number of times the algorithm's output satisfies $\Nash(\InducedGame{\ConditionDistribution})  
    \subseteq 
\Nash_{2\epsilon}(\hat{\GameTuple}_{\Samples})$ and 
$\Nash_{2\epsilon}(\hat{\GameTuple}_{\Samples}) 
    \subseteq 
\Nash_{4\epsilon}(\InducedGame{\ConditionDistribution})$ to the total number of times it executes. As per our guarantees, this rate should be above the black line $1 - \delta$ (and it is). Note that we test these containments only for pure $\epsilon$-Nash equilibria.

To test the extent to which the bounds computed by \GS{} are tight, we contract the value of $\epsilon$ output by \GS{} by a factor $\rho \in \{1.0, 0.875, 0.75, 0.625, 0.5\}$. Even so, \GS{} consistently meets its $1-\delta$ guarantee, and in these experiments design, it is very often the case that guarantees 
%of Theorem~\ref{thm:gs-guarantee} 
are met with empirical probability close to 1, except when $\rho = 0.5$ and $\delta < 0.15$. 
\amy{how many samples were used in these exp'ts?}

==> experiments/pspResults.tex <==
\paragraph{Evaluation of \PSP} 
We now compare the performance of \GS{} to \PSP{} with a doubling schedule initialized at 100 samples. (As usual, we fix $\delta = 0.1$.) Since our experimental testbed only includes small games, we present results only for the (Bonferroni) correction-based variants of these algorithms, leaving experiments using Rademacher averages for future work.
Our procedure to fairly compare them is as follows. We first run \PSP{} with $\epsilon = 0$, thereby forcing the algorithm to run to completion. In this way, we obtain the error rate corresponding to \PSP's final \GS{} invocation. We call this quantity $\smash{\hat{\epsilon}}_{\PSP}$, and we denote by $M_{\PSP}$ the total number of samples used upon termination.
%the sum of all samples used to estimate all quantities $\Utility_\PlayerIndex(\StratProfile)$. 
Now, since \GS{} takes in a number of samples which is used uniformly across all players and strategy profiles %$\Utility_\PlayerIndex(\StratProfile)$
to produce error rate $\smash{\hat{\epsilon}}_{\GS}$, we compute $\smash{\hat{\epsilon}}_{\GS}$ 
%(using Equation~\ref{eq:H}) 
assuming \GS{} runs on $\nicefrac{M_{\PSP}}{\SizeOfGame{\GameTuple}}$ samples. In other words, we assume a uniform budget of $\nicefrac{M_{\PSP}}{\SizeOfGame{\GameTuple}}$ samples per $\Utility_\PlayerIndex(\StratProfile)$. This strategy guarantees both algorithms use the same total number of samples. 

\Cref{fig:GSvsPSP} (b) depicts $\smash{\hat{\epsilon}}$, the approximation guarantee obtained for both algorithms, as a function of the number of samples, summarizing the results of experiments with 200 games of different sizes drawn from a $\RandomGame$ distribution, with $|P| \in \{ 2, 3, 4, 5 \}$ and $k \in \{ 2, 3, 4, 5 \}$.%
\footnote{Similar behavior was observed for $\RandomCongestionGame$ with with $|P| \in \{ 5, 6, 7, 8 \}$, $|E| \in \{ 2, 3, 4, 5 \}$, and $k = 2$.}
Game size, $\SizeOfGame{\GameTuple}$, is the number of parameters, meaning the number of utilities to be estimated, which equals the number of players times the number of strategy profiles.
%
\begin{comment}
\cyrus{Is it true that $M_{PSP} = \sum_{m_i \in \bm{P}} m_i$?}
\enrique{It is true, up to a constant factor of the size of the game!, i.e., $M_{PSP} = \SizeOfGame{\GameTuple}\sum_{m_i \in \bm{P}} m_i$.}
\end{comment}
%
The plot shows $\smash{\hat{\epsilon}}_{\PSP}$ in orange and $\smash{\hat{\epsilon}}_{\GS}$ in grey, on a logarithmic scale, thereby demonstrating that, for the same number of samples, \PSP{} yields better approximations: i.e., smaller values of $\smash{\hat{\epsilon}}$. Note, however, that \PSP{} relies on having sufficiently many strategy profiles to prune in the first place. For smaller games $\SizeOfGame{\GameTuple} \in \{8, 24\}$ and relatively small values of $\epsilon$, \GS{} produces slightly better approximations, because there is relatively little opportunity for pruning. For larger games $\SizeOfGame{\GameTuple} \in \{324, 1024\}$, \PSP{} consistently yields better approximations, and moreover, the error rate improves as a function of the size of the game.
%This relationship was observed for many different sizes of $\SizeOfGame{\GameTuple}$ beyond what is reported here.


==> experiments/set_of_plots_1.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \vspace{0.25cm}
        \includegraphics[width=\textwidth]{experiments/graphs/I7ISX8.png}
        %\captionsetup{justification=centering}  
        %\caption{95\% confidence intervals around $\epsilon$.}
        %\label{fig:samplesVepsilonCongestionGame}
    \end{subfigure}    
    \mbox{}\hspace{5mm}
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \vspace{0.25cm}
        \includegraphics[width=\textwidth]{experiments/graphs/7IMQS9_freq_nash_plot.png}
        %\captionsetup{justification=centering}
        %\caption{Frequency of pure $2\epsilon$-Nash equilibria}
        %\label{fig:nashHistogramCongestionGame}
    \end{subfigure}
    \vspace{-0.75cm}
    \caption{Performance of \GS{} with 1-ERA bounds.
    (a) 95\% confidence intervals around $\epsilon$ for games drawn from $\smash{\RandomCongestionGame(5, 5, 2)}$ using different levels of noise, namely $\NoiseCondition \in \{2,5,10\}$.
    (b) Frequency of pure $2\epsilon$-Nash equilibria in one game with 32 strategy profiles drawn from distribution $\RandomCongestionGame(5,5,2)$ with noise parameter $\NoiseCondition = 2$.}
    \label{fig:1ERA-GS-Performance}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{experiments/graphs/I7ISX8.png}
    \captionsetup{justification=centering}
    \caption{Average error as a function of the number of samples, for \GS{}.}
    %\caption{95\% confidence intervals around error tolerance $\epsilon$ produced by \GS{} as a function of the number of samples.}
    \label{fig:samplesVepsilonCongestionGame}
\end{figure}
\end{comment}

\begin{comment}
    \begin{figure}
        \centering
        \includegraphics[width=0.35\textwidth]{experiments/graphs/XB05FF.png}
        \captionsetup{justification=centering}  
        \caption{95\% confidence intervals around $\epsilon$ produced by \GS{} as a function of the number of samples.}
        \label{fig:samplesVepsilonRandomGame}
    \end{figure}
\end{comment}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{experiments/graphs/QE260V_freq_nash_plot.png}
    \captionsetup{justification=centering}
    \caption{Frequency of pure $2\epsilon$-Nash equilibria when feeding different sample sizes to \GS{} over 200 runs.}
    \label{fig:nashHistogramRandomGame}
\end{figure}
\end{comment}

==> experiments/set_of_plots_2.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \vspace{-0.3cm}
        \includegraphics[width=\textwidth]{experiments/graphs/failure_prob.png}
        \vspace{-0.25cm}
        %\captionsetup{justification=centering}  
        %\caption{\GS{} Empirical Success Rate.}
        %\label{fig:probFail}
    \end{subfigure}
    \mbox{}\hspace{5mm}
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \vspace{-0.3cm}
        \includegraphics[width=\textwidth]{experiments/graphs/GSvPSP.png}
        \vspace{-0.25cm}
        %\captionsetup{justification=centering}
        %\caption{\GS{} vs \PSP{} with Hoeffding Bounds.}
        %\label{fig:GvsPSP}
    \end{subfigure}
    \vspace{-0.75cm}
    \caption{GS vs.\ PSP. 
    (a) Empirical success rate for 200 games drawn at random from $\RandomCongestionGame(3, 3, 2)$ and another 200 games drawn at random from $\RandomGame(3,3)$, both with $\NoiseCondition = 5$. 
    (b) GS vs.\ PSP for 200 games of different sizes drawn from a $\RandomGame$ distribution, with $|P| \in \{ 2, 3, 4, 5 \}$ and $k \in \{ 2, 3, 4, 5 \}$.}
    \label{fig:GSvsPSP}
\end{figure}

==> expts/poa_expts_overview.tex <==
\section{POA Experiments Overview}

We discussed two ways of doing experiments, an exact and a Monte Carlo.

\subsection{Exact mixed ILP}

Following~\cite{sandholm2005mixed}, Mixed-Integer program (\ref{eq:mixed-ILP}) computes mixed-Nash equilibria of two-player games\footnote{I think it extends to more than two players, but let's focus on two players for simplicity.} with some objective function. I write the program here with our notation and specialized it to minimizing egalitarian welfare. 
%
A piece of notation I use here that I don't see in the paper is $\Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex$.


I use notation $[\cdot]$ to denote a variable over some indices, instead of stacking sub-indices. For example, $\pi[\Strategy_\PlayerIndex]$ for the probability of player $\PlayerIndex$ playing strategy $\Strategy_\PlayerIndex$ instead of writing $\pi_{\Strategy_\PlayerIndex}$. 

The decision variables, and their respective domains, are

\begin{center}
\begin{tabular}{rl}
$z \in \R$                                  & egalitarian welfare. \\ 
$\pi[\Strategy_\PlayerIndex] \in \R^+$        & probability of player $\PlayerIndex$ playing $\Strategy_\PlayerIndex$. \\
$\Utility_\PlayerIndex \in \R$              & maximum utility player $\PlayerIndex$ makes at $\epsilon$-equilibrium. \\
$\Utility[\Strategy_\PlayerIndex] \in \R$   & player $\PlayerIndex$'s expected utility of playing $\Strategy_\PlayerIndex$. \\
$r[\Strategy_\PlayerIndex] \in \R^+$          & player $\PlayerIndex$'s regret of playing $\Strategy_\PlayerIndex$. \\
$b[\Strategy_\PlayerIndex] \in \{0, 1\}$    & indicator whether $\Strategy_\PlayerIndex$ is allowed to have positive probability. \\
$y_\PlayerIndex \in \{0, 1\}$               & auxiliary variable to minimize egalitarian objective. 
\end{tabular}
\end{center}

The formulation is based around the following property. If $b[\Strategy_\PlayerIndex] = 1$, then the strategy $\Strategy_\PlayerIndex$ is not allowed to be in the support, $\pi[\Strategy_\PlayerIndex] = 0$. If $b[\Strategy_\PlayerIndex] = 0$, then $\Strategy_\PlayerIndex$ is allowed to be in the support but the regret of the strategy for the player must be $\epsilon$. Note that $\epsilon > 0$ is a parameter of (\ref{eq:mixed-ILP}).

\begin{equation}
\label{eq:mixed-ILP}
\begin{array}{lrcll}
\text{minimize}
    & z &\\\\
\text{subject to}
    % First Constraint
    & \displaystyle\sum\limits_{\Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex}  \pi[\Strategy_\PlayerIndex]
    & = &
    1,      
    & \forall \PlayerIndex \in \SetOfPlayers\\\\

    % Second Constraint
    & \Utility[\Strategy_\PlayerIndex]
    & = &
        \displaystyle\sum\limits_{\Strategy_{1 - \PlayerIndex} \in \StrategySet_{1 - \PlayerIndex}} 
        \pi[\Strategy_{1 - \PlayerIndex}]  \cdot \Utility(\Strategy_\PlayerIndex, \Strategy_{1 - \PlayerIndex}),
    & \forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex \\\\\

    % Third Constraint
    & \Utility_\PlayerIndex 
    & \ge &
        \Utility[\Strategy_\PlayerIndex],
    & \forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex \\\\\

    % Fourth Constraint
    & r[\Strategy_\PlayerIndex]
    & = &
        \Utility_\PlayerIndex - \Utility[\Strategy_\PlayerIndex],
    & \forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex \\\\\

    % Fifth Constraint
    & \pi[\Strategy_\PlayerIndex]
    & \leq &
        1 - b[\Strategy_\PlayerIndex],
    & \forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex \\\\\

    % Sixth Constraint
    & r[\Strategy_\PlayerIndex]
    & \leq &
        \infty \cdot b[\Strategy_\PlayerIndex] + \epsilon
    & \forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \StrategySet_\PlayerIndex \\\\\

    % Seventh Constraint
    & z
    & \geq &
        \Utility_\PlayerIndex - \infty \cdot y_\PlayerIndex
    & \forall \PlayerIndex \in \SetOfPlayers \\\\

    % Eight Constraint
    & \displaystyle\sum\limits_{\PlayerIndex \in \SetOfPlayers} y_\PlayerIndex
    & = &
        |\SetOfPlayers| - 1
    & \forall \PlayerIndex \in \SetOfPlayers 
\end{array}
\end{equation}

\enrique{The above MILP minimizes $\inf_{\StratProfile \in \epsilon-\textrm{EQ}} \{  \min_{\PlayerIndex} \Utility_\PlayerIndex(\StratProfile)\}$}

\amy{But you can't solve this: $\inf_{\StratProfile \in \StratProfileSpace} \{  \min_{\PlayerIndex} \Utility_\PlayerIndex(\StratProfile) + \Lambda \Regret(\StratProfile) \}$?}

\amy{$\sup_{\StratProfile \in \StratProfileSpace} \Welfare(\StratProfile) - \inf_{\StratProfile \in \textrm{EQ}} \Welfare(\StratProfile)$}
\amy{max min (unrestricted) minus min min over equilibria}

\cyrus{$\sup_{\StratProfile \in \StratProfileSpace} \Welfare(\StratProfile) - \inf_{\StratProfile \in \StratProfileSpace} \{ \Welfare(\StratProfile) + \lambda \Regret(\StratProfile) \}$}

\enrique{$\sup_{\StratProfile \in \StratProfileSpace} \min_{\PlayerIndex} \Utility_{\PlayerIndex}(\StratProfile) - \inf_{\StratProfile \in \StratProfileSpace} \{  \min_{\PlayerIndex} \Utility_\PlayerIndex(\StratProfile) + \lambda \Regret(\StratProfile) \}$}

\enrique{$\sup_{\StratProfile \in \StratProfileSpace} \min_{\PlayerIndex} \Utility_{\PlayerIndex}(\StratProfile) - \inf_{\StratProfile \in \StratProfileSpace} \{  \min_{\PlayerIndex} \Utility_\PlayerIndex(\StratProfile) + \lambda \max_{\PlayerIndex \in \SetOfPlayers} \sup_{\StratProfile'_{\PlayerIndex} \in \StratProfileSpace_{\PlayerIndex}} \Regret_{\PlayerIndex} (\StratProfile_{\PlayerIndex}, \StratProfile'_{\PlayerIndex}, \StratProfile_{-\PlayerIndex}) \}$}

\todo{1. minimize objective, instead of maximize; 2. move from this formulation to the Lagrangian, to make things smooth}

Note that for POA we need the unrestricted egalitarian-maximizing strategy profile in addition to the egalitarian-maximizing state over $\epsilon$-equilibria given by (\ref{eq:mixed-ILP}). I think computing the value of the unrestricted egalitarian-maximizing state either reduces to checking egalitarian value of all pure strategies or is a simple LP. 

Equipped with mixed ILP (\ref{eq:mixed-ILP}) (and a solution to the unrestricted egalitarian-maximizing welfare), we can run experiments as follows

\begin{enumerate}
    \item Draw a poker game, $\GameTuple$. 
    \item Assume that we can compute all exact quantities for $\GameTuple$. \\
    For example, using (\ref{eq:mixed-ILP}) on $\GameTuple$ with $\epsilon = 0$, we can compute the exact egalitarian POA of $\GameTuple$.
    \item Run PSP on $\GameTuple$ and get an estimated game $\hat{\GameTuple}$ that is a  $\epsilon$-uniform approximation of $\GameTuple$.
    \item Run (\ref{eq:mixed-ILP}) on $\hat{\GameTuple}$ with $2\epsilon$.\\
    Now we have POA for $\GameTuple$ and $\hat{\GameTuple}$. At this point we can check whatever POA guarantees we have. What are these?
\end{enumerate}


\subsection{Monte Carlo}

At a high-level, the Monte Carlo approach works as follow

\begin{enumerate}
    \item Draw a poker game, $\GameTuple$. 
    \item Run PSP on $\GameTuple$ and get an estimated game $\hat{\GameTuple}$. 
    \item From $\hat{\GameTuple}$ we can define a distribution over estimated games as follows \enrique{complete this}. 
    \item Run GAMBIT on a game drawn from the above defined distribution. Get a list of equilibria. Record the value of the one with minimum welfare (or whatever objective function, really). 
    \item Repeat and average across all repetitions!
\end{enumerate}


\subsection{Poker Game}

We consider the following 2-player poker game. The game is played using one deck of standard 52-cards. A card has exactly one suit and one rank. A suit is a member of set $\{C, D, H, S\}$, where $C$ stands for Clubs, $D$ for Diamonds, $H$ for Hearts, and $D$ for Spades. A rank is a member of set $\{2, 3, 4, 5, 6, 7, 8, 9, 10, J, Q, K, A\}$, where $J$ stands for Jack, $Q$ for Queen, $K$ for King, and $A$ for ace. A card with suite $X$ and rank $Y$ can be modeled as pair $(X, Y) \in \{C, D, H, S\} \times \{2, 3, 4, 5, 6, 7, 8, 9, 10, J,\allowbreak Q, K, A\}$. A hand consists of five cards from the deck. A random hand consists of 5 randomly chosen cards from the deck. In this game, all cards are selected without replacement. 

The game proceeds as follows. First, each player receives a random hand. After receiving their hands, players must simultaneously discard one card from their hand. Second, one random card is selected out of the remaining 42 cards in the deck. This card then completes a hand with the remaining four cards for each player. Finally, using the standard hand ranking\footnote{\url{https://en.wikipedia.org/wiki/List_of_poker_hands}} the winner with the highest-ranked hand wins and makes a utility of +1 while the other player makes a utility of -1.

We can model a round of this poker game in the language of our work as follows. Fix a hand for each player, say $(C_1^\PlayerIndex, C_2^\PlayerIndex, C_3^\PlayerIndex, C_4^\PlayerIndex, C_5^\PlayerIndex)$ where $C_j^\PlayerIndex$ is the $j$th card of player $\PlayerIndex \in \{1, 2\}$. Player $\PlayerIndex$'s pure strategy set is $\{C_1^\PlayerIndex, C_2^\PlayerIndex, C_3^\PlayerIndex, C_4^\PlayerIndex, C_5^\PlayerIndex\}$, i.e., the player can discard any card in his hand. The set of conditions consists of the cards remaining in the deck after removing the cards from the players' hands. Mathematically, $\ConditionSpace = \{C, D, H, S\} \times \{2, 3, 4, 5, 6, 7, 8, 9, 10, J,\allowbreak Q, K, A\} \setminus \{(C_1^\PlayerIndex, C_2^\PlayerIndex, C_3^\PlayerIndex, C_4^\PlayerIndex, C_5^\PlayerIndex)\}_{i=1,2}$. Note that given a condition $\ConditionValue \in \ConditionSpace$ (i.e., a card from the remaining deck) and the players' hands, each player's utility function is well-defined, as explained above.

Given a distribution $\ConditionDistribution$ over $\ConditionSpace$, we have a well-defined expected normal-form game. A player's expected utility function is given by the expected utility over the remaining deck under distribution $\ConditionDistribution$. As is normal of poker games, we experiment with $\ConditionDistribution$ being the uniform distribution over cards in the remaining deck. For concreteness, the expected utility is given by 

$$
\Expwrt{\ConditionValue \distributed \ConditionDistribution}{\Utility_\PlayerIndex(\StratProfile; \ConditionValue)} = 
\sum\limits_{
y \in 
\{C, D, H, S\} 
\times \{2, 3, 4, 5, 6, 7, 8, 9, 10, J, Q, K, A\} 
\setminus 
\{(C_1^\PlayerIndex, 
C_2^\PlayerIndex, 
C_3^\PlayerIndex, 
C_4^\PlayerIndex, 
C_5^\PlayerIndex)\}_{i=1,2}} 
(-1)^{{\bf 1}[\PlayerIndex \text{ lose}]} Pr[y]
$$

We can now denote by 
$\GameTuple(\{
(C_1^\PlayerIndex, 
C_2^\PlayerIndex, 
C_3^\PlayerIndex, 
C_4^\PlayerIndex, 
C_5^\PlayerIndex)\}_{i=1,2})$ 
the a game where players receive the corresponding hands. Note that there is natural distributions over these game, namely, the uniform distribution over pairs of hands. This distribution would then be our experimental distribution. An experiment would first consist of drawing a game from this experimental distribution and then run PSP with distribution $\ConditionDistribution$ over the remaining deck.




\subsection{Black-box optimization}

For simplicity, let's consider a 2-player.

Player 0 has a set of $n$ pure strategies, $\StrategySet_0 = \{\Strategy_{01}, \Strategy_{02}, \ldots, \Strategy_{0n} \}$.

Player 1 has a set of $m$ pure strategies, $\StrategySet_1 = \{\Strategy_{11}, \Strategy_{12}, \ldots, \Strategy_{1m} \}$. 

Denote by $\vec{\Strategy} = 
\left(
\pi[\Strategy_{0}], 
\pi[\Strategy_{1}]
\right)$ a mixed-strategy profile. 

Our objective function is to minimize $\Regret(\vec{\Strategy})$. Let's write this objective in detail.

\begin{center}
\begin{tabular}{llll}
$\Regret(\vec{\Strategy})$ 
    & = & 
    $\max(  \Regret_0(\vec{\Strategy}), 
            \Regret_1(\vec{\Strategy}) 
        )$ 
    & Definition of regret over all players.\\\\

    & = & 
    $\max\limits_{\PlayerIndex\in \{0, 1\}}\{
            \max\limits_{\pi[\Strategy'_{\PlayerIndex}]}
                \Utility_\PlayerIndex(\pi[\Strategy'_{\PlayerIndex}], \pi[\Strategy_{(1-\PlayerIndex)}])
            -
            \Utility_\PlayerIndex(\vec{\Strategy})
        \}$ 
    & Definition of regret of a player at $\vec{\Strategy}$.\\\\
\end{tabular}
\end{center}

This objective requires solving two inner optimization problems, one for each players' best response fixing the other player's mix. We can simplify that inner optimization problem by observing that, given a fixed mix of a player, the other player's best response set contains a pure strategy. Thus, the inner optimization problem reduces to a lookup among pure strategies instead of a linear program over mixed strategies. 

Abusing notation, we write $\Strategy_{ij}$ for the degenerate mix where the $i$th player plays its $j$th strategy.
The full objective function is then,

$$\Regret(\vec{\Strategy}) = 
\max\{
        \max\limits_{0 \le j \le n}
            \Utility_0(\Strategy_{0j}, \pi[\Strategy_{1}]) 
        -
            \Utility_0(\vec{\Strategy}), \quad 
        \max\limits_{0 \le j \le m}
            \Utility_1(\Strategy_{1j}, \pi[\Strategy_{0}])
        -
        \Utility_1(\vec{\Strategy})
\}
$$

Our optimization problem is then,

$$
\min\limits_{\vec{\Strategy}} 
\max\{
        \max\limits_{0 \le j \le n}
            \Utility_0(\Strategy_{0j}, \pi[\Strategy_{1}]) 
        -
            \Utility_0(\vec{\Strategy}), \quad 
        \max\limits_{0 \le j \le m}
            \Utility_1(\Strategy_{1j}, \pi[\Strategy_{0}])
        -
        \Utility_1(\vec{\Strategy})
\}
$$

\subsection{Sanity Check Experiments}

A first sanity check is to compute equilibria by minimizing regret using a black-box optimizer. 
I implemented prisoner's dilemma and then used a Bayesian optimizer from skopt's library to minimize the above objective. Bayesian optimization is usually unconstrained, an this is the case in skopt. Thus, I introduce penalties from deviation from valid probability distributions in the objective function. 

Over 100 runs of the optimizer with EI acquisition function, 50 calls to the optimizer and 10 random restart, the optimizer always but once found the unique equilibrium. For BoS, the result was similar, but the solver failed a bit more often and sometimes found one pure Nash, and sometimes the other. The solver never found the mixed Nash. 

However, for rock, paper, scissors, the solver never found the unique mixed Nash, and only sometimes did it get close to it. I am not very optimistic this approach would work for our experiments. 

Update: after a bit more hyper-parameter optimization (i.e., by hand trying different parameters of the solver), slightly better results occur. But, the task becomes computationally taxing, which is not surprising. 

==> expts/ppoa_expts.tex <==
\subsection{Pure Price of Anarchy Experiments}

\amy{Goals of the exp'ts
\begin{itemize}
\item to test the naive, unbounded estimator. is it really unbounded in practice?
\item which naive estimator? should we use $0$-Nash in the denominator, or $2\epsilon$-Nash. if we use the latter, eqa are guaranteed to exist. but  either denominator could still be very very small (or 0), b/c welfare could be very very small (or 0).
\item so maybe try both estimators, and then count how many times the denominator is zero b/c either 1. there are no eqa, vs.\ 2. how many times welfare is just too small. and: \emph{try to design env'ts where welfare won't be too small --- Enrique claims to have already done this}
\item something else we discussed trying was: measuring $\gamma$ -- the distance b/n the welfare of the set of eqa of the true game and that of the $4\epsilon$-eqa of the estimated game. we can then use the tighter bound of the conditional anarchy theorem.
\end{itemize}
}

The goal of this section is to show how to use the machinery developed in this paper to estimate the \emph{pure\/} price of anarchy.
The \mydef{pure price of anarchy} is defined by restricting both the numerator and denominator in definition of the price of anarchy to only pure strategies.
Formally,

\begin{definition}[The Pure Price of Anarchy]
Given game $\GameTuple$ with utility function $\Utility$, the \mydef{pure price of anarchy} (PPOA) is defined as $\AnarchyRatio (\GameTuple) \doteq \frac{\max_{\StratProfile' \in \StratProfileSpace} \Welfare (\Utility, \StratProfile')}{\min_{\StratProfile \in \Nash(\GameTuple)} \Welfare (\Utility, \StratProfile)}$.
\label{def:purePOA}
\end{definition}

\enrique{I will try to set up the experiments so that we avoid division by zero, for example, by having welfare much greater than $\epsilon$}. 

Henceforth, we assume that the ground-truth game $\GameTuple$ has at least one pure Nash equilibrium. By Theorem~\ref{thm:poa}, this assumption implies that any $\epsilon$-uniform approximation $\GameTuple'$ of $\GameTuple$ has at least one pure $2\epsilon$-Nash equilibrium. 

Fix a game $\GameTuple$. Given a sequence of $\epsilon$-uniform approximations $\{\GameTuple'_j\}_{j=1}^k$ 
%= \GameTuple'_1, \GameTuple'_2, \ldots, \GameTuple'_k$
of $\GameTuple$,
we construct the following empirical estimators\amy{Monte Carlo estimates?} of the bounds in Theorem~\ref{thm:poa}.  

\begin{enumerate}
    \item For the lower bound Equation~\ref{eq:POANaiveBounds}:
    \begin{eqnarray}
        L(\GameTuple) = \frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile) - \NumberOfPlayers\epsilon}{\max_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple)} \Welfare (\Utility, \StratProfile) + \NumberOfPlayers\epsilon};
        &
        \hat{L}(\{\GameTuple'_j\}_{j=1}^k) = \dfrac{1}{k}\mathlarger{\sum_{j=1}^k}\frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility'_j, \StratProfile) - \NumberOfPlayers\epsilon}{\max_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple'_j)} \Welfare (\Utility'_j, \StratProfile) + \NumberOfPlayers\epsilon} 
        \label{eq:empiricalLowerBound}
    \end{eqnarray}
    
    \item For the upper bound Equation~\ref{eq:POANaiveBounds}:
    \begin{eqnarray}
        U(\GameTuple) = \frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile) + \NumberOfPlayers\epsilon}{\min_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple)} \Welfare (\Utility, \StratProfile) -\NumberOfPlayers\epsilon}; &
        \hat{U}(\{\GameTuple'_j\}_{j=1}^k) = \dfrac{1}{k}\mathlarger{\sum_{j=1}^k}\frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility'_j, \StratProfile) + \NumberOfPlayers\epsilon}{\min_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple'_j)} \Welfare (\Utility'_j, \StratProfile) -\NumberOfPlayers\epsilon} 
        \label{eq:empiricalUpperBound}
    \end{eqnarray} 
    
    \item For the upper bound Equation~\ref{eq:POABetterBounds}:
    \amy{Enrique, please complete!!!}
    
    \item For the PPOA, for $x > 0$,
    %we use a family of estimators, $M_x(\GameTuple)$, defined as follows:
    \enrique{So far I have only experimented with $x \in \{0, 2\epsilon\}$}
    \amy{is there any theory about these estimators, when $x > 0$? like Eq'n 1 with $4x$ if your estimator uses $2x$?}
%    
    \begin{eqnarray}
        M_x (\GameTuple) = \frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile)}{\min_{\StratProfile \in \Nash_{x}(\GameTuple)} \Welfare (\Utility, \StratProfile)}; &
        \hat{M}_x (\{\GameTuple'_j\}_{j=1}^k) = \dfrac{1}{k}\mathlarger{\sum_{j=1}^k} \frac{\max_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility'_j, \StratProfile)}{\min_{\StratProfile \in \Nash_{x} (\GameTuple'_j)} \Welfare (\Utility'_j, \StratProfile)}
        \label{eq:empiricalMean}
    \end{eqnarray}

\end{enumerate}

==> finite-congestion-games.tex <==
\section{Finite Congestion Model}
%
A {\it finite congestion game}~\cite{christodoulou2005price} is a tuple $\CongestionGame = (\SetOfPlayers, \SetOfFacilities, (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}, (\FacilityCostFunction)_{\FacilityIndex\in\SetOfFacilities})$,
where $\SetOfPlayers = \{1, \ldots, \NumberOfPlayers\}$ is a set of players, $\SetOfFacilities = \{1, \ldots, \NumberOfFacilities\}$ is a set of facilities,
$(\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers} \subseteq 2^\NumberOfFacilities$ is the set of pure strategies for player $\PlayerIndex$. A strategy $\Strategy_\PlayerIndex \in \SetOfStrategies_\PlayerIndex$ is a set of facilities. Finally, $\FacilityCostFunction_\FacilityIndex$ is a cost function associated with facility $\FacilityIndex$.

A pure strategy profile $\Strategy = (\Strategy_1, \ldots, \Strategy_\NumberOfPlayers)$ is a vector of strategies, one for each player. In a finite congestion game, each player selects a strategy so as to minimize their costs. Given a profile of strategies $\Strategy$, the cost for player $\PlayerIndex$ for $\Strategy$ is defines as $\PlayerCost_\PlayerIndex(\Strategy) = \sum_{\FacilityIndex\in\Strategy_\PlayerIndex} \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex(\Strategy))$, where $\NumberOfPlayers_\FacilityIndex(\Strategy)$ is the number of players selecting facility $\FacilityIndex$ in $\Strategy$.

A {\it pure strategy profile} is a Nash equilibrium if no player has an incentive to unilaterally deviate to another pure strategy. Mathematically, $\Strategy^*$ is a pure Nash equilibirum if $\forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \SetOfStrategies_\PlayerIndex: \PlayerCost_\PlayerIndex(\Strategy^*) \le \PlayerCost_\PlayerIndex(\Strategy^*_{-\PlayerIndex}, \Strategy_\PlayerIndex)$, where $(\Strategy^*_{-\PlayerIndex}, \Strategy_\PlayerIndex)$ is the strategy profile obtained if just player $\PlayerIndex$ deviates from $\Strategy^*_\PlayerIndex$ in $\Strategy^*$. 
In~\cite{rosenthal1973class} it was shown that this class of games have at least one pure Nash equilibria provided that each facility's cost function $\FacilityCostFunction_\FacilityIndex$ is a function of the number of players selecting that facility only, i.e., $\FacilityCostFunction_\FacilityIndex = \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex)$.

The {\it system's cost} of strategy $\Strategy$ is defined as the sum of the cost incurred by each player in $\Strategy$ which we denote by $\SystemCost(\Strategy) = \sum_{\PlayerIndex\in\SetOfPlayers} \PlayerCost_\PlayerIndex(\Strategy)$. The optimal system's cost is defined as $\SystemCost^* = \min\limits_{\Strategy \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}} \SystemCost(\Strategy)$
%
\section{Price of Anarchy}
%
The ratio between the worst possible system's cost of a Nash equilibrium (in mixed or pure strategies) and the optimum system's cost was first proposed in \cite{koutsoupias1999worst} as a measure of the effectiveness of a system and later dubbed the {\it price of anarchy}~\cite{papadimitriou2001algorithms,roughgarden2002bad}. Since congestion games always have a pure Nash equilibrium, is natural to investigate the {\it pure price of anarchy} (PPA) where one considers only Nash equilibria in pure strategy in this class of games. Mathematically, the PPA of a finite congestion game $\PurePriceOfAnarchy(\CongestionGame)$ is defined as follows.
%
\begin{definition}[The pure price of anarchy (PPA)]
Let $\CongestionGame$ be a congestion game (in general, any game for which pure Nash equilibria is guaranteed to exists). 
We denote the pure price of anarchy (PPA) of $\CongestionGame$ by $\PurePriceOfAnarchy(\CongestionGame)$ and define it as:
\begin{equation}
    \PurePriceOfAnarchy(\CongestionGame) = \dfrac{\max\limits_{\{\Strategy^* \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}
                                                \mid \Strategy^* \text{ is a pure Nash equilibrium}\}} \SystemCost(\Strategy^*)}
                                             {\SystemCost^*}
\label{eq:PPA}
\end{equation}
\label{def:PPA}
\end{definition}
%
Most known theoretical results for pure price of anarchy in finite congestion games make strong assumptions about the functional form of $\FacilityCostFunction_\FacilityIndex$. For example, authors in~\cite{christodoulou2005price} showed that when $\FacilityCostFunction_\FacilityIndex(k) = k$, the PPA is 5/2.
%
\begin{example}
Consider the following example of a finite congestion game due to~\cite{christodoulou2005price}. There are 3 players and 6 facilities. Partition the set of facilities in two, $\SetOfFacilities_1 = \{h_1, h_2, h_3\}$ and $\SetOfFacilities_2 = \{g_1, g_2, g_3\}$. Each player has two strategies: $\SetOfStrategies_1 = \{\{h_1, g_1\}, \{g_2, h_3, h_2\}\}, $
$\SetOfStrategies_2 = \{\{h_2, g_2\}, \{g_2, h_3, h_2\}\},$ and
$\SetOfStrategies_1 = \{\{h_3, g_3\}, \{g_1, h_2, h_1\}\}$. If the cost of facilities is given by $\FacilityCostFunction_\FacilityIndex(k) = k$ for all $\FacilityIndex \in \SetOfFacilities_1 \cup \SetOfFacilities_2$, then one can verify that the profiles of strategies $\Strategy_1 = (\{h_1, g_1\}, \{h_2, g_2\}, \{h_3, g_3\})$ and $\Strategy_2 = (\{g_2, h_3, h_2\}, \{g_2, h_3, h_2\}, \{g_1, h_2, h_1\})$ are both Nash equilibria. In this case, $\Strategy_1$ is the social optimum with $\SystemCost(\Strategy_1) = 3 \cdot 2$ while $\SystemCost(\Strategy_2)=3 \cdot 5$. Note that this implies a PPA of 5/2.
\label{ex:PPA}
\end{example}
%
\subsection{The $\epsilon$-Pure Price of Anarchy}
Since we are interested in solving games that are too complex to be amenable to analytical solutions, we define a notion of $\epsilon$-price of anarchy which is amenable to estimation from data. 
%Before defining it, we need to define the measure of a cost of a syn. 
%
\begin{definition}[The $\epsilon$-pure price of anarchy ($\epsilon$-PPA)]
%
Let $\epsilon > 0$ and $\CongestionGame$ be a congestion game (in general, any game). 
%Let $\SystemCost_\epsilon = \{\Strategy \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers} \mid \SystemCost(\Strategy) \le \SystemCost^* + \epsilon\}$, i.e., the set of all strategy profiles whose cost is within $\epsilon$ of the cost of the system's cost minimizing strategy. 
We define the $\epsilon$-pure price of anarchy as the following ratio
\begin{equation}
    \PurePriceOfAnarchy_\epsilon(\CongestionGame) = 
    \dfrac
{\max\limits_{\{\mathbb{\Strategy^*} \mid \mathbb{\Strategy^*} \text{is an $\epsilon$-sink equilibrium}\}} \SystemCost(\mathbb{\Strategy^*})}
{\min\limits_{\{\mathbb{\Strategy^*} \mid \mathbb{\Strategy^*} \text{is an $\epsilon$-sink equilibrium of the UM graph}\}} \SystemCost(\mathbb{\Strategy^*})}
        %{\min\limits_{\Strategy \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}} \SystemCost(\Strategy)}
\label{eq:epsPPA}
\end{equation}
\label{def:epsPPA}
\end{definition}
Note that we overload notation and used $\SystemCost(\mathbb{\Strategy})$ to denote the cost of sink $\mathbb{\Strategy} = \{\Strategy_1, \ldots, \Strategy_k\}$. We still need to define exactly which metric we care about for a sink, e.g., average cost would be $\SystemCost(\mathbb{\Strategy}) = \SystemCost(\{\Strategy_1, \ldots, \Strategy_k\}) = \dfrac{1}{k}\sum_{l=1}^k \SystemCost(\Strategy_l)$. (Note to self, for $\epsilon$ large enough, $\PurePriceOfAnarchy_\epsilon$ is always 1).

A few more comments about Definition~\ref{def:epsPPA}. Note that in the numerator we consider the worst possible {\it $\epsilon$-sink equilibrium} instead of the worst possible $\epsilon$-pure Nash as we did for Definition~\ref{def:PPA} (formal definition of $\epsilon$-sink equilibria pending but in a nutshell: a sink of the $\epsilon$-best response graph is an $\epsilon$-sink equilibrium). 
The reason is simple: once we relax the Nash solution concept to $\epsilon$-Nash, 
\amy{this makes no sense; relaxing a definition cannot make existence go away. existence must fail for some other reason, such as noisy payoffs.}
we no longer have a guarantee of existence in pure strategies, even for congestion games. Consequently, we instead consider sink equilibria, which is the natural generalization of pure Nash equilibria, but of course, up to an $\epsilon$ error. 

Using our current tools, we can estimate both numerator and denominator. Note, however, that we can estimate the numerator with probability at least $1 - \delta_n$ and denominator with probability $1 - \delta_d$. Consequently, we can estimate the ratio with probability $(1-\delta_n)(1-\delta_d)$.


\section{Mechanism Design}
%
Suppose now we take the role of a {\it mechanism designer} trying to modify the rules of a finite congestion game so as to minimize the overall congestion across all players. Suppose we have access to players' preferences (understood here as the set of strategies $(\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}$) but we are not allowed to change them as these are set by the players a priori. Instead, as the designers, we can only change the cost functions for different facilities. In this case, we next illustrate, in the context of example~\ref{ex:PPA}, how one can chose cost functions so as to minimize the price of anarchy.

{\it {\bf Remark}: Note that as currently formulated, we don't believe this example makes a lot of sense. The problem that we have is that the denominator in the calculation of PPA -equation~(\ref{eq:PPA})- is not fixed but may vary as a function of the cost of the facilities. In particular, note how in the new game we have a higher cost in the optimal system's cost than in the optimal system's cost of the original game but still a lower system's cost than in the bad Nash of the original game. This means that we have sacrificed a potential lower overall cost for a higher cost that is more likely to be played. In other words, we have reduced the price of anarchy but in the process we have change the value of the optimal solution, something we believe to be an undesirable property.}
%
\begin{example} 
Let us consider the following variation of example~\ref{ex:PPA}. If we define  $\FacilityCostFunction_g(k) = k$ for $g \in \SetOfFacilities_1$ and
$\FacilityCostFunction_h(k) = 2k$ for $h \in \SetOfFacilities_2$, then in the ensuing game strategy $\Strategy_1$ will be the unique pure Nash equilibrium. Moreover, the unique pure Nash will coincide with the optimal system's cost, i.e., the strategy profile with minimum overall cost. Note that in this case the PPA is 1.

This example illustrates the possibility of using mechanism design to select the parameters of the game (in the above example, the facilities' cost functions where we restrict to select only their slope) to optimize a designers' objective function (in the example, the PPA). \end{example}
%
\section{Experiments}
%
In this section, we investigate the empirical performance of our algorithms. 
\subsection{Experimental Setup}
%
We experiment with a distribution of random, finite congestion games which we call $RFC(\NumberOfPlayers, \NumberOfFacilities)$ consisting of games $\CongestionGame$ with $\NumberOfPlayers$ players and $\NumberOfFacilities$ facilities. The cost for player $i$ is defined as 
$\PlayerCost_\PlayerIndex(\Strategy) = \sum_{\FacilityIndex\in\Strategy_\PlayerIndex} \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex(\Strategy)) + \xi$ where $\xi$ is a random noise.
\amy{why is there random noise? cost can't be defined this way, unless we are okay giving up existence of PNE.}

What remains to model are (1) the topology of preferred strategies for each player (these should model some interesting situation), and (2) the form of the facilities' costs and the form of the noise (note that we know that only for simple form of facilities' costs we have bounds on the PPA). 

The following are proposals for both (1) and (2).

\subsubsection{Players' preferences}
I propose we test the following topologies for players' preferences. 

\underline{Power Law}: under this topology, each player $\PlayerIndex$ has a random number of pure strategies $n_\PlayerIndex \sim U[a, b]$ where $a < b \in \{1,\ldots, 10\}$. Note that $n_\PlayerIndex \le 2^{\NumberOfFacilities}-1$. Each pure strategy  $\Strategy_{\PlayerIndex, k}$, where $k \in \{1, \ldots, n_\PlayerIndex\}$ is constructed as follow. The probability that facility $j \in \{1, \ldots, \NumberOfFacilities\}$ is in $\Strategy_{\PlayerIndex, k}$ is given by a simple power law $p[j \in \Strategy_\PlayerIndex] = \alpha^{-j}$, where $\alpha \in [0,1]$ is a free parameter. Note that we have the option of enforcing a hard requirement of $n_\PlayerIndex$ strategies, or we may allow strategy repetitions in which case $n_\PlayerIndex$ is just an upper bound on the number of strategies for player $\PlayerIndex$. 

The interpretation of $\alpha$ is that for higher (lower) values of $\alpha$ we model a system with a more (less) diverse set of preferred facilities. In this model, we chose facilities independent of each other. This model then correspond to a situation where there is a clearly preferred facility, e.g., a very busy metro station, and other less preferred facilities, e.g., stations at the outskirts of a city. 

However, a more interesting/complex model would be one where the probability of selecting a facility is influenced by the probabilities of other facilities (for example, to go back home from work in the metro, one may need to change stations and thus, stations that are close to each other in certain paths are preferable). In this case, one could have an underlying graph (e.g., map of Tokyo metro) of preferences (can we use CATS for this?). 

\subsubsection{Noise}
We could start with simple Gaussian noise $\xi \sim \mathcal{N}(\mu, \sigma)$ for suitable choices of $\mu, \sigma$, and/or uniform noise $\xi \sim U(c, d)$ for suitable choices of $c < d$. However, since congestion games as described in this document are finite and discrete, I find it hard to interpret continuous noise in this model. An alternative is to introduce discrete noise, for example, by using a geometric distribution. This last noise model the situation where we can't measure exactly the number of people selecting a facility but instead can only have an integer approximation.
%
\subsection{Metrics}
%
We need metrics for at least:
\begin{enumerate}
    \item Sample complexity (e.g., how many samples as a function of $\epsilon,\delta$)
    \item System's cost (and maybe individuals' costs)
    \item Accuracy of outcomes, if ground-truth is known (e.g., for instances where we know (or have bounds on) the PPA). How long and how many samples does it take to get the right answer?
    \item Time complexity.
    \item Proportion of outcomes where the algorithm fails (an empirical measure of $\delta$).
\end{enumerate}

==> future_work.tex <==
\paragraph{Future experimental work}
Thus far, we have only experimented with learning pure strategy $\epsilon$-Nash equilibria.
%, choosing congestion games as a test environment explicitly for this purpose. 
Our experiments are small enough that we can use exhaustive search to determine ground truth. Computing mixed strategy Nash equilibria is intractable (PPAD-complete)~\cite{daskalakis2009complexity};
%, and even approximating them is difficult\amy{insert a citation on attempts to approximate mixed Nash};
accordingly, estimating them remains a challenge. 

%\cyrus{We could note here that in b/n pruning criteria, such as pruning by strategy profile when \emph{all\/} players have high regret, or pruning dominated strategies noniteratively, also work.}

Having said that, a potentially interesting statistical vs.\ computational trade-off exists that warrants further investigation 
when the goal is to estimate mixed strategy equilibria.  While fully computing $\Rationalizable_{\epsilon}(\GameTuple)$ may incur \emph{statistical\/} savings by avoiding sampling profiles that are deemed %dominated
non-equilibria early on, iteratively computing $\Rationalizable_{\epsilon}(\GameTuple)$ comes at a \emph{computational\/} cost.
%should we spend computational resources to compute $\Rationalizable_{\epsilon}(\GameTuple)$ to achieve statistical savings, or settle for noniteratively removing $\epsilon$-dominated strategies, thereby incurring a lower computational and higher statistical cost?

\begin{comment}
\amy{i believe this next paragraph (on pure strategy eqa) should be deleted.}
In the pure strategy equilibrium case, there are also potentially interesting tradeoffs to explore.  Eliminating strategy profiles at which \emph{any\/} agent exhibits regret, as we do, may incur some statistical savings by avoiding sampling player-strategy profile combinations that can be deemed irrelevant early on. However, eliminating strategy profiles only when multiple agents exhibit regret might also incur statistical savings\amy{how???} by leading to earlier pruning of adjacent profiles that would not have been pruned otherwise.  Heuristics for the detection of these combinations is an interesting future research direction.
%\enrique{there is a combinatorial problem embedded here. Which combination of player's utilities should we look at when deciding to prune a strategy? this is a function of a profile and its neighbors, where we look at the same combination for adjacent profiles.}
\end{comment}

The experiments we have run thus far, in simple, synthetic environments, were designed to illustrate the advantage of our algorithms in a controlled setting. In future work, we plan to study more complicated games, including large enough games so that bounds that are game-size dependent---such as those that require correction procedures, cf.\ \Cref{thm:Hoeffding}---are statistically intractable. Since our algorithms are agnostic to the noise distribution, we will also test their robustness to other forms of noise, such as multiplicative and unbounded noise.
%assuming a subgaussian and related assumptions.

==> gini.tex <==

\newcommand{\lv}{\bm{}}
\newcommand{\pv}{\bm{p}}

\paragraph{Gini Social Welfare}
We now define the \emph{generalized Gini social welfare function} (GGF).  [as used by \citep{siddique2020learning}]

\begin{definition}[The Generalized Gini Mean \citep{weymark1981generalized}]
Suppose a \emph{sentiment vector} $\lv \in \R^{\NumberOfPlayers}$ and \emph{decreasing stochastic weights vector} $\pv \in [0, 1]^{\NumberOfPlayers}$ (i.e., $1 \geq \pv_{1} \geq \pv_{2} \geq \dots \geq \pv_{\NumberOfPlayers} \geq 0$ and $\norm{\pv}_{1} = 1$), %\citet{weymark1981generalized} defines
the \emph{generalized Gini social welfare function} (GGF) is
\[
\Gini_{\pv}(\lv) \doteq \sum_{i=1}^{\NumberOfPlayers} \pv_{i}%^{\downarrow}
\lv_{i}^{\uparrow}
\enspace,
\]
where $\lv^{\uparrow}$ denotes the terms of $\lv$ in \emph{ascending sorted order}.
\end{definition}

The weights vector $\pv$ control the trade-off between the importances of well-off and impoverished agents, and we recover \emph{utilitarian} welfare with $\pv = (\frac{1}{\NumberOfPlayers}, \frac{1}{\NumberOfPlayers}, \dots, \frac{1}{\NumberOfPlayers})$, and \emph{egalitarian} welfare with $\pv = (0, \dots, 0, 1)$.

\if 0
The requirement of increasing $\pv$ is intimately tied to fairness, as it ensures more weight is placed on is both \emph{necessary} and \emph{sufficient} for the GGF to satisfy the Pigou-Dalton principle.
We may immediately extend the concept to malfare by reversing this constraint, requiring instead that $\pv$ be \emph{increasing}, i.e., $0 \leq \pv_{1} \leq \pv_{2} \leq \dots \leq \pv_{\NumberOfPlayers} \leq 1$.
Here the importance placed on groups \emph{increases} with their rank, which is both necessary and sufficient for the \emph{anti Pigou-Dalton principle} (\cref{def:cardinal-axioms} axiom \ref{def:cardinal-axioms:apd}), where the egalitarian case is again the most extreme, characterized by $\pv = (1, 0, \dots, 0)$.

Note that it is equally valid to define the GGF malfare in terms of descending $\lv^{\downarrow}$, i.e.,
\[
\Gini_{\pv}(\lv) \doteq \sum_{i=1}^{\NumberOfPlayers} \pv_{i}%^{\downarrow}
 \lv_{i}^{\downarrow}
 \enspace,
\]
in which case the decreasingness constraint on $\pv$ is the same for welfare and malfare.
We prefer the former definition, as the algebraic form of the malfare and welfare GGF is identical (as with the power-mean), and then the choice of welfare or malfare (PD or APD axiom) generates \emph{constraints} on $\pv$.
Furthering this aesthetic pleasure is the fact that for both the power-mean and GGF, the utilitarian $p$ (respectively, $\pv$) coincide for welfare and malfare, and the egalitarian $p$ (respectively, $\pv$) attain an elegant symmetry of negation (respectively, reversal).
\fi

\amy{End of the Generalized Gini Social Welfare Function!}


==> ijcai_abstract.tex <==
\begin{abstract}
We tackle a fundamental problem in empirical game-theoretic analysis (EGTA), that of learning equilibria in simulation-based games.
Such games cannot be described in analytical form; instead, a black-box simulator can be queried to obtain noisy samples of utilities.
Our approach to EGTA is in the spirit of probably approximately correct (PAC) learning. 
We design algorithms that learn so-called empirical games, which uniformly approximate the utilities of simulation-based games from finitely many samples.
These algorithms can be instantiated with various concentration inequalities.
Building on earlier work, we first apply Hoeffding's bound, but as the size of the game grows, this bound eventually becomes statistically intractable; hence, we also use the Rademacher complexity.
Our main theorem states: with high probability, all equilibria of the simulation-based game are approximate equilibria in the empirical game (perfect recall); and conversely, all approximate equilibria in the empirical game are approximate equilibria in the simulation-based game (approximate precision).
We evaluate the performance of our algorithms on several synthetic games, showing that they are robust to different forms of noise, make frugal use of data, and produce accurate estimates more often than the theory predicts.
\end{abstract}

==> introduction.tex <==
%\cyrus{We prove properties about approximations, and show that some things are possible with approximations, which implies they are possible with high probability using estimates.}

\section{Introduction}
\label{sec:intro}

Game theory is the \emph{de facto\/} standard conceptual framework used to analyze the strategic interactions among 
%independent and 
rational agents in multi-agent systems. At the heart of this framework is the theoretical notion of a game. In a game, each player (henceforth, an agent) chooses a strategy 
%from a set of strategies 
and earns a utility that in general depends on the profile (i.e., vector) of strategies chosen by all the agents.

%Mathematically, any finite\amy{why finite?}\enrique{I don't think infinite games have normal-form representation which is what this sentence is getting at} game can be represented by its \mydef{normal-form}, 
The most basic representation of a game is the \mydef{normal form}, which can be visualized as a matrix containing all agents' utilities at all strategy profiles.
There are many techniques available to analyze normal-form games.
Analyzing a game means predicting its outcome, i.e., the strategy profiles that one can reasonably expect the agents to play.
Perhaps the most common such prediction
%in the well-studied class of non-cooperative games 
is that of \mydef{Nash equilibrium}~\citep{nash1950equilibrium}, where each agent plays a \mydef{best-response} to the strategies of the others: i.e., a strategy that maximizes their utility.
More generally, at an $\epsilon$-Nash equilibrium agents best respond to other agents' strategies up to an additive error of $\epsilon$.
%In other words, in an $\epsilon$-Nash equilibrium, agents tolerate forgoing up to $\epsilon$ of the payoffs they could have achieved by choosing an alternative strategy. 
%This relaxation is natural; setting $\epsilon$ to zero recovers the classic formulation of Nash equilibrium.

This paper is concerned with analyzing games for which a complete and accurate description is not available.
While knowledge of the number of agents and their respective strategy sets is available, we do not assume {\it a priori} access to the game's utility function.
Instead, we assume access to a 
%black-box \amy{could be white-box. why not?}
simulator from which we can sample noisy utilities associated with any strategy profile.
Such games have been called \mydef{simulation-based games}~\citep{vorobeychik2008stochastic} and
\mydef{black-box games}~\citep{picheny2016bayesian},
and their analysis is called \mydef{empirical game theoretic analysis} (EGTA)~\citep{wellman2006methods,jordan2007empirical}.
EGTA methodology has been applied in a variety of practical settings for which simulators are readily available, including trading agent analyses in supply chain management~\citep{vorobeychik2006empirical,jordan2007empirical}, ad auctions~\citep{jordan2010designing}, and
energy markets~\citep{ketter2013autonomous};
designing network routing protocols~\citep{wellman2013analyzing}; strategy selection in real-time games~\citep{tavares2016rock}; and the dynamics of reinforcement learning algorithms, such as AlphaGo \citep{tuyls2020bounds}.
%\amy{btw, what are real-time games?}
%\enrique{games where strategies can be changed in real-time}.

The aim of this work is to design learning algorithms that can generate an estimate $\hat{Y}$ of a game-theoretic property $Y \in \mathcal{Y}$ of a simulation-based game $\GameTuple$, with a guarantee $\norm{Y - \hat{Y}}_{\mathcal{Y}} \leq \epsilon$ w.h.p., where $\norm{\cdot}_{\mathcal{Y}}$ is some norm 
%used to measure error
over the space of properties $\mathcal{Y}$.
%
\cyrus{It may have been a mistake to measure error with $\norm{Y - \hat{Y}}_{\mathcal{Y}}$.  Initially, this was the obvious choice, because when $\mathcal{Y}$ is the space of utility functions (or games), we can measure error with $\norm{\cdot}_\infty$.  However, in the perfect-precision and perfect-recall cases, there's asymmetry, we then have some asymmetry, as we need to ensure $Y \subseteq \hat{Y}$, and given that, our error metric is based on the most incorrect member of $\hat{Y}$.  I think the fix is to define an error measurement as a function, rather than a norm.  I don't really know what to call this; it's roughly analogous to a loss function, but I'm open to ideas.}
We tackle this problem using the \mydef{probably approximately correct} (PAC) learning framework~\citep{valiant1984theory}.
Our algorithms learn so-called \mydef{empirical games}~\citep{wellman2006methods}, which are estimates of simulation-based games constructed via sampling.
We argue that empirical games so constructed yield \mydef{uniform approximations} of simulation-based games, meaning all utilities in the empirical game tend toward their expected counterparts,
%in the simulation-based game,
\emph{simultaneously}.

This notion of uniform approximation is central to our work: we prove that several game-theoretic properties are Lipschitz continuous in utilities, and hence can be accurately estimated, given only a uniform approximation.  
\amy{We call such properties ``smooth.'' (or regular, or something).}
Most notable among the \amy{regular} properties is the set of equilibria of a game: when one game $\GameTuple'$ is a uniform approximation of another $\GameTuple''$, all equilibria in $\GameTuple'$ are approximate equilibria in $\GameTuple''$~\citep{tuyls2020bounds}
\amy{insert reference to AAMAS paper + EA}.
\amy{Other examples of smooth properties include: \ldots}
Our learning algorithms, which learn empirical games that are uniform approximations of simulation-based games well estimate \emph{all\/} \amy{smooth} properties of the latter.

When a game estimate $\hat{\GameTuple}$ uniformly approximates a (true) game $\GameTuple$, all equilibria in $\GameTuple$ are approximate equilibria in $\hat{\GameTuple}$, and all equilibria in $\hat{\GameTuple}$ are approximate equilibria in $\GameTuple$.
As a result, a uniform approximation implies perfect recall,%
\footnote{We use the term \mydef{recall}
in the information retrieval sense. The juxtaposition of the two words ``perfect'' and ``recall'' is not a reference to extensive-form games.} as \emph{all\/} true positives---equilibria in $\GameTuple$---are at least approximate equilibria in $\hat{\GameTuple}$; and \emph{approximately\/} perfect precision, as all false positives---equilibria in $\hat{\GameTuple}$ but not necessarily in $\GameTuple$---are at least approximate equilibria in $\GameTuple$.
%Related past work focused either on estimating a single equilibrium (e.g.,~\citep{jordan2008searching}), or only on establishing perfect recall~\citep{tuyls2020bounds}.
As our learning algorithms, well estimate all \amy{smooth} properties of simulation-based games, we generalize known perfect-recall/approximately perfect-precision results~\citep{tuyls2020bounds} \amy{insert reference to AAMAS paper + EA} beyond just the set of equilibria.

%Our learning algorithms can be instantiated with various concentration inequalities,
%%to handle different types of games, 
%and do not in general assume asymptotic normality.  Our results instead depend on showing that all (or multiple)
%%estimated 
%utilities in the empirical game tend toward the expected utilities in the simulation-based game,
%%their expectations,
%simultaneously.  Generic univariate concentration inequalities like Hoeffding's only handle one value at a time; we thus apply a union bound to handle the multiple hypothesis testing that arises when estimating a game.  For very large games, this approach becomes statistically intractable, so we also present an alternative technique using Rademacher averages that simultaneously bounds all the utilities in an empirical game.
%%about their expectations.  
%These latter bounds are data-dependent, but are never more than a constant-factor looser (additively) than the 
%%Hoeffding + union bound 
%former.  Furthermore, in some cases, such as when utilities are correlated,
%%\amy{i am tring to avoid the use of the term ``expectations''}
%%or when they are tightly concentrated about their expectations,
%these latter bounds can vastly outperform the former.
%\amy{Cyrus, please replace this last sentence as necessary w/ a new one summarizing your new discussion of how the bounds grow in factored games.}

Following~\citep{AAMAS paper}, we develop a pruning algorithm that samples ``progressively,'' meaning dynamically, as information about the game unfolds (due to additional calls to the simulator).
%iteratively pruning strategies along the way, and thereby has the potential to expedite learning by obtaining tighter bounds than \GS, given the same number of samples.
%


\PSP{} is a meta-algorithm, parameterized by a game-theoretic property and a corresponding pruning criterion that only prunes strategy profiles that are provably irrelevant to accurately learning the property of interest.
%
Prior art~\citep{elomaa2002progressive,riondato2015mining, riondato2018abra} uses progressive sampling to obtain a desired accuracy at a fixed failure probability by guessing an initial sample size, computing Rademacher bounds, and repeating with larger sample sizes until the desired accuracy is attained.
Our work enhances this strategy with \emph{pruning}: at each iteration, parameters that have already been sufficiently well estimated for the task at hand (here, equilibrium estimation) are pruned, so that subsequent iterations of \PSP{} do not refine their bounds.  

Although we consider only classical MCP correction methods,
pruning is also compatible with more modern techniques, such as Rademacher complexity.
%the former: explicitly obtain tighter confidence intervals as the number of parameters decreases
%the latter: depend on the parameters being estimated (though in a subtler manner than classical methods)
%the Rademacher averages grow monotonically with the set of parameters being estimated, but the growth doesn't depend only on the number of parameters, but rather on the (subtle) relationships between them, and it can be 0, for instance if one parameter is a convex combination (linear interpolation) of two others
In both cases, pruning represents both a statistical and computational improvement over earlier progressive sampling techniques.

\if 0
Our learning algorithms can be instantiated with various concentration inequalities.  Building on earlier work~\citep{tuyls2020bounds}, we first apply Hoeffding's bound, but as the size of the game grows, this bound eventually becomes statistically intractable; hence, we also use Rademacher bounds.
\fi

%\cyrus{Note that PSP can use various termination criteria to learn different things.}

We empirically evaluate both \GS{} and \PSP{} with a Bonferroni correction on randomly generated games and finite congestion games~\citep{rosenthal1973class}.
%for which it is known that pure strategy Nash equilibria always exist~\citep{rosenthal1973class}.
We show that they make frugal use of data, accurately estimate properties
%\amy{would be good to test out other properties as well, like welfare-maximizing strategy profiles}
%\enrique{agreed. For the journal version, lets revisit the experiments and brainstrom about how we can expand them. }
of games more often than the theory predicts, and are robust to different forms of noise.
We further show that \PSP{} can significantly outperform \GS, the current state-of-the-art~\citep{tuyls2020bounds}, relying on far fewer data to produce the same (and often times, better) error rates.

In the simulation-based games of interest here, a running assumption is that simulation queries are exceedingly expensive, so that the time and effort required 
%to run the simulator 
to obtain sufficiently accurate utility estimates dwarves that of any other relevant computations, including equilibrium computations.  This assumption is reasonable in so-called \mydef{meta-games}~\citep{tavares2016rock}, where agents choice sets comprise a few high-level heuristic strategies, not intractably many low-level game-theoretic strategies.  Thus, our primary concern is to limit the need for sampling, while still %ensuring that we are 
well estimating a game.


In future work, we plan to study the estimation of other properties of games for which estimation is non-trivial, such as Pareto optimality~\citep{pareto1927manual}.
%and sink equilibria~\citep{goemans2005sink}.


\begin{comment}
Having established that our methodology can be used to solve empirical games (up to our $\epsilon, \delta$ guarantees), we show how it can be extended to estimate the empirical pure price of anarchy~\citep{koutsoupias1999worst}.  We then demonstrate empirically that our learning algorithms are capable of accurately estimating the true pure price of anarchy in a restricted class of congestion games~\citep{christodoulou2005price}. Finally, \enrique{Would be cool to finalize with something like:} we use our learning algorithms  to learn the pure price of anarchy for a distribution\amy{class?} of finite congestion game that resembles real-world usage of a restricted section of the Tokyo metro. We report the perhaps surprising result that the \amy{empirical} price of anarchy for this distribution\amy{class?} is much less than the theoretical worst-case upper-bound.\amy{do we have a worst-case upper bound for this imaginary class?}
\end{comment}

==> lambda-stable.tex <==

\if 0
In this section, we give an example of a property of a game that is not well behaved, and thus cannot be estimated using the methodology developed in this paper.
That property is a welfare-optimizing equilibrium, and its corresponding value, be it welfare-maximizing or welfare-minimizing, and be it utilitarian, egaliatarian, or some other power-mean welfare.
We show that this property is not well behaved by counterexample.
\fi

\if 0
SETS
extreme equilibrium outcomes
maximal consonant equilibrium outcome \\
maximal dissonant equilibrium outcome

extreme $\Lambda$-stable outcomes
maximal consonant $\Lambda$-stable outcome \\
maximal dissonant $\Lambda$-stable outcome

VALUES
maximal equilibrium consonance \\
maximal equilibrium dissonance

maximal $\Lambda$-stable consonance \\
maximal $\Lambda$-stable dissonance
\fi


\section{Estimating Extreme Welfare Equilibria}

In this section, we study the estimation of extreme equilibria in games, measured in terms of the welfare achieved.
An extreme equilibrium can be the best (optimal) or the worst (pessimal),
and the welfare can be utilitarian, egalitarian, or any other monotonically non-decreasing measure of welfare, including power-mean welfare.
%\amy{any monotonic welfare function. broader than just the power-mean welfare functions.}
We call the welfare-maximal equilibria maximally \emph{consonant}, and the welfare-minimizing ones, maximally \emph{dissonant}.
Analogously, we call the values of these equilibria the maximal consonance and dissonance, respectively.

As it turns out, neither the maximally consonant and maximally dissonant equilibria, nor their values, can be estimated using the methodology developed in this paper, because these properties are not Lipschitz continuous in utilities.
Consequently, we define relaxations of these properties, that we call maximally consonant and maximally dissonant $\Lambda$-stable outcomes, which are similar in spirit to their equilibrium counterparts, but which are well behaved.
Specifically, we replace the equilibrium constraints with their Lagrangian relaxations based on a tunable parameter $\Lambda \ge 0$.
This change in the definitions does not alter the spirit of the properties, only the letter, because as $\Lambda$ goes to infinity, the penalty for violating the constraints becomes infinite, so they are not violated.
Further, when $\Lambda$ is finite, these definitions can be understood as permitting small oscillations around extreme equilibria, thus expanding the scope of acceptable play.

For extreme $\Lambda$-stable outcomes, we obtain a positive result, namely, for all games and for all $\epsilon > 0$, there exists a sample size $\NumberOfSamples$ s.t.\ we can $\epsilon$-estimate them.
However, having overcome what might have appeared to be the shortcoming that was preventing the estimation of extreme equilibria, we find ourselves facing a more serious stumbling block.
In particular, although we can now derive a more satisfying bound on these extreme consonance and dissonance properties, given an $\epsilon$-uniform approximation of a game, this bound grows with $\Lambda$.
In other words, fixing the number of samples and letting $\Lambda$ increase so as to produce solutions closer and closer to an extreme equilibrium, yields a larger and larger confidence interval around the property's estimate.
Alternatively, fixing $\epsilon$, as $\Lambda$ grows, $\epsilon$-accurate estimation of the property requires more and more samples.
This result is not surprising, as we have effectively interpolated between two extreme cases: $0$-stable outcomes, which are easy to estimate, and $\infty$-stable outcomes, which cannot be estimated.

%\amy{After conversation with Yasser, we realize this result does not require a second game. One will do. The point is that the welfare of the worst $\gamma$ eqm of a game can differ from the welfare of the worst (exact) eqm by an arbitrary amount. That is the source of this so-called inapproximability.}

\newcommand{\constant}{c}

\begin{figure}[htbp]
\vspace{-0.25cm}
\centering
\begin{subfigure}[t]{0.4\textwidth}
\centering
\begin{game}{2}{2}
      & $A$     & $B$\\
$A$   & $1+\constant,1+\constant$ & $1,0$\\
$B$   & $0,1$                     & $1-\gamma,1-\gamma$
\end{game}
\end{subfigure}
%
\begin{subfigure}[t]{0.4\textwidth}
\begin{game}{2}{2}
      & $A$     & $B$\\
$A$   & $\constant-\gamma,\constant-\gamma$ & $0,\constant$\\
$B$   & $\constant,0$ & $1,1$
\end{game}
\end{subfigure}
\vspace{-0.25cm}
\caption{Inapproximable utilitarian welfare of a pessimal and an optimal equilibrium.}
\label{fig:inapproxWorstWelfare}
\end{figure}

\if 0
\begin{subfigure}[t]{0.5\textwidth}
\centering
\begin{game}{2}{2}
      & $A$     & $B$\\
$A$   & $1+\constant,1+\constant$  & $1,-1$\\
$B$   & $-1,1$   & $1,1$
\end{game}
\caption{Game $\GameTuple'$}
\end{subfigure}
\fi

%\amy{presumably, optimal equilibria are also inapproximable}

\begin{observation}[Pessimal Equilibria are Inapproximable]
\label{obs:counterexample}
Consider the game family $\GameTuple (\gamma)$ parameterized by $\gamma \ge 0$ depicted in Figure~\ref{fig:inapproxWorstWelfare}.
For $\GameTuple \doteq \GameTuple (0)$ and $\GameTuple (\gamma)$ for some $\gamma > 0$
with corresponding utilities $\Utility, \Utility_\gamma$, it holds that
$\forall \epsilon \ge \gamma, \constant > \gamma$,
$\norm{\Utility - \Utility_\gamma}_\infty \leq \epsilon$, but
$\displaystyle \smallabs{
    \smallinf{\StratProfile \in \Nash(\Utility)}
        \Welfare(\StratProfile; \Utility) \, \ - 
    \smallinf{\StratProfile \in \Nash(\Utility_\gamma)}
        \Welfare(\Utility_\gamma, \StratProfile)
    } > \constant$.
\end{observation}

\begin{proof}
%Consider 2 $\times$ 2 family of games shown in Figure~\ref{fig:inapproxWorstWelfare}, and assume $\constant > \gamma > 0$.
The only and thus maximally dissonant Nash equilibrium of $\GameTuple$ is $(A,A)$, with utilitarian welfare $2 + 2 \constant$.
However, $(B,B)$ is an $\gamma$-Nash equilibrium with utilitarian welfare $2 - 2 \gamma$; further, it is the maximally dissonant such equilibrium, since $2 + 2 \constant > 2 - 2 \gamma$.
By assumption, $\GameTuple (\gamma)$ is an $\epsilon$-uniform approximation of $\GameTuple$, but the utilitarian welfare of
\amy{worst => max. diss.}
the worst exact Nash and the worst $\gamma$-Nash differ by $2(c - \gamma) > c$: i.e., arbitrarily.
%essentially: up to the range of values of the game
\end{proof}

\if 0
\amy{\bf OLD!}
\begin{proof}
Assume $\constant > \gamma > 0$.
%\amy{since this is a counterexample, it's fine to just exhibit one. that is, it's fine to assume $\constant > \gamma$.}
Consider the pair of 2 $\times$ 2 games $\Utility$ and $\Utility'$ shown in Figure~\ref{fig:inapproxWorstWelfare}. 
Since the utilities of these games are equal everywhere except at profile $(B,B)$, where they differ by $\gamma$ for both agents, it follows that $\norm{\Utility - \hat{\Utility}}_\infty \leq \gamma$. 
Now, note that the unique Nash equilibrium in $\Utility$ is the pure strategy profile $(A, A)$, with utilitarian welfare $2 + 2\constant$.
%\cyrus{Can we prove this is the only Nash?} 
%\enrique{yes we can, by IEDS}
Game $\hat{\Utility}$ has two pure strategy equilibria: profile $(A, A)$ with utilitarian welfare $2 + 2 \constant$, and profile $(B, B)$ with utilitarian welfare $2$. Since $\constant > 0$, the minimum utilitarian welfare equilibrium in $\hat{\Utility}$ is $2$. (Note that any mixed-strategy equilibria must have welfare strictly greater than 2.)
But then, $|(2 + 2 \constant) - 2| = 2 \constant > \constant$. 
\end{proof}
\fi

\if 0
\begin{verbatim}
NEW
positive result:
for all $\epsilon$, there exists sample size $m$ s.t.\ we can estimate Lambda-maxNash. \\
negative result:
for all $\epsilon$, there does not exist an $m$ that is sufficient to estimate all maxNash. \\
counterexample is a family of games that is inestimable when $\gamma$ is smaller than $\epsilon$.

OLD
min = best Nash
max = worst-case over free parameters (utilities and condition distribution)
minimax sample complexity cannot distinguish these between two quantities
---inf welfare in Gamma and Gamma'---
because it cannot estimate the utilities of (B,B) well enough
\end{verbatim}
\fi

\if 0
A proof of this fact would reduce the mean-estimation problem to learning these properties.
For all $\gamma > 0$, the \emph{mean-estimation problem\/} is to determine the expected value of a random variable to within $\gamma$-accuracy.
If we can determine w.h.p.\ that the entries in $B$ are not 1, or equivalently, that $\gamma=0$,
then we could solve the mean-estimation problem.
\amy{HOW?}
\fi

These counterexamples can be used to show that there does not exist a finite sample size $m < \infty$ that is sufficient to $\epsilon$-estimate maximally consonant and maximally dissonant equilibria, or their values.
A proof of this fact would reduce a special case of mean-estimation 
%the problem of determining whether a coin's bias is \emph{not\/} 1 
to learning these properties.
Imagine two biased coins, one that is always heads, and another that is heads with probability $1-\gamma$.
The problem is to distinguish between the two.
A player is given one of them, and asked to determine which one it is.
We construct a simulation-based game from this problem using the basic structure of the LHS game in Figure~\ref{fig:inapproxWorstWelfare}.
The simulator returns deterministic utilities for all profiles except $B,B$.
At $B,B$, it flips the coin, returning $1,1$ when it sees heads, and $0,0$ otherwise.
Note that as $\gamma$ approaches zero, the number of coin flips required to see even a single tail with fixed positive probability approaches infinity, thus so too must the sample complexity of estimating the worst Nash equilibrium.
A similar construction can be applied to the game on the RHS of Figure~\ref{fig:inapproxWorstWelfare} holds for the best equilibrium.
As $\gamma$ is simply a game parameter, we thus conclude that \emph{no\/} finite sample size is sufficient to uniformly estimate the extreme equilibria of all games (of a given size and range), i.e., extreme equilibria are inapproximable.

\if 0
Make $B$ Bernoulli with bias $\gamma$.
As $\gamma \to \infty$, it becomes impossible to determine whether $B$ will ever realize a tail at all.

The number of coin flips $n$ required to see a tail with probability $\delta$ approaches $1 - \nicefrac{\gamma}{n}$ (probability of $n$ heads).
\fi

\if 0
CLAIM: there exist two games, u and u', same range c, s.t.\ they differ in this property by up to c, and the sample complexity of distinguishing b/n the two games is unbounded.

PROOF: to determine if game is u or u',
u is when $\gamma=0$, u' o/w
is B,B 1 or something smaller than 1?
reduction:
construct game
if can distinguish, can solve the mean estimation problem
but, there are lower bounds for mean estimation
require var/eps$^2$ samples
take eps as small as we want, and that takes the sample complexity as large as we want
\fi

\begin{corollary}
For all $\epsilon$, there does not exist a finite sample size $m < \infty$ that is sufficient to $\epsilon$-estimate maximally consonant and maximally dissonant equilibria, or their values.
\end{corollary}


\if 0

%It is tempting to think that $\norm{\GameTuple - \GameTuple'}_\infty \leq \gamma$ implies a bound on $\left| \Anarchy (\GameTuple) - \Anarchy (\GameTuple') \right|$.  While the assumption does indeed imply a bound on the optimal welfare, it does not imply a bound on the worst equilibrium welfare, because in general we can't obtain a fixed-width confidence interval about the welfare of the worst true equilibrium.  Consequently, for any fixed $\gamma$, $\abs{\Anarchy (\GameTuple) - \Anarchy (\GameTuple')}$ is unbounded.

Although optimal welfare is bounded (\cref{lemma:welfare}),
%and regardless of \amy{consistency} (\cref{lemma:consistent}),
the difference between the welfares of the worst equilibria in the game and its estimate can be unbounded.
%we can't obtain a fixed-width confidence interval about the welfare of the worst exact equilibrium,
To illustrate this point, consider that $\GameTuple$ may have an arbitrarily bad $0$-equilibrium that has regret $2\gamma$ in $\GameTuple'$, making the denominator in $\Anarchy (\GameTuple')$ too large relative to that of $\Anarchy (\GameTuple)$.  Likewise, $\GameTuple'$ can have an arbitrarily bad 0-equilibrium that is a $2\gamma$ equilibrium in $\GameTuple$, making the denominator of $\Anarchy (\GameTuple')$ too small relative to that of $\Anarchy (\GameTuple)$.  Consequently, this naive estimation strategy can be arbitrarily incorrect in both directions, for any finite $\gamma$.
Nonetheless, we can and do bound the POA:
first, in a somewhat unsatisfying manner,
making no assumptions on $\GameTuple$;
and later, more convincingly,
after making suitable assumptions on $\GameTuple$.

\todo{I (Cyrus) claim that such a thing can occur, and it definitely can for pure equilibria, but I would like to see an example in mixed games.  I think a modified prisoner's dilemma would work, where slight changes would encourage cooperative play?}

\[
\begin{matrix}
(a, a) & (1, -1) \\
(-1, 1) & (b, b) \\
\end{matrix}
\]

We can take $a > 1$ to be arbitrarily large to set the optimal welfare.  Now, for $b < 1$, this is the only equilibrium \todo{I think, please confirm}, but for $b \geq 1$, we obtain a second equilibrium that is arbitrarily worse than the first. 

\fi


\newcommand{\MaxDis}[1][]{{\rm{MD}_{#1}}}
\newcommand{\MaxCon}[1][]{{\rm{MC}_{#1}}}

Next, we derive natural bounds on extreme equilibria, both from above and below, albeit loosely.
We then present an unnatural, yet sufficient, condition under which the upper (lower) bound on the maximally dissonant (consonant) equilibrium value can be tightened.
We write $\MaxDis(\Utility)$ and $\MaxCon(\Utility)$ to denote the set of maximally dissonant and maximally consonant equilibria of the game defined by $\Utility$.
\amy{so far, same notation for values and eqa/witnesses}
As all elements of these sets have the same values, we overload this notation, using it to denote both the set (i.e., the witnesses) and the value of all its elements.

%Using our approximation framework, it is straightforward to upper and lower bound extreme equilibria; in general, however, the gap may be arbitrarily wide.  
Given a game $\Utility$, the maximally dissonant equilibrium value $\MaxDis (\Utility)$ is upper bounded by the maximally consonant one $\MaxCon (\Utility)$.
To obtain a lower bound on $\MaxDis (\Utility)$,
we consider the value of the maximally dissonant $2\epsilon$-equilibria in an $\epsilon$-approximation $\Utility'$ of $\Utility$, which underestimates the maximally dissonant equilibrium value of $\Utility$.
Similarly, to obtain an upper bound on $\MaxCon (\Utility)$, we consider the value of the maximally consonant $2\epsilon$-equilibria in $\Utility'$, which overestimates the maximally consonant equilibrium value of $\Utility$.
Note that both these bounds can be arbitrarily loose, as the extreme $2\epsilon$-equilibria in $\Utility'$ may not correspond to extreme equilibria in $\Utility$ (see Observation~\ref{obs:counterexample}).
%To ensure that no exact equilibrium's welfare goes uncounted,
That said, we can tighten this bound if we assume that the welfare of \emph{every\/} $\alpha$-Nash equilibrium in $\Utility$ approximates 
(by $\alpha\gamma$ for some $\gamma > 0$)
that of an exact Nash equilibrium (also in $\Utility$), as this assumption enables accurate estimation of the welfare of extreme equilibria.

We now formalize these arguments.
%
As usual, we fix two compatible games
%$\GameTuple$ and $\GameTuple'$ 
characterized by utility functions $\Utility$ and $\Utility'$, 
and we assume that $\Utility'$ is an $\epsilon$-uniform approximation of $\Utility$.

\begin{theorem}[Approximating Extreme Equilibria]
\label{thm:bestNash}
Fix $\epsilon > 0$.
Assume $\Welfare: \StratProfileSpace \times (\StratProfileSpace \to \R^{\NumberOfPlayers}) \to \R$
is monotonic non-decreasing so that $\Utility \preceq \bm{v}$ component-wise implies $\Welfare(\StratProfile; \Utility) \le \Welfare(\StratProfile; \bm{v})$, for all $\StratProfile \in  \StratProfileSpace$ and utilities $\Utility$ and $\bm{v}$.
It holds that:

\if 0
extreme equilibrium outcomes
maximal consonant equilibrium outcome \\
maximal dissonant equilibrium outcome
\fi

\begin{equation}
\inf_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\StratProfile; \Utility' - \epsilon) \leq \MaxDis (\Utility) \leq \MaxCon (\Utility) \leq
\sup_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\StratProfile; \Utility' + \epsilon) \enspace .
\label{eq:worstNashNaiveBounds}
\end{equation}

Suppose further that $\exists \gamma > 0$
s.t.\ $\forall \alpha > 0, \forall \StratProfile \in \Nash_{\alpha}(\Utility), \exists s' \in \Nash (\Utility)$
s.t.\ $\abs{\Welfare (\StratProfile; \Utility) - \Welfare (\StratProfile; \Utility')} \leq \alpha \gamma$.
%
We may then refine the upper bound on the $\MaxDis(\Utility)$ as
%\begin{equation}
$\MaxDis(\Utility) \leq \inf_{\StratProfile \in \Nash (\Utility')} \Welfare (\StratProfile; \Utility' + \epsilon) + 2 \gamma \epsilon$,
%\enspace ,
%\label{eq:worsyNashBetterBounds}
%\end{equation}
%
and similarly, the lower bound on the $\MaxCon(\Utility)$ as
%\begin{equation}
$\sup_{\StratProfile \in \Nash (\Utility')} \Welfare (\StratProfile; \Utility' - \epsilon) - 2 \gamma \epsilon \leq \MaxCon(\Utility)$.
%\enspace .
%\label{eq:worsyNashBetterBounds}
%\end{equation}
\end{theorem}

\begin{proof}
The first claim follows as
\begin{align*}
\inf_{\StratProfile \in \Nash_{2\epsilon} (\Utility')} \Welfare (\StratProfile; \Utility' - \epsilon) & \leq \inf_{\StratProfile \in \Nash (\Utility)} \Welfare (\StratProfile; \Utility' - \epsilon) & \Nash (\Utility) \subseteq \Nash_{2\epsilon} (\Utility') \\
& \leq \inf_{\StratProfile \in \Nash (\Utility)} \Welfare (\StratProfile; \Utility) \ = \ \MaxDis(\Utility) & \textsc{monotonicity} \\
& \leq \sup_{\StratProfile \in \Nash (\Utility)} \Welfare (\StratProfile; \Utility) \ = \ \MaxCon(\Utility)  & \inf_{x \in X} f(x) \leq \sup_{x \in X} f(x) \\
& \leq \sup_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\StratProfile; \Utility) & \Nash (\Utility) \subseteq \Nash^\diamond_{2\epsilon}(\Utility') \\
& \leq \sup_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\StratProfile'; \Utility + \epsilon) & \textsc{monotonicity}
\end{align*}

We now show the second claim:
%Assume that $\exists \gamma > 0$ s.t.\ $\forall \alpha > 0$ and $\forall \StratProfile \in \Nash_{\alpha}(\Utility), \exists s' \in \Nash (\Utility)$ s.t.\ $\abs{\Welfare (\StratProfile; \Utility) - \Welfare (\StratProfile; \Utility')} \leq \alpha \gamma$.
\[
\inf_{\StratProfile \in \Nash (\Utility)} \Welfare(\StratProfile; \Utility) 
    \leq 
\inf_{\StratProfile \in \Nash_{2\epsilon} (\Utility)} \Welfare(\StratProfile; \Utility) + 2 \epsilon \gamma
    \leq 
\inf_{\StratProfile \in \Nash (\Utility')} \Welfare(\StratProfile; \Utility) + 2 \epsilon \gamma
    \leq 
\inf_{\StratProfile \in \Nash (\Utility')} \Welfare(\StratProfile; \Utility' + \epsilon) + 2 \epsilon \gamma
\]
where the first inequality is by assumption, with $\alpha = 2\epsilon$; 
the second follows because 
$\Nash (\Utility') \subseteq \Nash_{2\epsilon} (\Utility)$; and
the last, by monotonicity.
%
Similarly,
\[
\sup_{\StratProfile \in \Nash (\Utility')} \Welfare(\StratProfile; \Utility' - \epsilon) - 2 \epsilon \gamma
    \leq 
\sup_{\StratProfile \in \Nash (\Utility')} \Welfare(\StratProfile; \Utility) - 2 \epsilon \gamma
    \leq 
\sup_{\StratProfile \in \Nash_{2\epsilon} (\Utility)} \Welfare(\StratProfile; \Utility) - 2 \epsilon \gamma
    \leq 
\sup_{\StratProfile \in \Nash (\Utility)} \Welfare(\StratProfile; \Utility)
\]
where the first inequality follows by monotonicity;
the second follows because 
$\Nash (\Utility') \subseteq \Nash_{2\epsilon} (\Utility)$; and
the third inequality is by assumption, with $\alpha = 2\epsilon$.
\end{proof}

The condition that $\left| \Welfare (\StratProfile; \Utility) - \Welfare (\StratProfile; \Utility') \right| \leq \alpha \gamma$ is essentially a variant of the \emph{$\epsilon$-$\Delta$ approximate stability} property introduced by Awasthi \emph{et al.\/} \citep{awasthi2010nash}, who find that many natural games, such as matching pennies and rocks-paper-scissors, satisfy these conditions.  Interestingly, while they use the condition to bound the error induced by \emph{computational\/} approximation, our usage demonstrates that it can also be used to control the error due to \emph{statistical\/} approximation.


%This result is prototypical of a large family of related bounds.  The first claim holds for both pure and mixed Nash equilibria, and variants of both should hold for other solution concepts.


As the condition of Theorem~\ref{thm:bestNash} is difficult to justify, we now propose an alternative quantity as a substitute measure for extreme equilibria, namely extreme $\Lambda$-stable outcomes, in which we replace the equilibrium constraints with their Lagrangian relaxation.
%based on a tunable parameter $\Lambda \ge 0$.
We now write $\MaxDis[\Lambda] (\Utility)$ ($\MaxCon[\Lambda] (\Utility)$) to denote the maximally dissonant (consonant) $\Lambda$-stable \emph{outcomes\/} of the game defined by $\Utility$.
\amy{overloading notation!}

\begin{definition}
\label{def:Lambda-stable}
Given a game $\GameTuple$ with corresponding utilities $\Utility$, and $\Lambda \ge 0$, a \mydef{maximally dissonant $\Lambda$-stable outcome} is an element of
$\MaxDis[\Lambda] (\Utility) \doteq \inf_{\StratProfile \in \StratProfileSpace} \Welfare(\StratProfile; \Utility) + \Lambda \Regret(\StratProfile; \Utility)$.
A \mydef{maximally consonant $\Lambda$-stable outcome} is defined analogously: i.e.,
$\MaxCon[\Lambda] (\Utility) \doteq \sup_{\StratProfile \in \StratProfileSpace} \Welfare(\StratProfile; \Utility) - \Lambda \Regret(\StratProfile; \Utility)$.
\end{definition}

These new quantities are Lipschitz continuous in utilities, as we argue next, and thus are better behaved than extreme equilibria, in that they can be well estimated via a uniform approximation.

Thinking ahead to the next section, we also provide a proof that
$\MaxDis_{\Lambda}^* (\Utility)$ and $\MaxCon_{\Lambda}^* (\Utility)$ are Lipschitz continuous in utilities.
These quantities are analogous to their counterparts, but are defined in terms of the \mydef{excess regret} $\Regret^{*}(\StratProfile; \Utility)$, which is defined as $\Regret^{*}(\StratProfile; \Utility) \doteq \Regret(\StratProfile; \Utility) - \inf_{\StratProfile'} \Regret(\StratProfile'; \Utility)$.
%
Note that the Lipschitz constant of $\Regret^{*}(\StratProfile; \Utility)$ is 4, a result which can be obtained via similar techniques.

%\amy{more complex than the earlier cases. that's why we provide the syntax tree.}

\begin{theorem}
\label{thm:Lambda-stable}
Assume $\Welfare: \StratProfileSpace \times (\StratProfileSpace \to \R^{\NumberOfPlayers}) \to \R$ is %$\lambda_{\Welfare}$-Lipschitz continuous in $\Utility$.
a $\lambda_{\Welfare}$-Lipschitz property.
It holds that
$\MaxDis[\Lambda] (\Utility)$ is $\lambda_{\Welfare} + 2\Lambda$-Lipschitz, which immediately implies that
$\abs{ \MaxDis[\Lambda] (\Utility) - \MaxDis[\Lambda] (\Utility') } \leq (\lambda_{\Welfare} + 2\Lambda) \epsilon$.
%\norm{ \Utility -  \Utility' }_{\infty}
Likewise, for $\MaxCon[\Lambda] (\Utility)$.
%
It also holds that
$\MaxDis_{\Lambda}^* (\Utility)$ is $\lambda_{\Welfare} + 4\Lambda$-Lipschitz, which immediately implies that
$\abs{ \MaxDis_{\Lambda}^* (\Utility) - \MaxDis[\Lambda] (\Utility') } \leq (\lambda_{\Welfare} + 4\Lambda) \epsilon$.
%\norm{ \Utility -  \Utility' }_{\infty}
Likewise, for $\MaxCon_{\Lambda}^* (\Utility)$.
\end{theorem}

\begin{proof}
We prove this theorem using the Lipschitz calculus (Theorem~\ref{thm:lipschitz-properties}).
By Lemma~\ref{lem:regret-2Lipschitz}, Regret is 2-Lipschitz.
Moreover $\inf$ provides a 1-Lipschitz multiplicative factor.
Finally, addition requires that we add the Lipschitz constants of the corresponding addends.
We begin at the leaves in Figure~\ref{fig:lipschitz}, computing Lipschitz constants, and back those values up the syntax tree to arrive at $2(\lambda_{\Welfare} + \Lambda)$ Lipschitz constant for $\MaxDis[\Lambda] (\Utility)$.
%
The inequality then follows via Observation~\ref{obs:lipschitz-uniform}.

The proof in the remaining three cases---$\MaxCon[\Lambda] (\Utility)$, 
$\MaxDis_{\Lambda}^* (\Utility)$, and
$\MaxCon{\Lambda}^* (\Utility)$---are analogous.
\end{proof}

\begin{figure}
\begin{center}
\begin{tikzpicture}[xscale=2,yscale=0.9]

%\node[rectangle,draw=black] (sub) at (0, 0) {$-: ( \lambda_{\Welfare} ) + (\lambda_{\Welfare} + 2\Lambda)$};

%\node[rectangle,draw=black] (sup) at (-1, -1) {$\displaystyle\sup_{\StratProfile \in \StratProfileSpace}: 1 \times (\lambda_{\Welfare})$};
\node[rectangle,draw=black] (inf) at (1, -1) {$\displaystyle\inf_{\StratProfile \in \StratProfileSpace}: 1 \times (\lambda_{\Welfare} + 2\Lambda)$};

%\node[rectangle,draw=black] (w1) at (-1, -2) {$\displaystyle\Welfare (\StratProfile): \lambda_{\Welfare}$};

\node[rectangle,draw=black] (plus) at (1, -2) {$\displaystyle+: (\lambda_{\Welfare}) + (2\Lambda) $};

\node[rectangle,draw=black] (w2) at (0.5, -3) {$\displaystyle\Welfare (\StratProfile): \lambda_{\Welfare}$};

\node[rectangle,draw=black] (times) at (1.5, -3) {$\displaystyle\times: (\Lambda) \times (2)$};
%\node[rectangle,draw=black] (times) at (1.5, -3) {$\Lambda \Regret (\StratProfile)$};

\node[rectangle,draw=black] (Lam) at (1, -4) {$\Lambda: \Lambda$};

\node[rectangle,draw=black] (reg) at (2, -4) {$\Regret (\StratProfile; \Utility): 2$};

%\draw[->] (sub) -- (sup);
%\draw[->] (sub) -- (inf);

%\draw[->] (sup) -- (w1);

\draw[->] (inf) -- (plus);

\draw[->] (plus) -- (w2);
\draw[->] (plus) -- (times);

\draw[->] (times) -- (Lam);
\draw[->] (times) -- (reg);

\end{tikzpicture}
\begin{tikzpicture}[xscale=2,yscale=0.9]

%\node[rectangle,draw=black] (sub) at (0, 0) {$-: ( \lambda_{\Welfare} ) + (\lambda_{\Welfare} + 2\Lambda)$};

%\node[rectangle,draw=black] (sup) at (-1, -1) {$\displaystyle\sup_{\StratProfile \in \StratProfileSpace}: 1 \times (\lambda_{\Welfare})$};
\node[rectangle,draw=black] (inf) at (1, -1) {$\displaystyle\inf_{\StratProfile \in \StratProfileSpace} : 1 \times (\lambda_{\Welfare} + 4\Lambda)$}; %TODO:  $(\downarrow) (\swarrow) \dots

%\node[rectangle,draw=black] (w1) at (-1, -2) {$\displaystyle\Welfare (\StratProfile): \lambda_{\Welfare}$};

\node[rectangle,draw=black] (plus) at (1, -2) {$\displaystyle+: (\lambda_{\Welfare}) + (4\Lambda) $};

\node[rectangle,draw=black] (w2) at (0.5, -3) {$\displaystyle\Welfare (\StratProfile): \lambda_{\Welfare}$};

\node[rectangle,draw=black] (times) at (1.5, -3) {$\displaystyle\times: (\Lambda) \times (4)$};
%\node[rectangle,draw=black] (times) at (1.5, -3) {$\Lambda \Regret (\StratProfile)$};

\node[rectangle,draw=black] (Lam) at (1, -4) {$\Lambda: \Lambda$};

\node[rectangle,draw=black] (reg) at (2, -4) {$\Regret^{*} (\StratProfile; \Utility): 4$};

%\draw[->] (sub) -- (sup);
%\draw[->] (sub) -- (inf);

%\draw[->] (sup) -- (w1);

\draw[->] (inf) -- (plus);

\draw[->] (plus) -- (w2);
\draw[->] (plus) -- (times);

\draw[->] (times) -- (Lam);
\draw[->] (times) -- (reg);

\end{tikzpicture}
\end{center}
\vspace{-0.25cm}
\caption{Abstract syntax tree derivation of the Lipschitz constant for $\MaxDis[\Lambda] (\Utility)$, left, and $\MaxDis_{\Lambda}^* (\Utility)$, right.}
\vspace{-0.25cm}
\label{fig:lipschitz}
\end{figure}

Not only are extreme $\Lambda$-stable outcomes mathematically preferable to extreme equilibria because of their estimation properties, we believe they are also as, if not more, justifiable as descriptors or predictors of the play of a game.
%
The standard motivation for considering welfare \emph{at equilibrium\/} is that we expect ideal players to converge to equilibrium play.
On the other hand, it is reasonable to expect non-ideal players 
%in changing environments and/or with incomplete information 
to play near, but not exactly at, equilibria.
By expanding the scope of 
%non-cooperative 
play to include approximate equilibria, we are able to accommodate more realistic behavior.
At the same time, the parameter $\Lambda$ allows us to control the extent to which non-equilibrium play is acceptable.
Taking $\Lambda = 0$ ignores equilibrium behavior entirely, while at the other extreme, taking $\Lambda \to \infty$, $\MaxDis[\Lambda] (\Utility) \to \MaxDis (\Utility)$ (likewise, $\MaxCon[\Lambda] (\Utility) \to \MaxCon (\Utility)$), because as $\Lambda$ goes to infinity, the penalty for violating the constraints becomes infinite, so they are not violated.

We can interpret $\Lambda$-stable outcomes that deviate from equilibrium play as ranging from fully cooperative to fully non-cooperative.
The welfare term is a cooperative one, where the players are colluding to make the world as wonderful (or terrible) a place as possible.
The regret term, in contrast, is non-cooperative, but $\Lambda$ permits some flexibility in behavior.
In the case of a maximally dissonant (colluding) outcome,
%\amy{strategy profile}
$\Lambda = 0$ implies the players are all playing pessimally: i.e., 
%even worse than playing their minimax strategies, 
they are colluding to cause as much suffering to all players (including themselves) as possible.
The opposite is true of maximally consonant (colluding) outcome, where players are colluding to create a utopia.
On the other hand, as $\Lambda \to \infty$, the players move away from cooperative behavior towards rational
%selfish, as well, since they are working for themselves ONLY
equilibrium (i.e., non-cooperative) behavior.
%%%In other words, for finite $\Lambda$, players are not necessarily colluding, but nor are they necessarily playing near equilibrium.
%nor are they 100% SELFISH
Indeed, $\Lambda$-stability allows us to model a range of cooperative to non-cooperative behaviors.
%%%from fully cooperative to fully non-cooperative.


==> main.tex <==
\input{templates/ec/ec_header}


% OLD
%\input{introduction}
%\input{related_work}
%\input{outline}

\input{new_intro}
\ifpoa{\input{extreme}}
\input{new_related}

\input{game_theory}
\input{lipschitz}
\input{mixed}
\input{uniform}
\input{precision-recall}

\input{empirical_games}
\input{concentration}
\input{hoeffding}
\input{bennett}
%\input{rademacher}

%\input{outline}
\input{schedule}
\input{algorithms/PSP_well}
\input{correctness}
\input{efficiency}

% ENRIQUE
%\input{pruning_expts}

% BHASKAR
\input{bhaskar_experiments/intro}
\input{bhaskar_experiments/setup}
\input{bhaskar_experiments/algos}
\input{bhaskar_experiments/properties}

\ifpoa{
% POA
\input{poa/lambda-stable}
\input{poa/poa_thewellwellory}
\input{poa/modified_poa}
\input{poa/discussion}
}

\if 0
\input{poa/ppoa_est_algo}
\input{expts/ppoa_expts}
\input{poa/ppoa_examples}

\include{expts/poa_expts_overview}
\fi

\input{new_conc}
%\input{future_work}
%\input{conclusion}

\if 0
\begin{acks}
This work was supported in part by NSF Grant CMMI-1761546.
\end{acks}
\fi

\pagebreak[3]

% Bibliography
{
\bibliographystyle{ACM-Reference-Format}
\bibliographystyle{plainnat}
%\tiny

%\bibliographystyle{abbrv}
%\renewcommand*{\bibfont}{\footnotesize}
%\def\bibfont{\footnotesize}
\bibliography{bibliography}
}

\pagebreak[4]



\iftrue
\appendix
\onecolumn

\renewcommand\thefigure{\thesection.\arabic{figure}}
\renewcommand\thealgorithm{\thesection.\arabic{algorithm}}

\input{appendix/lipschitz-proofs}

\input{appendix/finite-sample-bounds-proofs}

\section{Derived Games}
\input{correlated}
\input{team_games}

\input{sampling_schedule}
\input{appendix/algorithm-proofs}

\ifpoa{
\input{poa/poa_appendix}
\input{expts/anarchy_gap_experiments}
}
\fi


\input{templates/ec/ec_footer}
%\input{templates/one_column_footer}This work was supported in part by NSF Grant CMMI-1761546, the NEC-AIST AI Cooperative Research Laboratory, and NSF Award RI-1813444.


==> old_abstract.tex <==
\begin{abstract}
We tackle a fundamental problem in empirical game-theoretic analysis (EGTA), that of learning equilibria and other properties of simulation-based games.
Such games cannot be described in analytical form; instead, a black-box simulator can be queried to obtain noisy samples of utilities.
Our approach to EGTA is in the spirit of probably approximately correct 
%(PAC) 
learning. 
We design algorithms that learn so-called empirical games, which uniformly approximate the utilities of simulation-based games with finite-sample guarantees.
These algorithms can be instantiated with various concentration inequalities.
Building on earlier work, we first apply Hoeffding's bound, but as the size of the game grows, this bound eventually becomes statistically intractable; hence, we also use the Rademacher complexity.
%
Our main results state: with high probability, all equilibria of the simulation-based game are approximate equilibria in the empirical game (perfect recall); and conversely, all approximate equilibria in the empirical game are approximate equilibria in the simulation-based game (approximately perfect precision).
%
%Our main results then state: with high probability, an empirical game constructed via our algorithms includes all the Nash equilibria of the corresponding simulation-based game, so that all true positives are approximate equilibria in the empirical game (perfect recall); conversely, every $2 \epsilon$-Nash in the empirical game is a $4 \epsilon$-Nash in the corresponding simulation-based game, so that all false positives in the empirical game are indeed approximate equilibria (approximately perfect precision).  
%
We evaluate 
%the performance of 
our algorithms on several synthetic games, showing that they make frugal use of data, produce accurate estimates more often than the theory predicts, and are robust to different forms of noise.
We close by applying our theory to estimating the price of anarchy in empirical, and hence, simulation-based, games.
\end{abstract}

%Our work is a contribution to the incipient theoretical literature on EGTA for simulation-based games.
%We present a framework for learning games from data such that an ensuing game estimate is an $\epsilon$-uniform approximation of a game with high probability; and we show that such an estimate allows us to estimate properties (e.g., equilibria) of the game.}

==> old_intro.tex <==

\if 0

\amy{uniform alone is sufficient for properties alone (without computing extrema)...might even be necessary in some cases. but, non-uniform---opt'y pruning---is sufficient AND more efficient for finding extrema of properties. (well-estimated pruning is useful even for estimating properties alone.)}


The aim of this work is to design learning algorithms that can generate an estimate $\hat{Y}$ of a property $Y \in \mathcal{Y}$ of a simulation-based game $\GameTuple$, with a guarantee $\norm{Y - \hat{Y}}_{\mathcal{Y}} \leq \epsilon$ w.h.p., where $\norm{\cdot}_{\mathcal{Y}}$ is some norm 
%used to measure error
nover the space of properties $\mathcal{Y}$.
\cyrus{It may have been a mistake to measure error with $\norm{Y - \hat{Y}}_{\mathcal{Y}}$.  Initially, this was the obvious choice, because when $\mathcal{Y}$ is the space of utility functions (or games), we can measure error with $\norm{\cdot}_\infty$.  However, in the perfect-precision and perfect-recall cases, we then have an asymmetry, as we need to ensure $Y \subseteq \hat{Y}$, and given that, our error metric is based on the most incorrect member of $\hat{Y}$.  I think the fix is to define an error measurement as a function, rather than a norm.  I don't really know what to call this; it's roughly analogous to a loss function, but I'm open to ideas.}

we define a ``true'' functional: knows true utility
w(s; u) = welfare at that profile wrt game u
we estimate this functional, wrt estimated utilities
w(s; u') = welfare at that profile wrt game u'

***uniform guarantee over changes to the second argument:
for any value of strat profile and second arg, true welfare and est welfare are similar.
if can get uniform guarantee over first arg, utility, can get uniform guarantee over property.

Lipschitz:
sup over domain of first arg of functional.
domain = set of all strat profiles.

fix true utility in true game, and estimated util in empirical game. now given a uniform guarantee over the domain of the functional (b/c the rest is fixed), true functional is approximated by the estimated functional at every strat profile.

We tackle this problem using the \mydef{probably approximately correct} (PAC) learning framework~\citep{valiant1984theory}.
Our algorithms learn so-called \mydef{empirical games}~\citep{wellman2006methods}, which are estimates of simulation-based games constructed via sampling.
We argue that empirical games so constructed yield \mydef{uniform approximations} of simulation-based games, meaning all the players' utilities in the empirical game tend toward their expected counterparts,
%in the simulation-based game,
\emph{simultaneously}.

This notion of uniform approximation is central to our work: we prove that several game properties are \emph{well behaved}, meaning they are Lipschitz continuous in utilities, and hence can be accurately estimated, given only a uniform approximation.
\amy{We call such properties ``smooth.'' (or regular, or something)...$\lambda$-Lipschitz properties}
Most notable among the \amy{regular} properties is the set of equilibria of a game: when one game $\GameTuple'$ is a uniform approximation of another $\GameTuple''$, all equilibria in $\GameTuple'$ are approximate equilibria in $\GameTuple''$~\citep{tuyls2020bounds}
\amy{insert reference to AAMAS paper + EA}.
\amy{Other examples of smooth properties include: \ldots}
Our learning algorithms, which learn empirical games that are uniform approximations of simulation-based games well estimate \emph{all\/} $\lambda$-Lipschitz properties of the latter.

\fi


==> outline.tex <==
\section{Outline of Proofs}

\amy{
1. old correctness, was for fixed $T$, but might fail. $\hat{\epsilon}$ might not be less than $\epsilon$. \\
2. plan: endogenously derive a $T$ dependent on $\epsilon$ so that we never fail. \\
3. correctness proof: 
step a. for a sufficiently large $T$, we never fail (b/c we fall back to Hoeffding at the max $T$);
step b. here's how to find $T$
}

to find the schedule: \\
first question: what is the smallest sample size where i can make progress?
using Bennett, can derive a lower bound on this sample size.
\[
m_{0} \geq \frac{\UtilityRange \ln \frac{3T\abs{\GameTuple}}{\delta} }{3\epsilon}
\]
using Hoeffding, can derive an upper bound on this sample size.
\[
m_{T} \leq \frac{\UtilityRange^{2} \ln \frac{3T\abs{\GameTuple}}{\delta} }{2\epsilon^{2}}
\]
now, for any value of $T$, i need b/n this many and that many samples to terminate.

assume don't want to overshoot by more than a factor of 2.
using a doubling schedule b/n upper and lower bounds.
how many times to double? base 2 of log of ratio of max over min sample size.
in that ratio: all dependence on $T$ divides out.
so the result is a schedule that is independent of $T$.
can now go back and plug in for the first $m$, based on the derived value of $T$, and double to arrive at subsequent values of $m$.

why geometric? b/c i want to be efficient. want multiplicative guarantee.

\bigskip

why is this hard? \\
correctness needs a schedule. \\
efficiency needs a schedule. \\
the schedule is derived to optimize efficiency but is constrained to be correct.

outline of intuition for the schedule: \\
what is the smallest sample size where you could make progress? AND what is the largest sample size you would ever need a la Hoeffding. \\
add the idea that you want your algo to be efficient. multiplicative efficiency implies doubling, so i don't overshoot a sufficient sample size by more than a factor of 2. \\
can now derive a schedule that is satisfactory given those constraints. (could perhaps do better.)

correctness: \\
a. eventually everything is pruned. (use Hoeffding; union bound) \\
b. when something is pruned it is correct to do so.
use empirical variance to upper bound variance (empirical Bennett bound).

efficiency: \\
not enough to say you will prune eventually, must prove you will prune at a certain, specific point. \\
whp empirical variance is small enough to prune \\
make a correction for empirical variance. \\
when you terminate is a function of variance.

one way to structure the argument: \\
lemma 1. given a schedule, correctness works. \\
lemma 2. given a schedule, efficiency works. \\
next: here's how to derive a schedule that works. \\
thm: the algorithm is correct and efficient. \\
\amy{we actually tell the story in the opposite order}

btw, opposite techniques in the two proofs: flipping variance and empirical variance (upper vs. lower tail bound on empirical variance)


==> overview.tex <==
\paragraph{Overview}
This paper is organized as follows. 
In \Cref{sec:approx},
we present our approximation framework, in which we show that certain properties of games are \emph{approximable}: i.e., they are approximately preserved by uniform game approximations.
In \Cref{sec:learn}, we present our learning framework, in which we show that empirical games uniformly 
%approximate simulation-based games
converge to their 
%simulation-based 
expected counterparts with high probability, given finitely many samples.
We conclude that certain properties of simulation-based games are \emph{learnable} from finitely many samples: i.e., approximable with high probability.
%i.e., they are approximately preserved (by empirical games) w.h.p..
In \Cref{sec:algos}, we present two algorithms that uniformly learn simulation-based games; the first is expensive but always
%produces games with
yields guarantees, while the second is more statistically efficient, but can exhaust its sampling budget and fail.
Finally, in \Cref{sec:expts}, we experiment with these algorithms, showing that they can indeed learn properties of interest, often more efficiently than the theory suggests.

==> poa/old/old_poa.tex <==
\if 0

\begin{lemma}
\label{lemma:consistent}
If $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$,
then $\Anarchy (\GameTuple')$ is a ``consistent'' estimator of $\Anarchy (\GameTuple)$, \cyrus{in the sense that as $\epsilon$ tends to $0$, it converges to the true POA}.
\end{lemma}

\cyrus{Here's my take on a lemma.  It is ``consistent'' in the sense that a consistent estimator for $\GameTuple$ produces such a sequence, thus it can be used to construct a consistent estimator for the POA.}

\begin{lemma}
\label{lemma:consistent}
Suppose $\GameTuple$ and sequence $\hat{\GameTuple}$ such that $\lim_{n \to \infty} \norm{\GameTuple - \hat{\GameTuple}_n}_\infty = 0$.  Then $\lim_{n \to \infty} \Anarchy (\GameTuple_n) = \Anarchy (\GameTuple)$.
\end{lemma}

We now present upper and lower bounds on the POA,
making no assumptions on $\GameTuple$.
%These bounds depend on other properties of the estimated game, and
The gap between these bounds can be arbitrary,
%but unlike for the previous estimator, 
but unlike for $\Anarchy (\GameTuple')$,
we can at least obtain a range in which the true POA is guaranteed to lie.
Before stating this result, we first show an intermediary.

\begin{lemma}[Unequivocal Anarchy Lemma]
\label{lemma:welfare-we}
If $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, then
\[
\inf_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\GameTuple')}\Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon \leq \inf_{\StratProfile \in \Nash^\diamond(\GameTuple)}\Welfare (\Utility, \StratProfile) \leq \sup_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\GameTuple')}\Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon \enspace.
\]
%\[
%\inf_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\GameTuple')}\Welfare (\Utility', \StratProfile) - N(\epsilon + \GameTuple) \leq \inf_{\StratProfile \in \Nash^\diamond(\GameTuple)}\Welfare (\Utility, \StratProfile) \leq \sup_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\GameTuple')}\Welfare (\Utility', \StratProfile) + N(\epsilon + \GameTuple) \enspace.
%\]
\end{lemma}

\begin{proof}
We show both inequalities in a single chain.
%
\begin{align*}
\inf_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\Gamma')} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon & \leq \inf_{\StratProfile \in \Nash^\diamond(\Gamma)} \Welfare (\Utility', \StratProfile) -\NumberOfPlayers\epsilon & \Nash^\diamond(\Gamma) \subseteq \Nash_{2\epsilon}^\diamond(\Gamma') \\
& \leq \inf_{\StratProfile \in \Nash^\diamond(\Gamma)} \Welfare (\Utility, \StratProfile) & \textsc{\cref{lemma:welfare}} \\
& \leq \sup_{\StratProfile \in \Nash^\diamond(\Gamma)} \Welfare (\Utility, \StratProfile) & \textsc{Infimum-Supremum Inequality} \\
& \leq \sup_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\Gamma')} \Welfare (\Utility, \StratProfile) & \Nash^\diamond(\Gamma) \subseteq \Nash_{2\epsilon}^\diamond(\Gamma') \\
& \leq \sup_{\StratProfile \in \Nash_{2\epsilon}^\diamond(\Gamma')} \Welfare (\Utility, \StratProfile') + \NumberOfPlayers\epsilon & \textsc{\cref{lemma:welfare}}
\end{align*}
\end{proof}

Note that it should be possible to refine the upper bound in some cases: for instance we should be able to prove that a true equilibrium exists within a particular region, even if we can't compute it.  Similarly, in the discrete case, in some cases an equilibrium in $\Gamma'$ is provably an equilibrium in $\Gamma$. \amy{let's discuss at some point}

\begin{theorem}[Unequivocal Anarchy Theorem]
\label{thm:anarchy-unequivocal}
If $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, then we bound the true price of anarchy, taking the RHS to be $\infty$ whenever its denominator is zero:
\[
\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\sup_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon} \leq \Anarchy (\GameTuple) \leq  \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\max(0, \inf_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) -\NumberOfPlayers\epsilon)} \enspace.
\]
\end{theorem}

\begin{proof}
The structure of this proof is to show upper and lower bounds on the numerator and denominator of the POA, which implies upper and lower bounds on the POA itself.  We have already shown these bounds in \cref{lemma:welfare} and \cref{lemma:welfare-we}, respectively.
\end{proof}

%, so subsequently we show conditions under which we may guarantee that the interval containing the POA tends to $0$ with $\epsilon$.

While this result provides hard guarantees on the estimated POA, it is rather unsatisfying, as for any $\epsilon > 0$, in the lower bound, we use the \emph{supremum\/} $2\epsilon$-Nash in the estimated game to upper-bound the \emph{infimum\/} (true) Nash in the true game.  This is necessary, \amy{it isn't necessary, per se, since we do something different in the next part.} because not all $2\epsilon$-Nash in the estimated game correspond to Nash in true game.  However, as the gap between the supremum and infimum may be arbitrarily wide, this is also a poor estimator.  We now remove this dependence on the supremum equilibrium welfare by making an additional assumption that ensures all equilibria are well-behaved.

\begin{lemma}[Conditional Anarchy Lemma]
\label{lemma:anarchy-conditional}
If $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, and $\forall \StratProfile \in \Nash^{\diamond}_{4\epsilon}(\GameTuple), \exists s' \in \Nash^{\diamond}(\GameTuple)$ such that $\abs{\Welfare (\Utility, \StratProfile) - \Welfare (\Utility, \StratProfile')} \leq \NumberOfPlayers\gamma$, \amy{$\gamma$ is unquantified} then
\[
\inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile') - \NumberOfPlayers\epsilon \leq \inf_{s \in \Nash(\GameTuple)} \Welfare (\Utility, s) \leq \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile') + \NumberOfPlayers(\epsilon + \gamma) \enspace.
\]
Furthermore, if $\forall \StratProfile \in \Nash_{4\epsilon}(\GameTuple)$, $\exists \StratProfile' \in \Nash(\GameTuple)$ such that $\norm{\StratProfile - \StratProfile'}_1 \leq \alpha$, and furthermore, $\sup_{\PlayerIndex, \StratProfile'', \StratProfile''' (adj)} \abs{\Utility_\PlayerIndex(\StratProfile'') - \Utility_\PlayerIndex(\StratProfile''')} \leq \beta$, then $\gamma \leq \alpha\beta$.

%Equivalently,
%\[
%\inf_{s \in \Nash(\GameTuple)} \Welfare (\Utility, s) - \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile') \in [-\NumberOfPlayers\epsilon, \NumberOfPlayers(\epsilon + \gamma)] \enspace.
%\]
\end{lemma}

\begin{proof}
We first derive the upper bound.
%
\begin{align*}
\inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare (\Utility, s) - \!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\! \Welfare (\Utility', \StratProfile') \hspace{-3cm} & \hspace{3cm} \leq \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare (\Utility, \StratProfile) - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! \Welfare (\Utility', \StratProfile') & \Nash_{2\epsilon}(\GameTuple') \subseteq \Nash_{4\epsilon}(\GameTuple) \\
& \leq \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare (\Utility, \StratProfile) - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! (\Welfare (\Utility, \StratProfile') - \NumberOfPlayers\epsilon) & \norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon \\
& \leq \!\! \inf_{\StratProfile \in \Nash_{4\epsilon}(\GameTuple)} \!\! (\Welfare (\Utility, \StratProfile) + \NumberOfPlayers\gamma) - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! (\Welfare (\Utility, \StratProfile') - \NumberOfPlayers\epsilon) = \NumberOfPlayers(\epsilon + \gamma) & \textsc{Assumption}
\end{align*}

\noindent
We next derive the lower bound, by showing that $\inf_{\StratProfile' \in \Nash(\GameTuple')} \Welfare (\Utility', \StratProfile') - \inf_{\StratProfile \in \Nash(\GameTuple)} \Welfare (\Utility, \StratProfile) \leq \NumberOfPlayers\epsilon$.
%
\begin{align*}
\inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\!\! \Welfare (\Utility', \StratProfile') - \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare (\Utility, \StratProfile) \hspace{-3cm} & \hspace{3cm} \leq \!\!\!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare (\Utility', \StratProfile') - \!\!\!\! \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare (\Utility, \StratProfile) & \Nash(\GameTuple) \subseteq \Nash_{2\epsilon}(\GameTuple') \\
& \leq \!\!\!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! (\Welfare (\Utility, \StratProfile') + \NumberOfPlayers\epsilon) - \!\!\!\! \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare (\Utility, \StratProfile) = \NumberOfPlayers\epsilon & \norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon
\end{align*}

\cyrus{We need to make sure these results hold both for pure and mixed equilibria.}
\amy{yes, we do. the hypothesis pertains to mixed eqa, but the proof and the result, as stated, pertain only to pure.}
\end{proof}

The next theorem shows that we can obtain finite-sample bounds on the POA that tighten with $\gamma$ and $\epsilon$.  

\begin{theorem}[Conditional Anarchy Theorem]
\label{thm:anarchy-conditional}
Assume the condition in \cref{lemma:anarchy-conditional}.
Suppose further that an equilibrium exists.
%, and also that $\inf_{\StratProfile \in \Nash(\GameTuple')} \Welfare (\Utility', \StratProfile) > \NumberOfPlayers\epsilon$ (to avoid division by 0 or vacuous lower bounds).  
Then (again resolving division by $0$ as $\infty$) we bound the POA as
\[
\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers(\epsilon + \gamma)} \leq \Anarchy (\GameTuple) \leq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\min(0, \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon)} \enspace.
\]
\end{theorem}

\begin{proof}
Following the structure of the proof of \cref{thm:anarchy-unequivocal}, 
\cref{lemma:welfare} implies bounds on the numerators,
and \cref{lemma:anarchy-conditional}, on the denominators.
%This result follows from bounding the set of possible ratios, given that the worst equilibrium welfare is bounded by \cref{lemma:anarchy-conditional}, and the difference between optimal welfares is bounded by \cref{lemma:welfare}.
\end{proof}

\amy{eqa are unstable. this content will likely be stated in intro/motivation sections, and can be deleted here.}
In general, estimating the price of anarchy is difficult: note that the price of anarchy of the empirical estimate $\hat{\GameTuple}$ isn't an estimator for the price of anarchy in $\GameTuple$, \emph{even if} $\norm{\GameTuple - \hat{\GameTuple}}_\infty \leq \epsilon$.  This is because equilibria are \emph{unstable}, in the sense that small changes to the utility function can add or remove equilibria.  

\fi

==> poa/old/very_old_poa.tex <==
\subsection{The Price of Anarchy}

\section{Price of Anarchy}
\cyrus{This probably belongs at the end of the game theory, immediately before the Rademacher complexity stuff, in its own subsection.  It motivates learning all, rather than just 1, equilibrium.  To my knowledge, existing techniques don't let us estimate this.}

\begin{definition}[Welfare]
Given a strategy profile $\StratProfile$ and utility function $\Utility$, the \emph{welfare} of $\StratProfile$ in $\Utility$ is defined as $\Welfare(\Utility, \StratProfile) \doteq \sum_{\PlayerIndex \in \SetOfPlayers} \Utility_\PlayerIndex(\StratProfile)$.
\end{definition}
\begin{definition}[The Price of Anarchy]
Given game $\GameTuple$ with utility function $\Utility$, the mixed \emph{price of anarchy} is defined as $A(\GameTuple) \doteq \frac{\sup_{\StratProfile' \in \StratProfileSpace}\Welfare(\Utility, \StratProfile')}{\inf_{\StratProfile \in \Nash^\diamond(\GameTuple)}\Welfare(\Utility, \StratProfile)}$.  The pure price of anarchy is similarly defined, with the infimum over the set of pure Nash equilibria.
\end{definition}

It is tempting to think that $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$ implies a bound on $\abs{A(\GameTuple) - A(\GameTuple')}$.  While the assumption does indeed imply a bound on the optimal welfare, it does not imply a bound on the worst equilibrium welfare.  Consequently, $A(\GameTuple)$ and $A(\GameTuple')$ may differ by an arbitrary amount, for any $\epsilon$.  To illustrate this point, consider that $\GameTuple$ may have an arbitrarily bad $0$-equilibrium that is only an $\frac{\epsilon}{2}$ equilibrium in $\GameTuple'$, and by symmetry we may overestimate or underestimate the welfare of the worst equilibrium, and thus the price of anarchy.  We refer to the estimation strategy of approximating $A(\GameTuple)$ with $A(\hat{\GameTuple})$, for some empirical estimate $\hat{\GameTuple}$, as the \emph{naive POA estimator}.  We now present bounds on the POA when no assumptions are made on $\GameTuple$; we then find them unsatisfying (as the interval that contains the POA may be arbitrarily wide for any $\epsilon$), so subsequently we show conditions under which we may guarantee that the interval containing the POA tends to $0$ with $\epsilon$.

\cyrus{Need to be consistent with pure / mixed games here.}

\begin{theorem}[Unequivocal Anarchy Theorem]
Suppose $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$.  Then
\[
A(\GameTuple) \in \left[\frac{\sup_{\StratProfile^* \in \StratProfileSpace} \Welfare(\Utility', \StratProfile^*) - \NumberOfPlayers\epsilon}{\sup_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\GameTuple)} \Welfare(\Utility', \StratProfile) + \NumberOfPlayers\epsilon}, \frac{\sup_{\StratProfile^* \in \StratProfileSpace} \Welfare(\Utility', \StratProfile^*) + \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\GameTuple)} \Welfare(\Utility', \StratProfile) -\NumberOfPlayers\epsilon}\right] \enspace.
\]

\todo{Need to handle division by 0.}
\end{theorem}
\begin{proof}

\cyrus{it's pretty straightforward, just upper and lower bounds on the worst equilibrium.}

\end{proof}

While this result provides hard guarantees on the estimated price of anarchy, it is rather unsatisfying, as for any $\epsilon > 0$, in the lower-bound, we use the \emph{supremum} $2\epsilon$-Nash in the empirical game to upper-bound the \emph{infimum} Nash in the true game.  This is necessary, because worse Nash in the empirical game may not correspond to Nash in true game, however the gap between the supremum and infimum may be arbitrarily wide for any $\epsilon > 0$, making this a poor estimator.  We now remove this dependence on the supremum equilibrium welfare by making an additional assumption that ensures equilibria are well-behaved.

\begin{lemma}[Anarchy Lemma]
\label{lemma:anarchy}
Suppose games $\GameTuple,\GameTuple'$ where $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, and $\forall \StratProfile \in \Nash^{\diamond}_{4\epsilon}(\GameTuple)$, exists $s' \in \Nash^{\diamond}(\GameTuple)$ such that $\abs{\Welfare(\Utility, \StratProfile) - \Welfare(\Utility, \StratProfile')} \leq \NumberOfPlayers\gamma$.  Then 
\[
\inf_{s \in (\GameTuple)} \Welfare(\Utility, s) - \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \Welfare(\Utility', \StratProfile') \in [-\NumberOfPlayers\epsilon, \NumberOfPlayers(\epsilon + \gamma)] \enspace.
%\inf_{\StratProfile \in \Nash(\GameTuple)} \Welfare(\Utility, s) - \inf_{\StratProfile' \in \Nash(\GameTuple')} \Welfare(\Utility', \StratProfile') \in [-\NumberOfPlayers\epsilon, \leq \NumberOfPlayers(\epsilon + \gamma)] \enspace.
\]
\end{lemma}
\begin{proof}

We first show an upper-bound on the difference.

\begin{align*}
\inf_{\StratProfile \in \Nash(\GameTuple) \!\! } \!\! \Welfare(\Utility, s) - \!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\! \Welfare(\Utility', \StratProfile') \hspace{-3.5cm}&\hspace{3.5cm}\leq \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare(\Utility, \StratProfile) - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! \Welfare(\Utility', \StratProfile') & \Nash_{2\epsilon}(\GameTuple') \subseteq \Nash_{4\epsilon}(\GameTuple) \\
 &\leq \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \Welfare(\Utility, \StratProfile) \!\! - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! (\Welfare(\Utility, \StratProfile') - \NumberOfPlayers\epsilon) & \norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon \\
 &\leq \!\! \inf_{\StratProfile \in \Nash_{4\epsilon}(\GameTuple)} \!\! (\Welfare(\Utility, \StratProfile) + \NumberOfPlayers\gamma) - \!\! \inf_{\StratProfile' \in \Nash_{4\epsilon}(\GameTuple)} \!\! \Welfare(\Utility, \StratProfile') - \NumberOfPlayers\epsilon = \NumberOfPlayers(\epsilon + \gamma) & \textsc{Assumption} \\
\end{align*}

\todo{Need to put justifications in text for 2-col layout.}

We now lower-bound the difference, by showing that $\inf_{\StratProfile' \in \Nash(\GameTuple')} \Welfare(\Utility', \StratProfile') - \inf_{\StratProfile \in \Nash(\GameTuple)} \Welfare(\Utility, \StratProfile) \leq \NumberOfPlayers\epsilon$.

\begin{align*}
\inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple') \!\!\! } \!\!\! \Welfare(\Utility', \StratProfile') - \!\! \inf_{\StratProfile \in \Nash(\GameTuple)} \!\! \Welfare(\Utility, \StratProfile) \hspace{-3cm} & \hspace{3cm} \leq \!\!\!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare(\Utility', \StratProfile') - \!\!\!\! \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare(\Utility, \StratProfile) & \Nash(\GameTuple) \subseteq \Nash_{2\epsilon}(\GameTuple') \\
 &\leq \!\!\!\! \inf_{\StratProfile' \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! (\Welfare(\Utility, \StratProfile') + \NumberOfPlayers\epsilon) - \!\!\!\! \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \!\!\!\! \Welfare(\Utility, \StratProfile) = \NumberOfPlayers\epsilon & \norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon \\
\end{align*}

\end{proof}

\begin{theorem}[Anarchy Theorem]
\label{thm:anarchy}
Suppose as in \cref{lemma:anarchy}, that an equilibrium exists, and also that $\inf_{\StratProfile \in \Nash(\GameTuple')} \Welfare(\Utility', \StratProfile) > \NumberOfPlayers\epsilon$ (to avoid division by 0 or vaccuous lower bounds).  Then the price of anarchy $A(\GameTuple)$ lies in the interval
\[
\left[\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare(\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare(\Utility', \StratProfile) + \NumberOfPlayers(\epsilon + \gamma)}, \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare(\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare(\Utility', \StratProfile) - \NumberOfPlayers\epsilon}\right] \enspace.
\]
\end{theorem}
\begin{proof}

This result follows from bounding the set of possible ratios, given that the worst equilibrium utility is bounded by \cref{lemma:anarchy}, and the optimal social welfare differs between $\GameTuple$ and $\GameTuple'$ by no more than $\NumberOfPlayers\epsilon$ than over $\GameTuple'$.

\end{proof}

\cyrus{We need to make sure the above 2 results hold both for pure and mixed equilibria.}

This result shows that we can obtain finite-sample bounds on the price of anarchy that tighten with $\gamma$ and $\epsilon$.  In general, estimating the price of anarchy is difficult: note that the price of anarchy of the empirical estimate $\hat{\GameTuple}$ isn't an estimator for the price of anarchy in $\GameTuple$, \emph{even if} $\norm{\GameTuple - \hat{\GameTuple}}_\infty \leq \epsilon$.  This is essentially because equilibria are \emph{unstable} in the sense that small changes to the utility function can add or remove equilibria (estimating the maximal-welfare on the other hand is trivial).  To ensure that no true equilibrium goes uncounted in $\GameTuple$, we instead consider the worst-case $2\epsilon$-equilibrium in $\hat{\GameTuple}$, which underestimates the welfare-minimizing equilibrium.  We also require the assumption that each $4\epsilon$-Nash equilibrium approximates (more specifically has approximately the same welfare as) a 0-Nash equilibrium, as this ensures we don't underestimate the welfare-minimizer too badly.

\cyrus{This plugs into GS rather nicely, but PSP doesn't give the guarantees we need.  We should mention that a modified PSP that keeps strategies that may be involved in the welfare-maximizing strategy profile can be used here.  We can also separately learn the optimal-welfare, which is just a bandit problem.}



\par\bigskip

Broader Plan: we can definitely estimate a sets that contain but are not much larger than the Pareto frontier, the Nash equilibria, and the maximal welfare.

\par\bigskip

Efficiency frontiers, and learning families of games.

Thus it's a family of games, and we can learn them all simultaneously
and I'm thinking now if the game is multivariate, and we assume our objective is a nonnegative linear combination, then we can estimate the covariances, and do the same thing
optimize $E[x . w] - \lambda V[x . w]$, which we estimate as $\hat{E}[x] w - \lambda w^T \hat{\Sigma}$.

This is closely related to mechanism design: we could show that for this class of games where scalar utilities are polynomial functions of the vector-valued utilities, we can simultaneously learn every possible game in the family, thus we can select the game that optimizes (welfare, equilibria, pareto frontier, POA; anything we show to be learnable [TODO: PAC learnable, right?]).  The connection between learnability of different concepts (like POA, maximum welfare, Pareto optimal frontier) and simultaneously learning a family of games is really cool to me.


Technically we're using uniform convergence to learn a deterministic game, then we show that we also learn the mixed game, but that seems a little less interesting, because we still have to sample everything a bunch of times.  The mechanism design part is really cool, because we don't even need to play the newly designed games.


In a simple setting, we learn (co)moments of a vector-valued utility game, and the mechanism design allows us to adjust a polynomial objective.  In the more sophisticated setting, we learn the distribution over vector-valued utilities and the mechanism design allows us to adjust a Lipschitz function.


I guess we don't even need that though, it just has to be Lipschitz continuous
so that approximate knowledge of the vector-valued distribution is preserved
well, actually, it's 2 different things.  Polynomial is nice, because then we just have to learn moments
(comoments)
but if we want to allow for arbitrary Lipschitz continuous functions, then we have to approximate the multivariate distribution over utility values (the CDF)
because specific combinations might have higher or lower rewards.

We probably need to assume bounded moments for the polynomial setting, and bounded variance or expectation for the Lipschitz setting (depending on whether or not the Lipscihtz function is also bounded).

Not everything has to be continuous; we could allow for mechanism spaces that have a finite set of discrete values, and an additional Lipschitz continuous set.  We then learn each discrete component (increasing the number of parameters learned, but not the sample complexity).

Alternatively, we could allow discrete or continuous parameters to modify the output distribution of the game.  It then becomes a learning problem over a discrete or continuous space, as we must learn over these parameters as well.  This raises similar issues to the learning continuous games setting.

\par\bigskip

Computing optimal mechanisms is probably a nightmare even in the polynomial case, and it might be hopeless in the Lipschitz case.  However, our contribution here is the statistics, not the optimization.

%it is difficult to estimate the price of anarchy, because for any $\gamma > 0$, it is possible for the worst equilibrium in $\GameTuple'$ to differ arbitrarily from the worst equilibrium in $\GameTuple$.  To combat this, we instead consider the worst $2\epsilon$-equilibrium in $\GameTuple'$, and require that all $4\epsilon$-equilibria in $\GameTuple$ have welfare approximately equal to a true equilibrium.  These conditions are sufficient to ensure that estimated worst-case welfare approximates true worst-case welfare.

\cyrus{We should also talk about learning minimax and CKR-optimal actions for each player, and show how to learn as many game-theoretic notions as we can.}

\subsection{On Optimal Strategies}

Unsurprisingly, given $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, it holds that minimax strategies in $\GameTulple'$ are $2\epsilon$-minimax in $\GameTuple'$, which are themselves $4\epsilon$-minimax in $\GameTuple$.

Unfortunately, like POA, it is substantially harder to estimate CKR strategies.  This is because a small change to the utility of player $a$ may cause a strategy for $a$ to switch between dominated and rationalizable, which can massively impact the worst-case CKR utility for player $b$.  I think we get a wide interval (arbitrarily large for any $\epsilon$) of potential CKR strategies (and their values).  What assumption can we may to prevent this?

\subsection{On Game Variances}

We can learn variances as well as expectation, and then we can estimate optimal actions under a utility that balances variance and expectation.

TODO: Undominated $\to$ rationalizable.

TODO: In addition to symmetric, talk about 0-sum?

==> poa/old/very_very_old_poa.tex <==
\iffalse
%This result is fine, but I think it's subsumed by the strong anarchy lemma.
\begin{lemma}[Weak Anarchy Lemma]
\label{lemma:weak-anarchy}
Suppose a pure-strategy game $\Gamma$ and take $\Gamma'$ such that $\norm{\Gamma - \Gamma'}_\infty \leq \epsilon$.  Suppose also that every $4\epsilon$ Nash-equilibrium of $\Gamma$ is also a Nash-equilibrium of $\Gamma$.  Then (for $w$ the welfare function) 
\[\abs{\inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E(\Gamma')} w(\bm{u}', s')} \leq N_p\epsilon \enspace.
\]
\end{lemma}
\begin{proof}

By \cref{lemma:mixed-approximation} and assumption, $E(\Gamma) \subeteq E_{2\epsilon}(\Gamma') \subseteq E_{4\epsilon}(\Gamma) \subseteq E(\Gamma)$, consequently $E_{2\epsilon}(\Gamma') = E(\Gamma)$.  Now:

\begin{align*}
\abs{\inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E(\Gamma)} w(\bm{u}', s')} &= \abs{\inf_{s \in E(\Gamma)} \sum_{p} \bm{u}_p(s) - \inf_{s' \in E(\Gamma)} \sum_p \bm{u}'_p(s')} \\
 &\leq \abs{\inf_{s \in E(\Gamma)} \sum_{p} \bm{u}_p(s) - \inf_{s' \in E(\Gamma)} \sum_p \bm{u}_p(s') \pm \epsilon} \leq N_p\epsilon & ? \\
 &= \abs{\sum_{p} \pm \epsilon} = N_p\epsilon \\
\end{align*}

\end{proof}
\fi

\begin{definition}[Welfare]
\end{definition}

\begin{lemma}[Anarchy Lemma]
\label{lemma:anarchy}
Suppose stochastic games $\Gamma,\Gamma'$ where $\norm{\Gamma - \Gamma'}_\infty \leq \epsilon$, and $\forall s \in \text{E}_{4\epsilon}(\Gamma)$, exists $s' \in \text{E}(\Gamma)$ such that $\abs{w(\bm{u}, s) - w(\bm{u}, s')} \leq N_p\gamma$.  Then 
\[
\inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s') \in [-N_p\epsilon, N_p(\epsilon + \gamma)] \enspace.
%\inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E(\Gamma')} w(\bm{u}', s') \in [-N_p\epsilon, \leq N_p(\epsilon + \gamma)] \enspace.
\]
\end{lemma}
\begin{proof}

We first show an upper-bound on the difference.

\begin{align*}
\inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s') \hspace{-2cm}&\hspace{2cm}\leq \inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E_{4\epsilon}(\Gamma)} w(\bm{u}', s') & E_{2\epsilon}(\Gamma') \subseteq E_{4\epsilon}(\Gamma) \\
 &\leq \inf_{s \in E(\Gamma)} w(\bm{u}, s) - \inf_{s' \in E_{4\epsilon}(\Gamma)} (w(\bm{u}, s') - N_p\epsilon) & \norm{\Gamma - \Gamma'}_\infty \leq \epsilon \\
 &\leq \inf_{s \in E_{4\epsilon}(\Gamma)} (w(\bm{u}, s) + N_p\gamma) - \inf_{s' \in E_{4\epsilon}(\Gamma)} w(\bm{u}, s') - N_p\epsilon = N_p(\epsilon + \gamma) & \textsc{Assumption} \\
\end{align*}

We now lower-bound the difference, by showing that $\inf_{s' \in E(\Gamma')} w(\bm{u}', s') - \inf_{s \in E(\Gamma)} w(\bm{u}, s) \leq N_p\epsilon$.

\begin{align*}
\inf_{s' \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s') - \inf_{s \in E(\Gamma)} w(\bm{u}, s) &\leq \inf_{s' \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s') - \inf_{s \in E_{2\epsilon}(\Gamma')} w(\bm{u}, s) & E(\Gamma) \subseteq E_{2\epsilon}(\Gamma') \\
 &\leq \inf_{s' \in E_{2\epsilon}(\Gamma')} (w(\bm{u}, s') + N_p\epsilon) - \inf_{s \in E_{2\epsilon}(\Gamma')} w(\bm{u}, s) = N_p\epsilon & \norm{\Gamma - \Gamma'}_\infty \leq \epsilon \\
\end{align*}

\end{proof}

\begin{theorem}[Anarchy Theorem]
\label{thm:anarchy}
Suppose as in \cref{lemma:anarchy}, that an equilibrium exists, and also that $\inf_{s \in E(\Gamma')} w(\bm{u}', s) > N_p\epsilon$.  Then the price of anarchy $A(\Gamma) \in \left[\frac{\sup_{s \in \bm{S}} w(\bm{u}', s) - N_p\epsilon}{\inf_{s \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s) + N_p(\epsilon + \gamma)}, \frac{\sup_{s \in \bm{S}} w(\bm{u}', s) + N_p\epsilon}{\inf_{s \in E_{2\epsilon}(\Gamma')} w(\bm{u}', s) - N_p\epsilon}\right]$
\end{theorem}
\begin{proof}

This result follows from bounding the set of possible ratios, given that the worst equilibrium utility is bounded by \cref{lemma:anarchy}, and the optimal social welfare differs between $\Gamma$ and $\Gamma'$ by no more than $N_p\epsilon$ than over $\Gamma'$.

\end{proof}

This result shows that we can obtain finite-sample bounds on the price of anarchy that tighten with $\gamma$ and $\epsilon$.  In general, it is difficult to estimate the price of anarchy, because for any $\gamma > 0$, it is possible for the worst equilibrium in $\Gamma'$ to differ arbitrarily from the worst equilibrium in $\Gamma$.  To combat this, we instead consider the worst $2\epsilon$-equilibrium in $\Gamma'$, and require that all $4\epsilon$-equilibria in $\Gamma$ have welfare approximately equal to a true equilibrium.  These conditions are sufficient to ensure that estimated worst-case welfare approximates true worst-case welfare.

\cyrus{I'd like to prove that estimating price of anarchy is hard in the general case.  Can we lower-bound the sample complexity?}

==> poa/poa_theory.tex <==
\section{Estimating the Price of Anarchy}
\label{sec:poa}

We now set out to investigate approximations of the price of anarchy~\cite{koutsoupias1999worst} that follow from uniform approximations of games.
The price of anarchy is a way of comparing the best-case welfare to the worst-case welfare at equilibrium.
%%% SPACE
%i.e., the value of the maximally dissonant equilibrium.
%%% SPACE
%In other words,
It is a measure of how bad things can get when there is no
%government
cooperation, in which case the alternative is taken to be worst-case equilibrium play.

Our first result is negative: price of anarchy is not well behaved.
Even given a uniform approximation of a game, we cannot derive a satisfactory bound on its price of anarchy, as we cannot derive a satisfactory bound on the value of its
maximally dissonant equilibria (see Observation~\ref{obs:inapproximable}), a key component of the price of anarchy.
Still, following Theorem~\ref{thm:extremeNash}, we can bound the price of anarchy both from above and below, albeit loosely from below, \amy{check old theorem. also loose on one side or the other? assumption only tightens one direction. which one?} and then, under the same stability condition, %Theorem~\ref{thm:bestNash}
the lower bound can be tightened.
But, as already noted, this condition is difficult to justify.
Instead, we propose an alternative quantity as a substitute 
%measure
for the traditional price of anarchy.

Our substitute measure for the price of anarchy alters the traditional measure in two ways.
First, we replace the maximally dissonant equilibrium value with the value of the maximally dissonant $\Lambda$-stable outcome, for some $\Lambda \ge 0$.
Second, we replace the division with subtraction.
We refer to the traditional price of anarchy measure as the \mydef{anarchy ratio}, by analogy with competitive ratio, and our new measure as the \mydef{anarchy gap}.
Although we use the term ``gap" rather than ``price,"
we note that price of anarchy is traditionally defined as a ratio, dividing one quantity by another; as such, it is dimensionless, and thus not technically a price.
When you subtract the two quantities, however, the units are preserved, so that the result would indeed be a price.
%(measured in, say, \emph{utils}).
%meaning units of utility, which could be interpreted in monetary terms

%This first change in the definition does not alter the spirit of the price of anarchy, only the letter, because as $\Lambda$ goes to infinity, the penalty for violating the constraints becomes infinite, so they are not violated at equilibrium.
%Further, when $\Lambda$ is finite, the definition can be understood as permitting small oscillations around equilibria, thus expanding the scope of acceptable play to strategy profiles near equilibria.

As in the case of extreme equilibria, the first change in the definition does not alter the spirit of the price of anarchy, only the letter.
%
The second change, in contrast, is more material; it can, however, by justified mathematically.
First and foremost, replacing the division with a subtraction eliminates the possibility of dividing by a very small quantity.
Together with the first change, this second change renders the anarchy gap a Lipschitz property (Theorem~\ref{thm:anarchy-gap}).
%, because $\Lambda$-stable outcomes are Lipschitz continuous in utilities. %%% AND because of the Lipschitz calculus
In contrast, the anarchy ratio is not Lipschitz, even when it is defined in terms of $\Lambda$-stable outcomes.
As a result, the anarchy gap is well behaved, and thus can be well estimated using statistical EGTA methodology, while the anarchy ratio is not, and thus cannot.

Additionally, the price of anarchy was originally defined for complete-information games, so it was natural to extend the definition to incomplete-information games by computing the price of anarchy of the corresponding normal-form game, as is done in the study of the price of anarchy in auctions~\cite{roughgarden2016price}.
%\amy{expand!}
Computing the price of anarchy in this way, however, means dividing the `expected value of the optimal social welfare' by `the expected value of the maximally dissonant equilibrium value', rather than defining the price of anarchy as the expected value of `the optimal social welfare divided by the maximally dissonant equilibrium value': i.e., taking expectations before dividing rather than after.
Because of the linearity of expectations, the disparity between these two potential definitions of anarchy in games of incomplete-information disappears in a measure that is defined via subtraction rather than division: i.e., in the anarchy gap.

We start our technical discussion by defining the
%traditional notion of 
price of anarchy \cite{koutsoupias1999worst}.

\begin{definition}[Anarchy Ratio]
%%% SPACE
%Given game $\GameTuple$ with utility function $\Utility$,
The \mydef{anarchy ratio} is defined as $\AnarchyRatio (\Utility) \doteq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile)}{\inf_{\StratProfile \in \Nash (\Utility)} \Welfare (\Utility, \StratProfile)} = \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile)}{\MaxDis (\Utility)}$.
%
Likewise, the stability ratio%
\footnote{Some define the stability ratio as the reciprocal of $\StabilityRatio (\Utility)$.} is defined as
$\StabilityRatio (\Utility) \doteq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile)}{\sup_{\StratProfile \in \Nash (\Utility)} \Welfare (\Utility, \StratProfile)} = \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility, \StratProfile)}{\MaxCon (\Utility)}$.
\end{definition}

%\amy{$\AnarchyRatio_{\Lambda} (\Utility) \doteq \AnarchyRatio_{\Lambda} (\Utility)$}
%\amy{$\AnarchyRatio_{\Lambda}^{\diamond} (\Utility) \doteq \AnarchyRatio_{\Lambda} (\Utility^{\diamond})$}

%Fix two compatible games
%%$\GameTuple$ and $\GameTuple'$ 
%characterized by utility functions $\Utility$ and $\Utility'$, and assume $\Utility'$ is an $\epsilon$-uniform approximation of $\Utility$.
%
As argued above, a uniform approximation $\Utility'$ of $\Utility$ implies a uniform approximation of the extreme welfare of $\Utility$---the term in the numerator of the anarchy ratio.
It does not, however, imply a uniform approximation of the welfare of an extreme equilibrium in $\Utility$ (see Observation~\ref{obs:inapproximable})---the term in the denominator.
%
Just as we bounded the values of extreme equilibria from above and below in Theorem~\ref{thm:extremeNash}, 
%the next theorem employs the same arguments to 
we bound the anarchy ratio (\Cref{thm:approxPrices}).
These results are related because the anarchy ratio is defined in terms of the maximally dissonant equilibrium value.

%%% NEW (rearranged for WINE) !!!
\if 0
\begin{restatable}{theorem}{thmApproxPrices}
[Approximating the Prices of Anarchy and Stability]
%Fix $\epsilon > 0$. Assume $\Welfare: \StratProfileSpace \times (\StratProfileSpace \to \R^{\NumberOfPlayers}) \to \R$ is monotonic non-decreasing so that $\Utility \preceq \bm{v}$ component-wise implies $\Welfare(\StratProfile; \Utility) \le \Welfare(\StratProfile; \bm{v})$, for all $\StratProfile \in  \StratProfileSpace$ and utilities $\Utility$ and $\bm{v}$.
Assume as in Theorem~\ref{thm:extremeNash}.
Then, so long as the numerator and denominator of each bound is positive, 
%we may bound the anarchy and stability ratios as
%
%\begin{equation*}
$\max \left\{ 1, \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility' - \epsilon, \StratProfile)}{\sup_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\Utility' + \epsilon, \StratProfile)} \right\} 
\leq \StabilityRatio (\Utility)
%\end{equation*}
%\begin{equation*}
\leq \AnarchyRatio (\Utility) 
\leq  \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility' + \epsilon, \StratProfile)}{\inf_{\StratProfile \in \Nash_{2\epsilon}(\Utility')} \Welfare (\Utility' - \epsilon, \StratProfile)}$.
%\enspace .
%\label{eq:POANaiveBounds}
%\end{equation*}
\label{thm:approxPrices}
\end{restatable}
\fi
%%% END NEW (rearranged for WINE) !!!

%%% OLD !!!
\if 0
\begin{equation}
\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\sup_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\Utility')} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon} \leq \AnarchyRatio (\Utility) \leq  \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash^\diamond_{2\epsilon}(\Utility')} \Welfare (\Utility', \StratProfile) -\NumberOfPlayers\epsilon} \enspace.
\label{eq:POANaiveBounds}
\end{equation}
\fi

\if 0
This implies an improved lower bound on the price of 
\[
\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon(1 + 2\gamma)} \leq \AnarchyRatio (\GameTuple) \enspace. %\leq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\min(0, \inf_{\StratProfile \in \Nash_{2\epsilon}(\GameTuple')} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon)} \enspace.
\]
\fi

\if 0
%Furthermore, we may show a weaker bound that does not require evaluating infima over sets of approximate Nash equilibria:
%\[
%\AnarchyRatio(\GameTuple')\frac{1 + \frac{N\epsilon}{.}}{1 + \}
%\]

This implies multiplicative error bounds on the quality of the empirical POA \cyrus{I need to figure out the details here.}
\[
\AnarchyRatio(\GameTuple)(1 - ?) \leq \AnarchyRatio(\GameTuple') \leq \AnarchyRatio(\GameTuple)(1 + ?) \enspace.
\]
\fi
%%% END OLD !!!

%%% NEW (rearranged for WINE) !!!
\if 0
\begin{restatable}{corollary}{corApproxPrices}
Assume as in Cor.~\ref{cor:extremeNash}.
%Suppose further that $\exists \gamma > 0$ s.t.\ $\forall \alpha > 0, \forall \StratProfile \in \Nash_{\alpha}(\Utility), \exists s' \in \Nash (\Utility)$ s.t.\ $\abs{\Welfare (\Utility, \StratProfile) - \Welfare (\Utility, \StratProfile')} \leq \alpha \gamma$.
%
\if 0
%Unfortunately, it's not true:
We may then bound the rate at which the difference between the worst equilibrium welfare in $\GameTuple$ and $\GameTuple'$ tends to 0 linearly in $\epsilon$
\[
\abs{\inf_{\StratProfile \in \Nash(\GameTuple)} \Welfare(\Utility, \StratProfile) - \inf_{\StratProfile' \in \Nash(\GameTuple')} \Welfare(\Utility', \StratProfile')} \leq \NumberOfPlayers\epsilon(1 + 2\gamma) \enspace.
\]
Consequently, we may bound the price of anarchy as
\[
\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) - \NumberOfPlayers\epsilon}{\inf_{\StratProfile \in \Nash^\diamond(\GameTuple')} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon(1 + 2\gamma)} \leq \AnarchyRatio (\GameTuple) \leq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility', \StratProfile) + \NumberOfPlayers\epsilon}{\max(0, \inf_{\StratProfile \in \Nash^\diamond(\GameTuple')} \Welfare (\Utility', \StratProfile) -\NumberOfPlayers\epsilon(1 + 2\gamma))} \enspace.
\]
\fi
%
We may then refine the lower bound, improving the supremum (i.e., maximally consonant) equilibrium value to an infimum (i.e., maximally dissonant), 
again so long as 
%the numerator and denominator are
the denominator is positive, 
as
%\begin{equation*}
$\frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility' - \epsilon, \StratProfile)}{\inf_{\StratProfile \in \Nash (\Utility')} \Welfare (\Utility' + \epsilon, \StratProfile) + 2 \gamma \epsilon} \leq \AnarchyRatio (\Utility)$.
%\enspace .
%\end{equation*}
Analogously,
%\label{eq:POABetterBounds}
%\end{equation}
%
%\begin{equation*}
$\StabilityRatio (\Utility) \leq \frac{\sup_{\StratProfile \in \StratProfileSpace} \Welfare (\Utility' + \epsilon, \StratProfile)}{\sup_{\StratProfile \in \Nash (\Utility')} \Welfare (\Utility' - \epsilon, \StratProfile) - 2 \gamma \epsilon}$.
%\enspace .
%\label{eq:POABetterBounds}
%\end{equation*}
\label{cor:approxPrices}
\end{restatable}
%%% END NEW (rearranged for WINE) !!!
\fi

%%% OLD !!!
\if 0
To see the second claim, we observe that by monotonicity,
$\sup_{\StratProfile \in \StratProfileSpace} \Welfare(\Utility' - \epsilon, \StratProfile) \leq \sup_{\StratProfile \in \StratProfileSpace} \Welfare(\Utility, \StratProfile)$, and
%\begin{align*}
\[
\inf_{\StratProfile \in \Nash (\Utility)} \Welfare(\Utility, \StratProfile) 
    \leq 
\inf_{\StratProfile \in \Nash_{2\epsilon} (\Utility)} \Welfare(\Utility, \StratProfile) + 2 \epsilon \gamma
    \leq 
\inf_{\StratProfile \in \Nash (\Utility')} \Welfare(\Utility, \StratProfile) + 2 \epsilon \gamma
    \leq 
\inf_{\StratProfile \in \Nash (\Utility')} \Welfare(\Utility' + \epsilon, \StratProfile) + 2 \epsilon \gamma
%\end{align*}
\]
where the first inequality is by assumption, with $\alpha = 2\epsilon$; 
the second follows because 
$\Nash (\Utility') \subseteq \Nash_{2\epsilon} (\Utility)$; and
the last, by monotonicity.
Using this bound in the denominator yields the result.
\fi
%%% END OLD !!!


==> poa/ppoa_est_algo.tex <==
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{PPOA-Estimation}{$\GameTuple, \ConditionDistribution$}

\State \Input \amy{inputs should be at least $\GameTuple$ and some noise}

\State \Output

\State Fix $\delta = 0.1$

\For{$m \in \{10, 20, 30, \ldots, 100\}$}

    \For{$t = 1, 2, \ldots 100$}
        %\State Use \GS{} to construct an estimate $\GameTuple'_t$ of $\GameTuple$ with $m$ samples.
        
        \State $\epsilon \gets \GS (m, \amy{etc.})$
        
        \State $L_t = L(\GameTuple'_t)$
        \amy{do you mean something like: $L_t = L(\GameTuple'_1, \ldots, \GameTuple'_t)$}
    \EndFor
    
    \State \Return $\nicefrac{1}{100} \left( \sum_{t=1}^{100} L_t \right)$, with 95\% confidence intervals around this mean

\EndFor

\EndProcedure
\end{algorithmic}

\cyrus{I'm not sure why we have this: PSP can be used for PPOA estimation?}

\caption{PPOA-Estimation}
\label{alg:PPOAEstimation}
\end{algorithm}

==> poa/ppoa_examples.tex <==
%\subsection{Examples: Congestion Games}

\begin{figure}[t!]
\centering
%\vspace{-0.25cm}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=6cm,height=6cm,keepaspectratio]{poa/PPOA1-Analytical.png}
  %\caption{Congestion Game 1}
  \label{fig:congestionGamesSub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=6cm,height=6cm,keepaspectratio]{poa/PPOA2-Analytical.png}
  %\caption{Congestion Game 2}
  \label{fig:congestionGamesSub2}
\end{subfigure}
\vspace{-0.25cm}
\caption{Monte Carlo estimates of the pure price of anarchy and the bounds in Equation~(\ref{eq:POANaiveBounds}) as a function of the number of samples needed to construct $\epsilon$-uniform approximations of congestion game $\GameTuple_1$ (a) and $\GameTuple_2$ (b) w.h.p. \enrique{$\delta = 0.1$}. We denote the lower and upper bounds by $L(\GameTuple)$ and $U(\GameTuple)$, respectively, and the true PPOA by $A(\GameTuple)$.}
\label{fig:congestionGames}
\end{figure}

Figure~\ref{fig:congestionGames} compares the quality of these Monte Carlo estimates as a function of the number of samples needed to construct a sequence of games, each of which $\epsilon$-uniformly approximates one of two congestion games (described below) with high probability.
We simulate noise in these congestion games as described in~\Cref{subsec:experimentalSetup}.
This figure was generated using Algorithm~\ref{alg:PPOAEstimation}.
(The algorithm as shown only estimates $L$, but estimation of $U$ and $M$ is analogous.)

The two congestion games are defined as follows:

\vspace{-2.5mm}

\paragraph{Congestion Game 1}, $\GameTuple_1$.
There are six facilities, which we label 0, 1, 2, 3, 4, and 5; and three agents, A, B, and C, each with sets of pure strategies given by: 
$\StrategySet_A = \{\{0, 3\}, \{1, 5, 4\}\}, 
 \StrategySet_B = \{\{1, 4\}, \{2, 3, 5\}\}, 
 \StrategySet_C = \{\{2, 5\}, \{0, 3, 4\}\}$.
We refer to these strategies in order and so, strategy 0 of agent $A$ consists of the set of facilities $\{0, 3\}$.
There are two pure Nash, $(0, 0, 0)$ and $(1, 1, 1)$.
The utilitarian welfare of $(0, 0, 0)$ is $- 2 - 2 - 2 = -6$, which is also the utilitarian-welfare-maximizing strategy profile.
%(in congestion games, agents try to minimize their cost, defined as the congestion of their chosen facilities).
The welfare of $(1, 1, 1)$ is $-3 (1 + 2 + 2) = -15$.
Hence, the pure price of anarchy is $\nicefrac{-6}{-15} = \nicefrac{2}{5}$, the worst possible price of anarchy for this class of games~\cite{christodoulou2005price}.

At the worst Nash equilibrium in this game, all agents are indifferent between playing their equilibrium strategy and unilaterally deviating.
Consequently, the na\"ive PPOA estimator, $M_0 (\GameTuple)$, shown in blue in Figure~\ref{fig:congestionGames} (a), fails to estimate the PPOA, even given an $\epsilon$-uniform approximation of $\GameTuple_1$ with high probability.
An alternative estimator, $M_{2 \epsilon} (\GameTuple)$, which considers all (pure) $2\epsilon$-Nash equilibria, is shown in yellow.
By Observation~\ref{obs:learnability}.
%By Theorem~\ref{thm:lipschitz-properties} (\ref{thm:lipschitz-properties:equilibria})
all equilibria of $\GameTuple_1$ are $2 \epsilon$-equilibria of a uniform approximation of $\GameTuple_l$ with high probability; hence, $M_{2 \epsilon} (\GameTuple)$ estimates the PPOA.

\vspace{-2.5mm}

\paragraph{Congestion Game 2} $\GameTuple_2$. 
There are again six facilities, but only two agents A and B.
The strategies sets are:
$\StrategySet_A = \{\{0, 3\}, \{1, 4, 5\}\}, 
\StrategySet_B = \{\{1, 4\}, \{2, 3, 5\}\}$.
In this game, there is a unique pure-strategy Nash equilibrium: $(0, 0)$ with welfare $-2(1 + 1) = -4$.
This outcome is also utilitarian-welfare maximizing. 
Hence, the pure price of anarchy is 1.
%%%
% Results
Moreover, the unique equilibrium is strong in the sense that agents strictly prefer their equilibrium strategy to all potential unilateral deviations.
Consequently, even the na\"ive estimator, $M_0 (\GameTuple)$, shown in blue in Figure~\ref{fig:congestionGames} (b), converges (almost immediately) to the PPOA, given an $\epsilon$-uniform approximation of $\GameTuple_2$ with high probability.


==> poker.tex <==

52-card deck.
deal 5 cards to each player with no replacement.
action space: discard one of five cards. left with four.
dealer draws 1 communal card from another complete deck.
player that wins is the player that makes the best hand.
according to Wikipedia rank.
tie on the rank is a draw: score is zero.


one hand of a game!
condition: draw from the dealer deck.
utility is random: depends on realization of the dealer.


nfg rep'n: 50 numbers. all rvs.


will always do at least as well as Hoeffding.
sample complexity will never be worse (up to something).
run lots of game conditions.
lots of cells with high variance;
or lots of cells with low variance.
any cells with 0 variance -- want to prune immediately.
high variance, they just hang around.
how to summarize the game: max variance (or sum of the variances)

(log 1000 * more work for 1000 high variance cells, instead of 1
(to control for multiple comparisons)

work:
- use sum, calls to simulator (for a fixed sample/condition)
- use max, sample conditions

drawing the card from the deck is negligible)


we don't know variance, but techniques work well whether or not we know anything about the variance a priori
- make it trickier, by having the dealer draw two cards


set # of iterations as follows:
1. ratio of largest / smallest sample size
2. log base 2 (or alpha) of this ratio (to produce doubling schedule) = number of iterations
key: # iterations cancels in the ratio



==> pruning_expts.tex <==
\begin{SCfigure}[1.5]
\begin{minipage}{3.2in} %2/3 * 6.5 = 13/3 \approx 4.333
\centering
\vspace{-0.25cm}
\begin{tikzpicture}
\begin{scope}[blend mode=darken]
\node (x) at (0, 0) {
%\null\hspace{-0.275cm}
\includegraphics[width=0.5\textwidth]{experiments/num_discard_cards_1}\hspace{-0.15cm}
\includegraphics[width=0.5\textwidth]{experiments/num_discard_cards_2}\hspace{-0.25cm}\null
};
\end{scope}
\end{tikzpicture}
\vspace{-0.75cm} \\
\end{minipage}
\caption{%\scriptsize
Experiments with Poker Games: sample and query complexities, discarding $1$ card (left) and $2$ cards (right) from a $5$ card hand. % deck.
%sample (\ref{fig:poker:sample}) and query (\ref{fig:poker:query}) complexities.
%Red $+$ denote, and blue $\times$ denote
Each dot represents the \emph{variance} and \emph{query/sample} complexity of a single randomly sampled game instance.
Blue denotes the high-card tiebreaker games (higher variance), and red denotes the non-tiebreaking (lower variance) games.
In all plots, the upper solid line denotes the upper-bound on sample or query complexity of \Cref{thm:efficiency}, while the lower dashed
line denotes the corresponding lower bound (see~\Cref{sec:psp}), and the (flat) dotted line denotes the Hoeffding complexity bound (see~\Cref{thm:hoeffding-sc}), which is independent of variance.
Each plot depicts 150 randomly sampled games for both tiebreaking and non-tiebreaking games.
}
\label{fig:poker}
\end{SCfigure}

\if 0
\begin{figure}
\centering
\begin{subfigure}{0.40\textwidth}%{0.45\textwidth}
%\includegraphics[width=\textwidth]{experiments/cards7}
\includegraphics[width=\textwidth]{experiments/num_discard_cards_1}
\caption{Sample Complexity}
\label{fig:poker:sample}
\end{subfigure}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{0.40\textwidth}%{0.45\textwidth}
%\rotatebox{180}{\includegraphics[width=\textwidth]{experiments/cards7}}
\includegraphics[width=\textwidth]{experiments/num_discard_cards_2}
\caption{Query Complexity}
\label{fig:poker:query}
\end{subfigure}
\caption{Experiments with Poker Games: sample and query complexities, discarding $1$ and $2$ cards from a $5$ card deck. %sample (\ref{fig:poker:sample}) and query (\ref{fig:poker:query}) complexities.
%Red $+$ denote, and blue $\times$ denote 
Red denotes the high-card tiebreaker games (150 runs), and blue denotes the non-tiebreaking (lower variance) games (150 runs).
In all plots, the solid line denotes the upper-bound on sample / query complexity of the previous section.
}
\cyrus{Fix order issues, show upper / lower bounds.}
\label{fig:poker}
\end{figure}
\fi

\todo{
\begin{itemize}
\item experiments so far show: linear relationship b/n variance and complexity; very clear!
\item plotting blue (high variance) as well as red (low) would let us plot more of this linear relationship.
\item high- vs.\ low-variance games. wanted to explore range of possible variances. low-variance games should have lower complexity than the high-variance ones, but we cannot really see that right now. \\
\emph{plot without full opacity! make translucent.}
\item $\beta$ closer to 1, makes for smaller steps. $\beta=2$, makes for much bigger steps. large step sizes implies loose bound by factor up to $\beta$. \\
\emph{VARY/optimize the $\beta$ hyperparameter!} 
\item experiments so far show: bound is correct, and looks pretty tight as well...need to add lower bounds to the picture -- but they are over worst-case distributions, not universal.
\emph{cannot really plot competitive ratio, b/c of divide by zero. but should probably subtract out lower bounds, to show EXCESS work: i.e., subtract lower bound.}
\item report table with additional statistics: e.g.,
\begin{itemize}
\item failures, when bounds fail (b/c only high probability guarantee) -- sample/query complexity bounds never failed!
\item never checked correctness; that all approximations are within given $\epsilon$
\item number of pruned vs.\ unpruned strategy profiles
\item number of iterations?
\end{itemize}
\item Use gambit games; sample conditions using the nature player.
\end{itemize}
}

\paragraph{Experiments}
\label{sec:well_estimated_pruning_experiments}

We present experiments on a family of synthetic poker games to validate our algorithm and visualize the sharpness of our sample and query complexity bounds.

Each game represents the play of a single hand of poker.
In this game, each player holds a \emph{fixed hand} consisting of $n$ cards.
As their action, they each choose $k$ cards to discard, simultaneously.
The randomness of the game then consists of the dealer drawing $d$ cards, and placing them face up on the table.
Each player is scored based on their remaining hand and the dealer cards.
The higher-scorer wins 1 point, while the lower-scorer loses 1 point, with neither player scoring any points in case of ties.
We play with a standard 52 card deck, scoring 5-card hands, thus we require $n - k + d = 5$.
Hands are ranked according to the \href{https://en.wikipedia.org/wiki/List_of_poker_hands}{standard rules of poker} (i.e., in rank-order: straight flush, four of a kind, full house, flush, straight, three of a kind, two pairs, one pair).
We use two variants: in one, a high-card breaks ties; in the other, there is no tie breaker.
The former variant produces fewer ties than the latter, and consequently, higher variance games.
%The latter variant produces many more ties than the former, and consequently, lower variance games.

In \Cref{fig:poker}, we plot the total number of samples and queries required by \Cref{alg:psp} for randomly selected poker games (poker hands), with $n=5,k=1,d=1$ and $n=5,k=2,d=2$.
All experiments use $\varepsilon = 0.01$ and $\delta = 0.05$.
We observe that empirical sample consumption is always quite near to its upper-bound, but not once in 600 total runs was the bound violated.

We also plot the sample and query complexities of using a simple Hoeffding union bound (horizontal dotted line) in all cases.
We find that sample is quite large (near maximal) in many of these games, i.e., there exists a strategy profile for which winning or losing is a coin-toss. 
%the variance is close to 1, which is the max. therefore, 
As a result, our algorithm often does not improve upon Hoeffding for sample complexity.
For query complexity, even if the maximum variance is large, i.e., $\norm{\UtilityVariance}_{\infty} \approx 1$, since many profiles have much smaller variance, i.e., $\norm{\UtilityVariance}_{1, \infty}$ is not near-maximal, our algorithm often outperforms the Hoeffding bound.
In particular, we see better performance in the case of discarding 1 rather than 2 cards, as more discarding leaves more up to chance, and leading to higher-variance utilities.

%\cyrus{We observe that the upper bounds on sample and query complexity are sharp; during a total of X simulations the bound is violated y x times with our choice of $\delta$ we would expect no more than Z violations.}
%\amy{it was never violated, so we need to run many many more experiments for them to be violated}


==> rademacher.tex <==
\subsection{Rademacher Averages}
\label{section:concentration:rademacher}

%\cyrus{The PSP algorithm is based on earlier work in progressive sampling \citep{elomaa2002progressive,riondato2015mining,riondato2018abra}, but I think this point was somehow lost.}
%\amy{moved to related work}

Because Hoeffding's inequality assumes only bounded noise, it is often a loose bound, particularly for random variables that are tightly concentrated in a relatively small region of their domain.  
%Traditional multiple-comparisons correction procedures (such as the Bonferroni or \v{S}id\'{a}k procedures) introduce an $\mathcal{O}(\sqrt{\ln \abs{\UtilityIndices}})$ factor on confidence interval widths, which compounds this looseness.
Theorem~\ref{thm:Hoeffding} and Section 4.2 in~\cite{tuyls2018generalised} both use Hoeffding's inequality to first bound individual utilities, and then combine those individual bounds using a statistical correction procedure (i.e., Bonferroni and \v{S}id\'{a}k, respectively).  Unfortunately, these corrections amplify the errors: e.g., Theorem~\ref{thm:Hoeffding} requires an $\smash{\mathcal{O}(\sqrt{\ln \abs{\UtilityIndices}})}$ factor increase in the widths of the confidence intervals.

%Intuitively, Rademacher averages resemble permutation tests, but with appropriate assumptions, they yield rigorous generalization bounds.

In contrast, Rademacher averages---which
%%(\emph{a.k.a.\/} Rademacher complexity),
intuitively resemble permutation tests---bound
%but with appropriate assumptions, yield rigorous generalization bounds---bound
the deviation between (potentially infinitely) many utilities and their expectations directly.
%, using a single concentration inequality, and an additional data-dependent term.
\if 0
Rademacher averages, in contrast,
%which have been proposed as a solution to the multiple comparisons problem,
%from the theory of uniform convergence (see, for example, \cite{bartlett2002rademacher}), 
allows us to directly obtain simultaneous confidence intervals about all utilities, because instead of combining the results of many independent hypothesis tests, they essentially test (potentially infinitely) many hypotheses all at once.
\fi
%It thus has the potential to remove this $\mathcal{O}(\sqrt{\ln \abs{\UtilityIndices}})$ factor.
%\amy{closely related to multiple hypothesis testing: e.g., test if a few strat profiles are eqa; instead of trying to bound a bunch of things separately, it handles everything at once (even infinitely many things).}
%\amy{imagine you want to estimate the max expected value of 100 fns. could estimate exp value of all, and then take the largest one. you'd need a union bound. or, could directly estimate the exp value of the max, only! much less info. just one quantity. can be estimated using McDiarmid's inequality.}
For very large games, a Rademacher-based approach can yield bounds that are significantly tighter than classical methods.
%(see Remark~\ref{rem:size}).  
For small and medium-sized games, however, they are often looser.  Nonetheless, we show that under natural conditions, they are never looser by more than a constant factor.
%\amy{where is this shown? in the appendix?}
%\enrique{This is now argue for right after Theorem 3.7}

There are two equivalent definitions of Rademacher averages, one with families of \emph{sets}, which is often more natural for unsupervised learning problems, and one with families of \emph{functions}, which is usually more convenient for supervised learning.  We present yet a third, isomorphic, definition, which facilitates the analysis of expected normal-form games.

\begin{comment}
We mostly concern ourselves with \emph{scalar-valued games}, as we are interested in the analysis of scalar-equilibria. However, sometimes it is more convenient to work with vector-valued games, and given any function $\phi$ from $\R^m \to \R$, we can convert a vector-valued game to a scalar-valued game, by applying $\phi$ to the vector-utility to produce a scalar, and analyze it as desired.  This is of great practical use; to illustrate thrice, consider first perhaps a single resource is valued, but we don't know which a priori, thus we must learn the game for each, and later we take $\phi$ to be an indicator function, consider second a case where the relative value of each resource is unknown a priori, thus we take $\phi$ to be a linear function, and consider thirdly, perhaps our agents are risk-averse, and wish to consider not just expected payoffs but also their variances: here we could estimate \emph{means} $\mu$ and \emph{raw variances} $\sigma^2_r$, then $\phi$ could be a 2-argument function that t of the form $\phi(\mu, \sigma^2) = \mu - \lambda(\sigma^2_r - \mu^2)$ (mean-variance analysis), $\phi(\mu, \sigma^2) = \mu - \lambda\sqrt{\sigma^2_r - \mu^2}$ (Chebyshev tail bound), or $\phi(\mu, \sigma^2) = \frac{\mu}{\sqrt{\sigma^2_r - \mu^2}}$ (Sharpe ratio).
\end{comment}

\begin{comment}
With the expected game framework well-defined, our sampled games framework is now on rigorous footing.  We now define the \emph{Rademacher averages} of an expected statistical game.
\end{comment}

\begin{definition}[Rademacher Averages of Expected Normal-Form Games]
Consider a conditional normal-form game $\ConditionalGame{\ConditionSpace}$ together with distribution $\ConditionDistribution$ and take index set $\UtilityIndices \subseteq \SetOfPlayers \times \StratProfileSpace$.  Suppose $\smash{\Samples \doteq (\SamplePoint_1, \ldots, \SamplePoint_{\NumberOfSamples}) \distributed \ConditionDistribution^\NumberOfSamples}$, and take $\smash{\vsigma \distributed \Rademacher^\NumberOfSamples}$; the Rademacher distribution is uniform on $\pm 1$.  We define:

\begin{enumerate}

\begin{comment}
\item \textbf{Empirical Maximum Discrepancy} (EMD): Suppose $2 | \NumberOfSamples$, then \\ $\EMD{\NumberOfSamples}{\GameTuple,\StratProfileSpace'}{\Samples} \doteq \sup_{\StratProfile\in\StratProfileSpace',\PlayerIndex\in\SetOfPlayers} \frac{1}{\NumberOfSamples}\sum_{\SampleIndex = 1}^\NumberOfSamples (-1)^\SampleIndex \Utility_{\PlayerIndex}(\StratProfile ; \SamplePoint_\SampleIndex)$.

\amy{Cyrus, why don't we define
maximum discrepancy, taking expectations %
$\MD{\NumberOfSamples}{\GameTuple,\StratProfileSpace'}{\ConditionDistribution} \doteq \Expwrt{\Samples}{\EMD{\NumberOfSamples}{\GameTuple, \StratProfileSpace'}{\Samples}}$
%
we don't use ERA or RA in our exp'ts. so we don't need them, except in theory. why isn't MD of interest likewise, if the EMD bound is better than the 1-ERA bound?}

\cyrus{Amy, you are correct.  The MD is to the EMD as the RC is to the 1-ERC.  We don't really need all of these concepts, we can pick either the EMD or the 1-ERC.  Right now I'm leaning toward the 1-ERC and the RC, because it is better-known, and it's usually easier to prove stuff about it.  }
\enrique{in the definition of EMD we have no absolute values but our proof of lemma 1 is about the absolute value of EMD. Actually, same observation applies for RC}

\end{comment}

\item \textbf{1-Draw Empirical Rademacher Average} (1-ERA):
$\DERC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\Samples}{\vsigma} \doteq \sup\limits_{(\PlayerIndex, \StratProfile) \in \UtilityIndices} \Big\lvert \frac{1}{\NumberOfSamples}\sum_{\SampleIndex = 1}^\NumberOfSamples \vsigma_\SampleIndex \Utility_{\PlayerIndex}(\StratProfile ; \SamplePoint_\SampleIndex) \Big\rvert$

%\item \textbf{Empirical Rademacher Average} (ERA): $$\ERC{\NumberOfSamples}{\GameTuple,\StratProfileSpace'}{\Samples} \doteq \Expwrt{\vsigma}{\DERC{\NumberOfSamples}{\GameTuple,\StratProfileSpace'}{\Samples}{\vsigma}}$$

\item \textbf{Rademacher Average} (RA):
$\RC{\NumberOfSamples}{\GameTuple,\UtilityIndices}{\ConditionDistribution} \doteq \Expwrt{\Samples,\vsigma}{\DERC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\Samples}{\vsigma}}$
\end{enumerate}

\end{definition}

%Don't need these anymore, since we prune by strategy profile.
%Additionally, we omit the $\StratProfileSpace'$ argument, which is used to take a Rademacher average over a subset of the strategy profile space, when $\StratProfileSpace' = \StratProfileSpace$.

Observe that the 1-ERA can be computed exactly from one draw of $\Samples$ and $\vsigma$, whereas computing the RA involves taking an expectation over these random variables.  The RA is used to obtain tail bounds on the quality of estimates, but since the ERA is tightly concentrated about the RA, the ERA can also be used for this purpose.

%With EMD:
%While each of the above varies slightly, the EMD is in expectation less than the 1-ERC, which is by definition equal in expectation to the ERC and the RC. Furthermore, all are tightly concentrated about one another \cite{bartlett2002rademacher}, so it makes little difference which we compute.  We now present bounds on uniform convergence between empirical expected games and true expected games.

\begin{theorem}[Finite-Sample Rademacher Bounds for Expected Normal-Form Games]
Consider conditional normal-form game $\ConditionalGame{\ConditionSpace}$ together with distribution $\ConditionDistribution$ and index set $\smash{\UtilityIndices \subseteq \SetOfPlayers \times \StratProfileSpace}$ such that for all $\smash{\ConditionValue \in \ConditionSpace}$ and $\smash{(\PlayerIndex, \StratProfile) \in \UtilityIndices}$, it holds that $\smash{\Utility_{\PlayerIndex}(\StratProfile; \ConditionValue) \in [-{\nicefrac{\UtilityRange}{2}}, {\nicefrac{\UtilityRange}{2}}]}$, 
where $c \in \mathbb{R}$.
%and take $\smash{\eta \doteq \sqrt{\nicefrac{\ln(\slfrac{1}{\delta})}{2\NumberOfSamples}}}$ and $\smash{d \doteq \sqrt{\nicefrac{\ln(2\abs{\UtilityIndices})}{2\NumberOfSamples}}}$.
Then, with probability at least $\smash{1 - \delta}$ over $\smash{\Samples \distributed \ConditionDistribution^\NumberOfSamples}$, we may bound 
%the deviation between $\Utility(\cdot; \ConditionDistribution)$ and $\hat{\Utility}(\cdot; \Samples)$ over all $\smash{(\PlayerIndex, \StratProfile) \in \UtilityIndices}$ 
$\smash{\norm{\GameTuple_{\ConditionDistribution} - \hat{\GameTuple}_{\Samples}}_{\!\infty}}$ with the 1-ERA and the RA, respectively, as:
%
\begin{enumerate}
\item
$\displaystyle \sup_{(\PlayerIndex, \StratProfile) \in \UtilityIndices} \abs{\Utility_{\PlayerIndex} (\StratProfile; \ConditionDistribution) - \hat{\Utility}_{\PlayerIndex} (\StratProfile; \Samples)} \leq 2\DERC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\Samples}{\vsigma} + 3\UtilityRange\sqrt{\frac{\ln\left(\nicefrac{1}{\delta}\right)}{2\NumberOfSamples}}$

\item
$\displaystyle
\sup_{(\PlayerIndex, \StratProfile) \in \UtilityIndices} \abs{\Utility_{\PlayerIndex} (\StratProfile; \ConditionDistribution) - \hat{\Utility}_{\PlayerIndex} (\StratProfile; \Samples)} \leq 2\RC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\ConditionDistribution} + \UtilityRange\sqrt{\frac{\ln\left(\nicefrac{1}{\delta}\right)}{2\NumberOfSamples}} \leq \UtilityRange \sqrt{\frac{\ln(\abs{\UtilityIndices})}{2\NumberOfSamples}} + \UtilityRange\sqrt{\frac{\ln\left(\nicefrac{1}{\delta}\right)}{2\NumberOfSamples}}$
\end{enumerate}
\label{thm:Rademacher}
\end{theorem}

A proof of~\Cref{thm:Rademacher} appears in~\Cref{sec:proofs}.

Observe that the 1-ERA bound, Theorem~\ref{thm:Rademacher} (1), has no explicit dependence on the number of parameters $\abs{\UtilityIndices}$ being estimated; thus, unlike a correction-based approach, this bound can scale to arbitrarily large games (including infinite games) without necessarily incurring additive error $\Omega(\sqrt{\ln{\abs{\UtilityIndices}}})$.
%\amy{why $\Omega$, not $O$? also, why additive?} \cyrus{$\Omega$ because it's a lower bound, additive because it's an additive error bound.  we want to say that, with appropriate structure, it is possible to \emph{not} incur this additive error term.}
Moreover, the upper bound on the RA, Theorem~\ref{thm:Rademacher} (2), shows that the Rademacher bounds are never asymptotically worse than those obtained via Theorem~\ref{thm:Hoeffding}.

On the other hand, the 1-ERA is a data-dependent quantity; thus, it does not yield strong \emph{a priori\/} bounds.  Still, the 1-ERA bound %$\smash{\displaystyle 2\DERC{\NumberOfSamples}{\GameTuple, \UtilityIndices}{\Samples}{\vsigma} + 3\UtilityRange\eta}$
can be much tighter
than the RA upper bound, in which case the bounds of Theorem~\ref{thm:Rademacher} may outperform those of Theorem~\ref{thm:Hoeffding}.
For example, when utility values are \emph{correlated} with respect to $\ConditionDistribution$, then the supremum is over 
%the absolute value of
%\amy{i prefer to delete mention of the absolute value. is this very bad? b/c if we say it once, we should really say it twice.}
correlated variables, which is generally smaller than a supremum over 
%the absolute value of
uncorrelated variables---strongly correlated sets of variables behave like single variables in the supremum.  Even under anticorrelation, as in constant-sum games, we obtain this benefit, due to the absolute value in the 1-ERA definition.  Additionally, if some $\smash{(\PlayerIndex, \StratProfile) \in \UtilityIndices}$ experience more noise than others, the low-noise UtilityIndices should have a small effect on the 1-ERA, as they are less likely than high-noise UtilityIndices to realize the supremum.
%Even if it is now known \emph{a priori} that these properties hold, we expect the 1-ERA to be small, and correspondingly expect tighter bounds 
%%than in the general case.
%than the theorem suggests.

In \Cref{sec:comparingBounds}, 
%we discuss cases, specifically factored games and games with variable-scale noise, where the 
%%Rademacher
%bounds of \Cref{thm:Rademacher} are significantly tighter than those of \Cref{thm:Hoeffding}.
we design stylized games with particular properties for which we can prove that the 
%Rademacher
bounds of \Cref{thm:Rademacher} are significantly tighter than those of \Cref{thm:Hoeffding}.  Crucially, this performance holds regardless of whether it is known \emph{a priori} that such properties hold.  Consequently, the Rademacher bounds are an attractive choice when we suspect a game is well-behaved, but have insufficient \emph{a priori\/} knowledge to prove it possesses any particular property that would imply strong statistical bounds, as is typical of the simulation-based games analyzed using EGTA.  

\begin{remark}
\label{rem:size}
The second bound in Theorem~\ref{thm:Rademacher} tells us that the Rademacher bounds are never asymptotically worse than those obtained via Theorem~\ref{thm:Hoeffding}.  Their small-sample performance, however, is inferior.  Indeed, we can derive the minimum game size in which the former may outperform the latter by setting $c\sqrt{\nicefrac{\lnp{2\abs{\UtilityIndices}/\delta}}{2m}} = 3c\sqrt{\nicefrac{\lnp{1/\delta}}{2m}}$, and solving for $\abs{\UtilityIndices}$.
%which gives $\ln(2\abs{\UtilityIndices}/\delta) = 9\ln(1/\delta)$, thus $\abs{\UtilityIndices} = \frac{e^8}{2\delta}$.
Doing so yields $\abs{\UtilityIndices} = \nicefrac{1}{2\delta^8}$.  Taking $\delta = 0.1$, we obtain a minimum $\abs{\UtilityIndices}$ of $5 \times 10^7$.  Solving games of this magnitude is not entirely out of reach, even today, and with future increases in computing power, the asymptotic efficiency of the Rademacher bounds will only become more attractive.
\end{remark}

\begin{comment}
%\enrique{Thank you very much for the full derivation!, I don't think we need it for the arxiv, so I am commenting it out}
\cyrus{Full derivation: $c\sqrt{\nicefrac{\lnp{2\abs{\UtilityIndices}/\delta}}{2m}} = 3c\sqrt{\nicefrac{\lnp{1/\delta}}{2m}} \implies \lnp{2\abs{\UtilityIndices}/\delta} = 9\lnp{1/\delta} \implies \lnp{2\abs{\UtilityIndices}} + \lnp{1/\delta} = 9\lnp(1/\delta) \implies \lnp{2\abs{\UtilityIndices}} = 8\lnp{1/\delta} \implies \abs{\UtilityIndices} = \frac{1}{2\delta^8}$}
\end{comment}

\begin{comment}
\cyrus{I simplified the above result a lot, worrying about $c$ versus $c'$ seemed like a lot of complexity for little payoff.}
\enrique{With the simplification, I don't think the next paragraphs applies}.
The difference between $\UtilityRange$ and $\UtilityRange'$ is a bit subtle: $\UtilityRange$ is the \emph{range} of utility values permitted by the restriction of the conditional game $\GameTuple$ onto $\support(\ConditionDistribution)$, whereas $\UtilityRange'$ is the maximum amount of \emph{deviation} possible for any utility value between any pair of conditions $\ConditionValue, \ConditionValue' \in \support(\ConditionDistribution)$.  By construction, $\UtilityRange' \leq \UtilityRange$, and substantially so, when the utilities for any given strategy profile can't vary much under arbitrary conditions, but changing the strategy profile can produce large changes to utilities.  The EMD depends on $\UtilityRange$' rather than $\UtilityRange$, as the EMD is inherently \emph{centered} (by which we mean adding any constant to the utility function produces no change to the EMD, as an equal number of positive and negative terms are always subtracted), whereas the 1-ERC, ERC, and RC are not.  This suggests that, practically, the EMD bounds are superior, though as they give no theoretical insight, analytically, the RC bounds are superior.  Furthermore, as the EMD is tightly concentrated about the RC, the analytical RC bound ensures that worst-case performance of the EMD bound isn't too bad.
\end{comment}

\begin{comment}
%I'm not sure we'll figure out a satisfying way to do this before the deadline:
While these bounds are elegant, and provide us with finite-sample $\epsilon$-$\delta$ guarantees, often they are impractical, as they require that $c$ or $c'$ is \emph{bounded}, and indeed, that it is known \emph{a priori}.  Even in the simple case of payoffs with Gaussian noise, this assumption does not hold.  We now present \emph{asymptotic} $\epsilon$-$\delta$ guarantees that perform reasonably well for reasonably-sized samples and do not assume bounded rewards.
\end{comment}

\begin{remark}
While estimating an arbitrary game requires estimating $\smash{\NumberOfPlayers\prod_{i=1}^{\NumberOfPlayers}|\StrategySet_\PlayerIndex|}$ parameters, many games are defined by far fewer parameters.
\mydef{Symmetric games}, for example, where all agents' strategy sets are identical, and utilities depend only on the strategy an agent chooses and the \emph{number\/} of other agents that choose each strategy (not the agents' identities), can be substantially smaller.
Learning such games is easier; as fewer parameters need to be estimated, we can obtain tighter statistical bounds from the same number of samples.  
% Commenting out for ArXiv version, could revisit this later. 
%\todo{Connect this remark to the concept of index set (to motivate index sets).}
\end{remark}

\begin{remark}
Rademacher and Hoeffding bounds are just two possible choices of concentration inequalities.  Both require bounded noise, but this is not an inherent limitation of our approach.
We could obtain similar results under varied noise assumptions; e.g., we could assume (unbounded) subgaussian or subexponential noise, and substitute the appropriate Chernoff bounds.
%, which would be a major limitation of our work as compared to many empirical game theory papers, which often assume Gaussian noise.
%In this sense, our theory is relevant to prior work on empirical games that assumed Gaussian noise.
%\cyrus{Enrique: can you cite the relevant papers for the Gaussian assumption?  I believe most of Wellman's work assumes this?}
\end{remark}


==> related_work.tex <==
%THE NEW PAPER IS MUCH MORE EXTENSIVE THAN OLD, LEARNING MANY THINGS BEYOND EQA. MY FEELING IS THAT IF WE INCLUDE THIS PARAGRAPH, REVIEWERS COULD INTERPRET OUR WORK AS ONLY CONCERNING EQA, WHICH SEVERELY LIMITS ITS APPLICABILITY

\paragraph{Related Work}

The goal of empirical game-theoretic analysis is to solve games that are not directly amenable to theoretical analysis because they can be described only by repeatedly querying a simulator, and even then their description is necessarily noisy.
Most EGTA methods work by first estimating utilities to construct an empirical game, and then computing an approximate Nash equilibrium of that game.
One approach to estimating utilities is to sample a few strategy profiles, and then learn from those observations functions that generalize utilities to unseen data~\cite{vorobeychik2007learning,wiedenbeck2018regression}.
Another line of work proposes sampling heuristics based on, for example, information-theoretic 
principles~\cite{walsh2003choosing}, or variance reduction techniques in games with stochastic outcomes where agents employ mixed strategies~\cite{burch2016aivat}. 
To handle particularly complex games, hierarchical game reduction~\cite{wellman2006methods} can be used to reduce the size of the game. 
Recently, EGTA has been successfully applied in games with very large strategy spaces, like StarCraft~\cite{tavares2016rock}, by restricting their strategy spaces to small sets of predefined strategies (i.e., heuristics)---in other words, by solving them as meta-games.  

One distinguishing feature of our work \emph{vis \`a vis\/} much of the existing EGTA work is that we aim to estimate all equilibria of a simulation-based game, rather than just a single one (e.g., Jordan \emph{et al.}~\cite{jordan2008searching}).
Notable exceptions include Tuyls, \emph{et al.}~\cite{tuyls2018generalised}, Vorobeychik~\cite{vorobeychik2010probabilistic}, and Wiedenbeck~\cite{Wiedenbeck:2014:AGT:2615731.2616156}.
The first of these papers shows that all equilibria of a simulation-based game are also approximate equilibria in an empirical game: i.e., they establish perfect recall with finite-sample guarantees.
The second paper derives asymptotic results about the quality of the equilibria of empirical games: i.e., they establish perfect precision in the limit, as the number of samples tends to infinity.
Our main theorem unifies these two results, obtaining finite sample guarantees for both perfect recall and approximate precision.
We obtain our results in a manner that generalizes (in theory, if not in practice) the approach taken by Tuyls, \emph{et al.}~\cite{tuyls2018generalised}, and using Rademacher averages.
%\enrique{We could obtain similar results under varied noise assumptions; e.g., we could assume (unbounded) subgaussian or subexponential noise, and substitute the appropriate Chernoff bounds.}

The third of the aforementioned works, Wiedenbeck \emph{et al.}~\cite{Wiedenbeck:2014:AGT:2615731.2616156}, is perhaps closest in spirit to our own.
There the goals, like ours, are to characterize the quality of the equilibria in empirical games, and to exploit statistical information to save on sampling.
Their methods employ bootstrapping~\cite{EfroTibs93}; as such, they do not immediately afford any theoretical guarantees.  Still, it could be of interest to test our methods against theirs, under the usual EGTA assumption that little to nothing is known about how the games' utilities are distributed; but at first blush, it seems likely that neither would dominate.  Bootstrapping methods usually yield 
%smaller confidence intervals, 
stronger approximation guarantees,
but it is easy to construct examples where they are overly optimistic (e.g., when the sampling distribution is skewed, or in case there are outliers); thus, for applications that require a high degree of certainty, bootstrapping would likely not be the preferred method.

Sample complexity bounds are an essential tool in EGTA, as running the simulator is generally a computational bottleneck. In query complexity work (e.g., \cite{babichenko2016query,fearnley2015learning,jecmen2018bounding}), one seeks to bound the number of samples needed to approximate a mixed strategy Nash equilibrium. 
%Babichenko \emph{et al.\/}~\cite{babichenko2014simple} obtain asymptotic results\amy{???} to approximate three types of equilibria: Nash, correlated and coarse correlated. 
This line of work differs from our work in at least two critical aspects: (1) sampling is over mixed strategies, not noisy payoffs, and (2) one seeks a single equilibrium. Noisy payoffs may have little impact on their own, but when combined with seeking all equilibria, they are substantial, as we must account for multiple hypothesis testing (motivating our use of uniform convergence bounds). Moreover, since our methods estimate all equilibria, which essentially requires learning the entire game, lower bounds from the query complexity literature do not apply.  This difference is key; not only does estimating all equilibria yield a greater understanding of a game, single equilibria are not sufficient to estimate certain properties, such as the price of anarchy.

%\cite{fearnley2015learning,babichenko2016query} analyze the query complexity of the optimization problem of identifying approximate Nash, while \cite{jecmen2018bounding} study the query complexity of the hypothesis testing problem of determining whether a proposed strategy profile is an approximate Nash.

%The Rademacher complexity
Rademacher averages were introduced to the statistical learning theory literature for supervised learning \cite{koltchinskii2001rademacher,bartlett2002rademacher}, but have also been used in unsupervised learning problems like mining frequent itemsets \cite{riondato2015mining}, and sampling problems like betweenness centrality approximation \cite{riondato2018abra}.  
We estimate Rademacher averages using Monte-Carlo simulations, as suggested by Bartlett and Mendelson \cite{bartlett2002rademacher}; doing so, yields very tight generalization bounds.  Although a small number of supervised learning papers, including learning decision tree prunings \cite{kaariainen2004selective},
%\cyrus{Eli, do you have any publications with Lorenzo in this space?} % RadeFWER takes a similar approach, but is unpublished.
take this approach, computation of the requisite suprema is often intractable, 
%(e.g., when the hypothesis space is infinite, or when negative terms introduce non-convexities), 
%\amy{Many machine learning problems are over infinite hypothesis spaces, and even convex problems can become non-convex when some terms are negated.}
leading most to rely on looser analytical bounds instead.%
\footnote{Loose analytical bounds can be valuable, for the insight they provide into when the sample complexity is high or low.  We pursue this approach in Appendix~\ref{sec:comparingBounds}.}
In our application domain, namely EGTA as opposed to machine learning, simulations dominate run time, so effort that is spent computing more accurate bounds is well compensated for in the simulation savings that ensue.

%To supplement our Monte-Carlo bounds,\amy{bounds? what about ``approach" or ``estimate of the Rademacher complexity"} which we show experimentally outperform competing techniques \enrique{unfortunately, for this paper we cannot show this experimentally},

\amy{PAC-learnable paper?}

==> templates/aamas/aamas_footer.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% bibliography: see CFP for number of permitted pages

\bibliographystyle{ACM-Reference-Format}  % do not change this line!
\bibliography{bibliography}  % put name of your .bib file here

\end{document}

==> templates/aamas/one_column_footer.tex <==
\bibliographystyle{alpha} 
\bibliography{bibliography}  % put name of your .bib file here

\end{document}

==> templates/ec/ec_footer.tex <==
\end{document}

==> test.tex <==
$\PlayerUtilFun{\PlayerIndex}{\MixedStratProfileAlt}$
and
$\PlayerEstimatedUtilFun{\PlayerIndex}{\MixedStratProfileAlt}$
are not working!

\begin{enumerate}
    \item $\EstimatedUtility$
    \item $\EstimatedUtilityTwoParam{1}{2}$
    \item $\EstimatedUtilityOneParam{1}$     % Does not look good!
    \item $\EstimatedUtilityDistribution{1}$         % Does not look good!
    \item $\EstimatedUtilitySamples{1}$      % Does not look good!
    \item $\EstimatedUtilitySamplePoint{1}$ 
    \item $\EstimatedPlayerUtilityTwoParam{1}{2}{3}$
    \item $\EstimatedPlayerUtilityOneParam{1}{2}$       
    \item $\EstimatedPlayerUtilityDistribution{1}{2}$           
    \item $\EstimatedPlayerUtilitySamples{1}{2}$        
    \item $\EstimatedPlayerUtilitySamplePoint{1}{2}$    
\end{enumerate}

